Unipotent Representations of Complex Groups and Extended Sommers Duality

Let $G$ be a complex reductive algebraic group. In arXiv:2108.03453, we have defined a finite set of irreducible admissible representations of $G$ called `unipotent representations', generalizing the special unipotent representations of Arthur and Barbasch-Vogan. These representations are defined in terms of filtered quantizations of symplectic singularities and are expected to form the building blocks of the unitary dual of $G$. In this paper, we provide a description of these representations in terms of the Langlands dual group $G^{\vee}$. To this end, we construct a duality map $D$ from the set of pairs $(\mathbb{O}^{\vee},\bar{C})$ consisting of a nilpotent orbit $\mathbb{O}^{\vee} \subset \mathfrak{g}^{\vee}$ and a conjugacy class $\bar{C}$ in Lusztig's canonical quotient $\bar{A}(\mathbb{O}^{\vee})$ to the set of finite covers of nilpotent orbits in $\mathfrak{g}^*$.

==> Gamma.tex <==


Here, we describe...

\vspace{5mm}

\underline{$G_2$}. The only non-trivial cases are $\OO^\vee_1=A_1$ and $\OO^\vee_2=\widetilde{A}_1$. The covers $D(\OO^\vee_1)$ and $D(\OO^\vee_2)$ are birationally induced from the $\{0\}$ orbit in $\widetilde{A}_1$ and $A_1$ respectively. Thus, $D(\OO^\vee_1)$ is a $3$-fold cover of $G_2(a_1)$, and $D(\OO^\vee_2)=G_2(a_1)$, see \cite[Example 8.5.1]{LMBM}. In both cases the Galois group of the respective cover is trivial.

\vspace{5mm}

\underline{$F_4$}. Proposition \ref{prop:even} proves statement for orbits $A_1$, $A_1+\widetilde{A}_1$, $\widetilde{A}_2$, $A_1+\widetilde{A}_2$, and $C_3$. 

We know that there is a unique birationally pair $(L, \OO_L)$, such that $\OO_L$ is birationally rigid, and $F_4(a_1)=\Bind_L^G \OO_L$. Therefore, $\Bind_{A_1}^{F_4} \{0\}$ is the $2$-fold (universal) cover of $F_4(a_1)$. For the orbit $F_4(a_3)$ statement follows from the construction of $D$.

We focus on orbits $A_2+\widetilde{A}_1$, $B_2$, and $C_3(a_1)$. The dual orbit is $\OO=F_4(a_3)$, and $A(\OO)=S_4$. We use Atlas computations to find the central characters of the unipotent ideals corresponding to these covers, i.e. $\frac{1}{2}h^\vee$, and the number of irreducible HC bimodules with these central characters. The answers are $1$, $2$ and $2$ respectively, which determine the Galois group uniquely.

\vspace{5mm}

\underline{$E_6$}. We are interested only in $\OO^\vee$, such that $\OO=D(\OO^\vee)$ has non-trivial $A(\OO)$. Note that the map $D$ is injective. Therefore, if $A(\OO)\simeq S_2$, it is enough to find the birationally rigid datum for $\OO$. In all cases that can be done using \cref{Jacobson-Morozov}.

Therefore, it remains to consider the orbit $\OO=D_4(a_1)$. \cref{Jacobson-Morozov} proves statement for the orbit $\OO^\vee=2A_2+A_1$. Set $\widetilde{\OO}=\Bind_{A_3+A_1}^{E_6} \{0\}$. By the transitivity of birational induction, we have  $\widetilde{\OO}=\Bind_{D_5}^{E_6} \Bind_{A_3+A_1}^{D_5} \{0\}$. Since the orbit $\Bind_{A_3+A_1}^{D_5} \{0\}=(3^2, 1^4)$, we have $\widetilde{\OO}=\Bind_{D_5}^{E_6} (3^2, 1^4)$. We note that the orbit $(3^2, 1^4)\subset \fs\fo(10)$ has a codimension $2$ orbit in the closure with the corresponding singularity of type $A_1$. It follows that $\Spec(\CC[\widetilde{\OO}])$ has codimension $2$ leaves.

We have $A(\OO)\simeq S_3$, and there is a unique codimension $2$ orbit $\OO'=A_3+A_1\subset \overline{\OO}$ with the corresponding singularity of type $A_1$. We claim that $\widetilde{\OO}$ is a $3$-fold cover of $\OO$. Indeed, if degree of $\widetilde{\OO}$ is even, the universal cover $\widehat{\OO}$ is not $2$-leafless. Set $\widehat{X}=\Spec(\CC[\widehat{\OO}])$. Since $A(\OO')\simeq 1$, \cite[Lemma 7.6.13]{LMBM} implies that $\dim \fP^{\widehat{X}}\ge 6$. It contradicts to Lemma 7.6.14 in \emph{loc. cit.} So $\widetilde{\OO}$ is a $3$-fold cover of $\OO$, and the corresponding Galois group is trivial. 

On the other hand, $\Bind_{D_4}^{E_6} (2^2, 1^4)=\Bind_{D_5}^{E_6} \Bind_{D_4}^{D_5} (2^2, 1^4)$, and $\Bind_{D_4}^{D_5} (2^2, 1^4)$ is the $2$-fold (universal) cover of $(3^2, 1^4)$. Therefore, $D(D_4(a_1))$ is the universal cover of $D_4(a_1)$, and statement follows.

\vspace{5mm}

\underline{$E_7$}. If $A(\OO)\simeq S_2$, and $\OO$ is not one of $D_5(a_1)$, $A_4+A_1$, $D_4(a_1)+A_1$, $A_3+A_2$, $A_2+A_1$, we prove statement using \cref{Jacobson-Morozov} analogously to how it was done for $E_6$. 

Suppose that $\OO^\vee=A_4$. We need to show that the dual orbit $\OO=D_5(a_1)$ cannot be birationally induced from the Levi $A_4\subset E_7$. Set $X=\Spec(\CC[\OO])$. By \cite{fuetal2015}, we know that there is a unique codimension $2$ leaf in $X$, corresponding to the orbit $A_4+A_1$, and the monodromy action is not trivial. By \cite[Theorem 5.11]{BISWAS}, $H^2(\OO)\simeq 0$. Therefore, $\dim \fP^X=1$, and the orbit $\OO$ cannot be birationally induced from a Levi of corank $3$, such as $A_4$.

The arguments for $\OO^\vee=A_4+A_1$ and $\OO^\vee=E_6(a_1)$ are analogous, for each of them we have $\dim \fP^X=0$, the corresponding orbits $\OO=A_4+A_1$ and $\OO=A_2+A_1$ are birationally rigid.

If $\OO=D_4(a_1)+A_1$, then by \cite{fuetal2015} there are two codimension $2$ leaves in $X=\Spec(\CC[\OO])$, corresponding to the orbits $A_3+2A_1$ and $D_4(a_1)$, and the ciorresponding singularities are of type $A_1$. It follows that $\dim \fP^X\ge 2$. There is a unique pair of corank $2$ Levi $L$, and a nilpotent orbit $\OO_L\subset \fl$, such that $\OO=\Ind_L^{E_7} \OO_L$. This pair is $(A_5)', \{0\}$ \cite{deGraafElashvili}. Therefore, $\OO=\Bind_{(A_5)'}^{E_7} \{0\}$. Statement follows.

Suppose that $\OO=A_3+A_2$. Both $\OO$ and its universal cover $\widetilde{\OO}$ are birationally induced from birationally rigid orbits in corank $1$ Levis, namely $(2^2,1^6)\times \{0\}\subset D_5+A_1$ and $(3, 2^2, 1^5)\subset D_6$.
\todo{Insert an argument from Springer theory}

Consider $\OO=E_7(a_5)$. The corresponding Jacobson-Morozov Levi $L$ is of type $2A_2+A_1$, thus proving statement for $\OO^\vee=2A_2+A_1$. We note that $E_7(a_5)=\Ind_{E_6}^{E_7} D_4(a_1)$, and since $A^{E_7}(E_7(a_5))\simeq S_3 \simeq A^{E_6}(D_4(a_1))$, this induction is birational. Then statement for $\OO^\vee=(A_3+A_1)'$ and $\OO^\vee=D_4(a_1)$ follows from the earlier computation.

Finally, set $\OO=D_4(a_1)$. For $\OO^\vee=A_5+A_1$ statement follows from \cref{Jacobson-Morozov}. For $\OO^\vee=E_7(a_5)$ it is immediate from the construction. Suppose that $\OO^\vee=D_6(a_2)$. Set $\widetilde{\OO}=D(\OO^\vee)$, and $\widetilde{X}=\Spec(\CC[\widetilde{\OO}])$. We have $\dim \fP^{\widetilde{X}}=1$. The map $D$ is injective, thus $\widetilde{\OO}$ is either $2$-fold or $3$-fold cover of $\OO$. Similarly to the analogous argument for $D_4(a_1)\subset E_6$, the $2$-fold cover resolves the unique codimension $2$ singularity in $\overline{\OO}$. Since the Lie algebra $\fq$ of the reductive part $Q$ of the stabilizer of a point in $\OO$ is semisimple, it implies that if $\widetilde{\OO}$ is not birationally rigid, then it must be a $3$-fold cover of $\OO$. Therefore, the corresponding Galois group is trivial.

\vspace{5mm}

\underline{$E_8$}. If $A(\OO)=1$, we are done. If $A(\OO)=S_2$, and $\OO$ is not one of $E_7(a_3)$, $E_6(a_1)+A_1$, $D_7(a_2)$, $E_7(a_4)$, $D_6(a_1)$, $D_5(a_1)$, $A_4+2A_1$, $A_4+A_1$, $A_3+A_2$, $A_2+A_1$, then we can deduce statement from \cref{Jacobson-Morozov}.

Let us look at these orbits case by case.
\begin{itemize}
    \item[1. ]$\OO=E_7(a_3)$. By \cite{fuetal2015}, we have a unique codimension $2$ leaf $\fL$ in $X=\Spec(\CC[\OO])$, corresponding to the orbit $E_6(a_1)+A_1$, and the singularity of $\fL\subset X$ is of type $A_4$ with a non-trivial monodromy. The Lie algebra $\fq$ of the reductive part $Q$ of the stabilizer of a point in $\OO$ is semisimple. It follows that $\dim \fP^X=2$. Therefore, $\OO$ cannot be birationally induced from a corank $4$ Levi, such as $A_4$.
    \item[2.] $\OO=E_6(a_1)+A_1$. By \cite{fuetal2015}, we have a unique codimension $2$ leaf $\fL$ in $X=\Spec(\CC[\OO])$, corresponding to the orbit $D_7(a_2)$, and the singularity of $\fL\subset X$ is of type $A_2$ with a non-trivial monodromy. The Lie algebra $\fq$ of the reductive part $Q$ of the stabilizer of a point in $\OO$ is isomorphic to $\CC$. It follows that $\dim \fP^X \le 2$. Therefore, $\OO$ cannot be birationally induced from a corank $3$ Levi, such as $A_4+A_1$.
    \item[3.] $\OO=D_7(a_2)$. Consider the Levi $D_7\subset E_8$, and set $\OO_L=(3^4, 1^2)$. We note that $\pi_1^L(\OO_L)\simeq \ZZ/2\ZZ$, and that $\OO_L=\Bind_{2A_3}^{D_7}\{0\}$, and $\OO_L=\Ind_{A_4+2A_1}^{D_7} \{0\}$, where the latter induction is not birational. Statement follows immediately.
    \item[4.] $\OO=E_7(a_4)$. Consider the Levi $E_7\subset E_8$, and set $\OO_L=A_3+A_2$. We note that $\pi_1^L(\OO_L)\simeq \ZZ/2\ZZ$. It is enough to show that $\OO_L=\Bind_{D_5+A_1}^{E_7} (2^2, 1^6)\times \{0\}$. That was proved above.
    \item[5.] $\OO=D_6(a_1)$. By \cite{fuetal2015}, we have two codimension $2$ leaves $\fL_1$, $\fL_2$ in $X=\Spec(\CC[\OO])$, corresponding to the orbits $D_5+A_1$ and $E_8(a_7)$ respectively. The singularity of $\fL_i\subset X$ is of type $A_1$ and $D_4$ with a monodromy action that quotients through $S_3$. It follows that $\dim \fP^X \ge 3$. There is a unique pair of corank $3$ Levi $L$, and a nilpotent orbit $\OO_L\subset \fl$, such that $\OO=\Ind_L^{E_8} \OO_L$. This pair is $A_5, \{0\}$ \cite{deGraafElashvili}. Therefore, $\OO=\Bind_{A_5}^{E_8} \{0\}$. Statement follows. \item[6.] $\OO=D_5(a_1)$. By \cite{fuetal2015}, we have a unique codimension $2$ leaf $\fL$ in $X=\Spec(\CC[\OO])$, corresponding to the orbit $A_4+A_1$, and the singularity of $\fL\subset X$ is of type $A_2$ with a non-trivial monodromy. The Lie algebra $\fq$ of the reductive part $Q$ of the stabilizer of a point in $\OO$ is semisimple. Therefore, $\dim \fP^X=1$, and $\OO$ cannot be birationally induced from a corank $2$ Levi $E_6$.
    \item[7.] $\OO=A_3+A_2$. Both $\OO$ and its universal cover $\widetilde{\OO}$ are birationally induced from birationally rigid orbits in corank $1$ Levis, namely $(2^2,1^6)\subset D_7$ and $2A_1\subset E_7$. We will need \todo{Springer theory}.
    \item[8.] $\OO=A_4+2A_1$, $A_4+A_1$ or $A_2+A_1$. These orbits are  birationally rigid, \cite[Proposition 3.8.3]{MBMat}, and therefore cannot be birationally induced from any proper Levi.
\end{itemize}
Next, we turn our attention to the special orbits $\OO$ with $A(\OO)\simeq S_3$.
\begin{itemize}
    \item[1.] $\OO=E_8(b_5)$. We note that $\OO=\Bind_{E_7}^{E_8} E_7(a_5)$, and $A(\OO)=A^{E_7}(E_7(a_5))$. Thus, statement follows from the one already considered above.
    \item[2.] $\OO=E_8(a_6)$. Statement for $\OO^\vee=2A_2+2A_1$ follows from \cref{Jacobson-Morozov}. By \cite{fuetal2015}, there is a unique codimension $2$ symplectic leaf $\fL\subset X=\Spec(\CC[\OO])$, corresponding to the orbit $D_7(a_1)$. The corresponding singularity is of type $A_3$ with a non-trivial monodromy action.
    
    We denote $\widetilde{\OO}^i$ to be an $i$-th fold cover of $\OO$, where $i$ is $2$, $3$ or $6$, and $\widetilde{X}^i=\Spec(\CC[\widetilde{\OO}^i])$. Set $\pi_i$ to be the map $\widetilde{X}^i\to X$, and $\widetilde{\fL}^i=\pi_i^{-1}(\fL)$. We claim that $\widetilde{X}^2$ has a unique codimension $2$ leaf with the corresponding singularity of type $A_1$. Indeed, if the singularity of (a connected component of) $\widetilde{\fL}^2$ is of type $A_3$, then the same is true for $\widetilde{\fL}^6$. Therefore, by \cite[Lemma 7.6.13]{LMBM} we have $\dim \fP^{\widetilde{X}^6}\ge 6$. But $\OO$ cannot be induced from any Levi of corank $6$. Thus, the corresponding singularity is of type $A_1$. Similarly, if $\widetilde{\fL}^2$ has $2$ connected components, then $\widetilde{\fL}^6$ has $6$ connected components because $A(D_7(a_1))\simeq \ZZ/2\ZZ$. So $\dim \fP^{\widetilde{X}^6}\ge 6$. The claim follows. As a corollary we have that $\widetilde{X}_6$ has $3$ codimension $2$ symplectic leaves, that are connected components of $\widetilde{\fL}^6$, and the corresponding singularities are of type $A_1$. The reductive part $Q$ of the stabilizer of a point in $\OO$ is trivial. Thus, we have $\dim \fP^{\widetilde{X}^2}=1$, and $\dim \fP^{\widetilde{X}^6}=3$. It follows that $\Bind_{D_4+A_1}^{E_8}(2^2, 1^4)\times \{0\}=\widetilde{\OO}^6$, and $\Bind_{A_3+2A_1}^{E_8}\{0\}\times \{0\}\sim \widetilde{\OO}^3$. The corresponding Galois groups are $S_3$ and $1$ respectively.
    \item[3.] $\OO=E_8(b_6)$. Statement for $\OO^\vee=A_3+A_2+A_1$ follows from \cref{Jacobson-Morozov}. By \cite{fuetal2015}, there are two $2$ symplectic leaf $\fL_1$, $\fL_2\subset X=\Spec(\CC[\OO])$, corresponding to the orbits $E_6(a_1)+A_1$ and $A_7$ respectively. The corresponding singularity is of type $A_2$ with a non-trivial monodromy action, and of type $A_1$ respectively.
    
    Let $\widetilde{\OO}^j$, $\widetilde{X}^j$, $\widetilde{\fL}_i^J$ be as above. We claim that $\widetilde{\fL}_2^2\subset \widetilde{X}^{2, reg}$. Indeed, suppose that the singularity of (a connected component of) $\widetilde{\fL}_2$ is of type $A_1$. Since $A(A_7)\simeq 1$, $\widetilde{\fL}_2$ has two connected components. The singularity of type $A_2$ cannot be resolved by taking a $2$-fold cover, therefore $\dim \fP^{\widetilde{X}^2}\ge 3$. But $\OO$ cannot be induced from any Levi of corank $3$. 
    
    A similar argument shows that $\widetilde{\fL}_1^3\subset \widetilde{X}^3$. Otherwise, we would have $\dim \fp^{\widetilde{X}^6}\ge 3$. The reductive part $Q$ of the stabilizer of a point in $\OO$ is trivial. It follows that $\dim \fP^{\widetilde{X}^2}$ is either $1$ or $2$, $\dim \fP^{\widetilde{X}^6}=0$, and $\dim \fP^{\widetilde{X}^3}$ is either $1$ or $3$ (by looking at all possible $3$-fold covers of singularity of type $A_1$). Thus, $\dim \fP^{\widetilde{X}^3}=1$ because $\OO$ cannot be induced from any Levi of corank $3$.
    
    It follows that $\Bind_{D_4+A_2}^{E_8}(2^2, 1^4)\times \{0\}=\widetilde{\OO}^2$, the corresponding Galois group is $S_2$.
    \item[4.] $\OO=D_4(a_1)$. For $\OO^\vee=E_6+A_1$, statement follows from \cref{Jacobson-Morozov}. For $\OO^\vee=E_8(b_5)$ it comes from the definition of the map $D$. By \cite{fuetal2015}, there is a unique codimension $2$ symplectic leaf $\fL\subset X=\Spec(\CC[\OO])$, corresponding to the orbit $A_3+A_1$. The corresponding singularity is of type $A_1$.

    Since the universal cover is birationally rigid, the $2$-fold cover is $2$-leafless. and therefore birationally rigid. It follows that $\Bind_{E_7}^{E_8}2A_1\sim \widetilde{\OO}^3$, and the corresponding Galois group is trivial.
\end{itemize}

Finally, we consider the orbit $\OO=E_8(a_7)$. For $\OO^\vee=A_4+A_3$ statement follows from \cref{Jacobson-Morozov}. For $\OO^\vee=E_8(a_7)$ it is immediate from the definition.

==> comment.tex <==
 \begin{comment}
        1) Assume that $a_t>0$. Then $b_s=0$, otherwise we have $c=0$, such that no $a_i$ and no $b_j$ equal to $c$. If $a_t>1$, then $b_{s-1}=1$. Set $\mu'=(2a_1-3, 2a_2-3, \ldots, 2a_t-3)$, and $\nu'=(2b_1-3, \ldots, 2b_{s-2}-3)$. A direct computation shows that $(\mu\cup \nu^C)^t=(t+s-1, t+s-1, t+s-1, t+s-1)\cup (\mu'\cup \nu'^C)^t$. We note that $\sum_{i=5}^{k}a_i=t+s-1-a_4\ge t+s-3$, so the statement follows.
        
        Thus, we have $a_t=1$, and $b_s=0$. We will first need to establish this statement for the case when $t=1$, and therefore $\mu=(3)$. By the discussion above $\nu=(2s-1, 2s-3, \ldots, 1)$, and $s$ is odd. Since we will use this computation later in a bit different setting we omit the requirement that $s$ is even, and consider both cases. 
        A direct computation shows that 
        \begin{align*}
            (\mu\cup \nu^C)^t=(s^3, s-1, s-3^4, s-5^4, \ldots,  2^4) \mbox{ if } s \mbox{ is odd};\\
            (\mu\cup \nu^C)^t=(s^3, s-1, s-3^4, s-5^4, \ldots,  1^4) \mbox{ if } s \mbox{ is even}.
        \end{align*}
        Thus,
        \begin{align*}
            (\mu\cup \nu^C)^t_C=(s^2, s-1^2, s-3^4, s-5^4, \ldots,  2^4, 1) \mbox{ if } s \mbox{ is odd};\\
            (\mu\cup \nu^C)^t_C=(s^3, s-2^2, s-3^2, s-4^2, s-5^2, \ldots,  1^2) \mbox{ if } s \mbox{ is even}.
        \end{align*}
        
        It is easy to see that the conditions for admitting a birationally rigid cover are satisfied.
         
        Assume that $t>1$. Set $l=a_{t-1}$, and set $\mu'=(2a_1-l-1, \ldots, 2a_{t-2}-l-1)$. Consider the number $p$ of all $i\le s$ such that $b_i\le l-1$ if $i$ is even, and $b_i\le l$ if $i$ is odd. If $p$ is even, set $\nu'=(2b_1-2l-1, \ldots, 2b_{s-p}-2l-1)$. If $p$ is odd, set $\nu'=(2b_1-2l-1, \ldots, 2b_{s-p}-2l-1, 1)$.
        
        We note that for all $i\le l-1$ we have $b_{s-i}=i$. 
        
        If $l$ is odd then for all $i\le l-1$ we have $b_{s-i}\le l-1$, and $b_{s-l}\ge l$, and therefore $p=l$ is odd. 
        
        Analogously, if $l$ is even then for all $i\le l-1$ we have $b_{s-i}\le l-1$, and $b_{s-l-1}\ge l+1$. Therefore, $p=l+1$ if $b_{s-l}=l$, and $p=l$ if $b_{s-l}\ge l+1$.
        
        A direct computation very similar to the one for the case $t=1$ shows that 
        \begin{align*}
            (\mu\cup \nu^C)^t=(s+t-1^3, s+t-2, s+t-4^4, \ldots,  s+t-p+1^4) \cup (\sum_{i=2p-1}^k m_i, \sum_{i=2p}^k m_i, \ldots, m_k).
        \end{align*}
        
        It follows that
        
        \begin{align*}
            (\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-2^2, s+t-3^2, s+t-4^2, \ldots,  s+t-p+1^2) \cup\\
            (\sum_{i=2p-1}^k m_i+1, \sum_{i=2p}^k m_i, \ldots, m_k)_C.
        \end{align*}
        
        We need to give a separate (although similar) argument for each of the cases of parity of $l$ and $p$
        \begin{itemize}
            \item $l$ is odd, $p$ is odd. Then $\mu\cup \nu^C=(\ldots, 2l+1, 2l-2^2, 2l-6^2, \ldots, 4^2,3)$. We have
            \begin{align*}
            (\mu\cup \nu^C)^t=(s+t-1^3, s+t-2, s+t-4^4, \ldots,  s+t-p+1^4, s+t-p-1^3, s+t-p-2) \cup \\
            (\sum_{i=2l+3}^k m_i, \sum_{i=2l+3}^k m_i, \ldots, m_k).
        \end{align*}
            Taking a C-collapse we get 
            \begin{align*}
            (\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-3^2, s+t-4^2, \ldots,  s+t-p^2, s+t-p-1^2, s+t-p-2) \cup \\
            (\sum_{i=2l+3}^k m_i, \sum_{i=2l+4}^k m_i, \ldots, m_k)^{+}_C,
        \end{align*}
        where $\bullet^{+}$ stands for adding $1$ to the first element of partition that is less than $s+t-p-2$. Since $s+t-p-2$ is even, we have $(\sum_{i=2l+3}^k m_i, \sum_{i=2l+4}^k m_i, \ldots, m_k)^{+}_C=(\sum_{i=2l+3}^k m_i+1, \sum_{i=2l+4}^k m_i, \ldots, m_k)_C$.
        
            We note that $(\sum_{i=2l+3}^k m_i+1, \sum_{i=2l+4}^k m_i, \ldots, m_k)=(\mu'\cup \nu'^C)^t$, and therefore  
            \begin{align*}
            (\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-3^2, s+t-4^2, \ldots,  s+t-p-1^2, s+t-p-2^2) \cup (\mu'\cup \nu'^C)^t_C.
        \end{align*}
        Since $\sum_{i=2l+3}^k m_i+1= s+t-p-2-m_{2l+2}+1\ge s+t-p-3$, it follows that $(\mu\cup \nu^C)^t_C$ admits a two-leafless cover.
        
        \item $l$ is even, $p$ is odd. Then $\mu\cup \nu^C=(\ldots, 2l+1, 2l^2, 2l-4^2, \ldots, 4^2,3)$, and the multiplicity of $2l+2$ equals $0$. We have
            \begin{align*}
            (\mu\cup \nu^C)^t=(s+t-1^3, s+t-2, s+t-4^4, \ldots,  s+t-p+1^4, s+t-p-1, s+t-p-2) \cup \\
            (\sum_{i=2l+3}^k m_i, \sum_{i=2l+4}^k m_i, \ldots, m_k).
        \end{align*}
            Taking a C-collapse we get 
            \begin{align*}
            (\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-3^2, s+t-4^2, \ldots,  s+t-p^2, s+t-p-2) \cup \\
            (\sum_{i=2l+3}^k m_i, \sum_{i=2l+4}^k m_i, \ldots, m_k)_C,
        \end{align*}
        
            We note that $(\sum_{i=2l+3}^k m_i, \sum_{i=2l+4}^k m_i, \ldots, m_k)=(\mu'\cup \nu'^C)^t$, and therefore  
            \begin{align*}
            (\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-3^2, s+t-4^2, \ldots,  s+t-p-1^2, s+t-p-2^2) \cup (\mu'\cup \nu'^C)^t_C.
        \end{align*}
        Since $\sum_{i=2l+3}^k m_i= s+t-p-2-m_{2l+2}=s+t-p-2$, it follows that $(\mu\cup \nu^C)^t_C$ admits a birationally rigid cover.
        
         \item $l$ is even, $p$ is even. Then $\mu\cup \nu^C=(\ldots, 2l+1, 2l, 2l-4^2, \ldots, 4^2,3)$, and the multiplicity of $2l+2$ equals $0$. We have
            \begin{align*}
            (\mu\cup \nu^C)^t=(s+t-1^3, s+t-2, s+t-4^4, \ldots,  s+t-p^4, s+t-p-1, s+t-p-2) \cup \\
            (\sum_{i=2l+3}^k m_i, \sum_{i=2l+4}^k m_i, \ldots, m_k).
        \end{align*}
            Taking a C-collapse we get 
            \begin{align*}
            (\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-3^2, s+t-4^2, \ldots,  s+t-p^2, s+t-p-1^3) \cup \\
            (\sum_{i=2l+3}^k m_i, \sum_{i=2l+4}^k m_i, \ldots, m_k)_C,
        \end{align*}
        
            We note that $(\sum_{i=2l+3}^k m_i, \sum_{i=2l+4}^k m_i, \ldots, m_k)=(\mu'\cup \nu'^C)^t$, and therefore  
            \begin{align*}
            (\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-3^2, s+t-4^2, \ldots,  s+t-p^2, s+t-p-1^3) \cup (\mu'\cup \nu'^C)^t_C.
        \end{align*}
        Since $\sum_{i=2l+3}^k m_i= s+t-p-1-m_{2l+2}\ge s+t-p-3$, it follows that $(\mu\cup \nu^C)^t_C$ admits a birationally rigid cover.
        
        \end{itemize}
        \end{comment}
        
        
        
        Assume that $\fg$ is exceptional. From \cite{LMBM} we already know the result for $c=1$, so we can assume that $c$ is non-trivial. Note that we can restrict attention to a conjugacy class $c\in \overline{A}(\OO)$. In the tables below for each distinguished pair $(\OO^\vee, c)$ with $c\neq 1$ we list the dual orbit $\OO=d_S(\OO^\vee, c)$. 
        
        $\fg=G_2$
         \begin{table}[H]
        \begin{tabular}{|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$ \\ \hline
           $(G_2(a_1), (12))$ & $\widetilde{A}_1$ & $1$ & $A_1$ & & $A_1$\\ \hline
           $(G_2(a_1), (123))$ & ${A}_1$ & $1$ & & & $A_1$\\ \hline
        \end{tabular}
    \end{table}
    In both cases $\Spec(\CC[\OO])$ has no codimension $2$ leaves, and $H^2(\OO,\CC)=\fz(\fq)=0$. Therefore, $\Spec(\CC[\OO])$ is $\QQ$-factorial terminal, and $\OO$ is birationally rigid.
    
    $\fg=F_4$
    
        For $(A_1, (12))$ and $(A_2, (12))$ we look at the Levi of type $B_3$, get $\pi_1^L\simeq \ZZ_2$.
        
        For $(C_3(a_1), (12))$ for Levi $L=C_3$, we have $\pi_1^L\simeq \ZZ_2$.
        For $(B_2, (12))$ take Levi $L=B_3$, we have $\pi_1^L\simeq \ZZ_2$.
         \begin{table}[H]
        \begin{tabular}{|c|c|c|c|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$ & $\pi_1(\OO)$& $\OO'\subset \overline{\OO}$ & not type $m$ & $\fq$ \\ \hline
           $(F_4(a_1), (12))$ & $A_1$ & $1$ &  & & $C_3$\\ \hline
           $(F_4(a_2), (12))$ & ${A}_1+\widetilde{A}_1$ & $1$ & & & $2A_1$\\ \hline
           $(F_4(a_3), (12))$ & $C_3(a_1)$ & $S_2$ & $\widetilde{A_2}+A_1$, $B_2$ & $B_2$ & $A_1$\\ \hline
           $(F_4(a_3), (123))$ & $A_1+\widetilde{A_2}$ & $1$ & $\widetilde{A_1}+A_2$ & & $A_1$\\ \hline
           $(F_4(a_3), (12)(34))$ & $B_2$ & $S_2$ & $\widetilde{A_1}+A_2$ & $\widetilde{A_1}+A_2$ & $2A_1$\\ \hline
           $(F_4(a_3), (1234))$ & $A_2+\widetilde{A}_1$ & $1$ & & & $A_1$\\ \hline
        \end{tabular}
    \end{table}
    
    We note that in all cases $\fz(\fq)=0$, so it is enough that the affinization $\Spec(\CC[\widehat{\OO}])$ of the universal cover $\widehat{\OO}$ of $\OO$ has no codimension $2$ orbits. We can focus on the codimension $2$ orbits with the singularities not of type $m$. 
    
    Let $\OO=C_3(a_1)$ and $\OO'=B_2$. The corresponding singularity of $\OO'\subset \overline{\OO}$ is of type $2A_1$. Assume that $X=\Spec(\CC[\widehat[\OO])$ is singular in codimension $2$. Since $\pi_1(\OO')\simeq S_2$, there are at least $2$ singular symplectic leaves over $\OO'$, and thus $\dim \fP^X\ge 2$. However, by \cite[Tables]{deGraafElashvili} ${\OO}$ cannot be induced from any Levi of corank $2$, leading to a contradiction. Therefore, $\Spec(\CC[\widehat{\OO}])$ is $\QQ$-factorial terminal, and $\widehat{\OO}$ is birationally rigid.
    
    Let $\OO=B_2$ and $\OO'=\widetilde{A}_1+A_2$. The corresponding singularity of $\OO'\subset \overline{\OO}$ is of type $A_1$. Assume that $X=\Spec(\CC[\widehat[\OO])$ is singular in codimension $2$. Since $\pi_1(\OO')\simeq 1$, there are at least $2$ singular symplectic leaves over $\OO'$, and thus $\dim \fP^X\ge 2$. However, by \cite[Tables]{deGraafElashvili} ${\OO}$ cannot be induced from any Levi of corank $2$, leading to a contradiction. Therefore, $\Spec(\CC[\widehat{\OO}])$ is $\QQ$-factorial terminal, and $\widehat{\OO}$ is birationally rigid.
    
     $\fg=E_6$
     
        For $(D_4(a_1), (12))$ take $L=D_5$, get $\pi_1^L\simeq \ZZ_2$.
        For $(A_2, (12))$ take $L=D_5$, get $\pi_1^L\simeq \ZZ_2$.
        \begin{table}[H]
        \begin{tabular}{|c|c|c|c|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$ & $\pi_1(\OO)$& $\OO'\subset \overline{\OO}$ & not type $m$ & $\fq$ \\ \hline
           $(E_6(a_3), (12))$ & $3A_1$ & $1$ &  & & $A_2+A_1$\\ \hline
           $(D_4(a_1), (123))$ & $2A_2+A_1$ & $\ZZ_3$ & & & $A_1$\\ \hline
        \end{tabular}
    \end{table}
    
    In both cases $\Spec(\CC[\widehat{\OO}])$ has no codimension $2$ leaves, and $H^2(\widehat{\OO},\CC)=\fz(\fq)=0$. Therefore, $\Spec(\CC[\widehat{\OO}])$ is $\QQ$-factorial terminal, and $\widehat{\OO}$ is birationally rigid.
    
    $\fg=E_7$
    
        For $(E_6(a_3), (12))$ take $L=E_6$, get $\pi_1^L\simeq \ZZ_2$.
        For $(D_4(a_1), (12))$ and $(D_4(a_1), (123))$ take $L=E_6$, get $\pi_1^L\simeq S_3$.
        For $(A_2, (12))$ take $L=E_6$, get $\pi_1^L\simeq \ZZ_2$.
        
        For $(D_5(a_1), (12))$ and $(D_4(a_1)+A_1, (12))$ take $L=D_6$, we get $\pi_1^L\simeq \ZZ_2$.
        For  $(A_4, (12))$, $(A_3+A_2, (12))$ and $(A_2+A_1, (12))$ take $L=D_6$, we get $\pi_1^L\simeq \ZZ_2$.
        \begin{table}[H]
        \begin{tabular}{|c|c|c|c|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$ & $\pi_1(\OO)$& $\OO'\subset \overline{\OO}$ & not type $m$ & $\fq$ \\ \hline
           $(E_7(a_3), (12))$ & $(3A_1)'$ & $1$ &  & & $C_3+A_1$\\ \hline
           $(E_6(a_1), (12))$ & $4A_1$ & $1$ & & & $C_3$\\ \hline
           $(E_7(a_4), (12))$ & $A_2+2A_1$ & $1$ &  & & $3A_1$\\ \hline
           $(E_7(a_5), (123))$ & $2A_2+A_1$ & $1$ &  & & $2A_1$\\ \hline
           $(E_7(a_5), (12))$ & $(A_3+A_1)'$ & $1$ & $2A_2+A_1$ & & $3A_1$\\ \hline
           $(A_4+A_1, (12))$ & $A_3+A_2+A_1$ & $\ZZ_2$ & $A_3+A_2$ & $A_3+A_2$ & $A_1$\\ \hline
         \end{tabular}
    \end{table}
    
    Let $\OO=A_3+A_2+A_1$ and $\OO'=A_3+A_2$. By \cite[Tables]{deGraafElashvili} ${\OO}$ can be induced only from the zero orbit in $A_4+A_2$. Assume that $X=\Spec(\CC[\widehat[\OO])$ is singular in codimension $2$. Then both $\OO$ and $\widehat{\OO}$ are birationally induced from a proper Levi. That leads to a contradiction. Therefore, $\Spec(\CC[\widehat{\OO}])$ is $\QQ$-factorial terminal, and $\widehat{\OO}$ is birationally rigid.
    
    $\fg=E_8$
    
        Show that $(D_4(a_1)+A_2, (12))$, and are not distinguished. 
        
        For $(E_7(a_3), (12))$, $(E_6(a_1), (12))$, $(E_6(a_3), (12))$, $(A_4+A_1, (12))$, $(A_4, (12))$, $(A_3+A_2, (12))$, $(D_4(a_1)+A_1, (12))$, $(A_2+A_1, (12))$, $(A_2, (12))$, $(D_5(a_1), (12))$, and $(D_5(a_1), (12))$ take Levi $L=E_7$, $\pi_1^L\simeq \ZZ_2$.
        For $(D_4(a_1), (12))$ and $(D_4(a_1), (123))$ take $L=E_7$, we get $\pi_1^L=S_3$.
        
        For $(D_6(a_1), (12))$, $(A_4+2A_1, (12))$, $(D_4(a_1)+A_1, (12))$, $(2A_2, (12))$, and $(D_6(a_2), (12))$ take $L=D_7$, we get $\pi_1^L\simeq \ZZ_2$.
        
        For $(E_6(a_3)+A_1, (12))$ take $L=E_6+A_1$, we get $\pi_1^L\simeq \ZZ_2$.
        
        For $(D_4(a_1)+A_2, (12))$ take $L=D_5+A_2$, we get $\pi_1^L\simeq \ZZ_2$.
        
         \begin{table}[H]
        \begin{tabular}{|c|c|c|c|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$ & $\pi_1(\OO)$& $\OO'\subset \overline{\OO}$ & not type $m$ & $\fq$ \\ \hline
           $(E_8(a_3), (12))$ & $3A_1$ & $1$ &  & & $A_4+A_1$\\ \hline
           $(E_8(a_4), (12))$ & $4A_1$ & $1$ &  & & $C_4$\\ \hline
           $(E_8(b_4), (12))$ & $A_2+2A_1$ & $1$ &  & & $B_3+A_1$\\ \hline
           $(E_8(a_5), (12))$ & $A_2+3A_1$ & $1$ &  & & $G_2+A_1$\\ \hline
           $(E_8(a_6), (123))$ & $2A_2+A_1$ & $1$ &  & & $G_2+A_1$\\ \hline
           $(E_8(a_6), (12))$ & $A_3+2A_1$ & $1$ &  & & $B_2+A_1$\\ \hline
           $(E_8(b_6), (12))$ & $A_3+A_2+A_1$ & $1$ &  & & $2A_1$\\ \hline
           $(E_6(a_1)+A_1, (12))$ & $A_3+A_2+A_1$ & $1$ &  & & $2A_1$\\ \hline
           $(D_7(a_2), (12))$ & $2A_3$ & $1$ &  & & $B_2$\\ \hline
           $(E_8(a_7), (123)(45))$ & $A_5+A_1$ & $1$ & $A_4+A_3$ & & $2A_1$\\ \hline
           $(E_8(a_7), (12345))$ & $A_4+A_3$ & $1$ & & & $A_1$\\ \hline
           $(E_8(a_7), (1234))$ & $D_5(a_1)+A_2$ & $1$ & $A_4+A_3$ & & $A_1$\\ \hline
           $(E_8(a_7), (12)(34))???$ & $D_6(a_2)$ & $\ZZ_2$ & $A_5+A_1$, $D_5(a_1)+A_2$ & $D_5(a_1)+A_2$ & $2A_1$\\ \hline
           $(E_8(a_7), (12))???$ & $E_7(a_5)$ & $S_3$ & $E_6(a_3)+A_1$, $D_6(a_2)$ & $D_6(a_2)$ & $A_1$\\ \hline
           $(E_8(a_7), (123))$ & $E_6(a_3)+A_1$ & $\ZZ_2$ & $A_5+A_1$, $D_5(a_1)+A_2$ & $A_5+A_1$ & $G_2$\\ \hline
           $(D_4(a_1)+A_1, (123))$ & $E_8(b_6)$ & $S_3$ & $E_6(a_1)+A_1$, $A_7$ & $E_6(a_1)+A_1$, $A_7$ & $1$\\ \hline
           
        \end{tabular}
    \end{table}
    \todo{Which pair goes to which orbit?} Let $\OO=D_6(a_2)$ and $\OO'=D_5(a_1)+A_2$. The corresponding singularity of $\OO'\subset \overline{\OO}$ is of type $A_1$. Assume that $X=\Spec(\CC[\widehat[\OO])$ is singular in codimension $2$. Since $\pi_1(\OO')\simeq 1$, there are at least $2$ singular symplectic leaves over $\OO'$, and thus $\dim \fP^X\ge 2$. However, by \cite[Tables]{deGraafElashvili} ${\OO}$ cannot be induced from any Levi of corank $2$, leading to a contradiction. Therefore, $\Spec(\CC[\widehat{\OO}])$ is $\QQ$-factorial terminal, and $\widehat{\OO}$ is birationally rigid.
    
    Let $\OO=E_7(a_5)$ and $\OO'=D_6(a_2)$. The corresponding singularity of $\OO'\subset \overline{\OO}$ is of type $2A_1$. Assume that $X=\Spec(\CC[\widehat[\OO])$ is singular in codimension $2$. Since $\pi_1(\OO')\simeq \ZZ_2$, there are at least $6$ singular symplectic leaves over $\OO'$, and thus $\dim \fP^X\ge 6$. However, by \cite[Tables]{deGraafElashvili} ${\OO}$ cannot be induced from any Levi of corank $6$, leading to a contradiction. Therefore, $\Spec(\CC[\widehat{\OO}])$ is $\QQ$-factorial terminal, and $\widehat{\OO}$ is birationally rigid.
    
     Let $\OO=E_6(a_3)+A_1$ and $\OO'=A_5+A_1$. The corresponding singularity of $\OO'\subset \overline{\OO}$ is of type $A_1$. Assume that $X=\Spec(\CC[\widehat[\OO])$ is singular in codimension $2$. Since $\pi_1(\OO')\simeq 1$, there are at least $2$ singular symplectic leaves over $\OO'$, and thus $\dim \fP^X\ge 2$. However, by \cite[Tables]{deGraafElashvili} ${\OO}$ cannot be induced from any Levi of corank $2$, leading to a contradiction. Therefore, $\Spec(\CC[\widehat{\OO}])$ is $\QQ$-factorial terminal, and $\widehat{\OO}$ is birationally rigid.
     
      Let $\OO=E_8(b_6)$ and $\OO'=E_6(a_1)+A_1$. The corresponding singularity of $\OO'\subset \overline{\OO}$ is of type $A_2$. Assume that $X=\Spec(\CC[\widehat[\OO])$ is singular in a preimage of a point of $\OO'$ under the natural map $X\to \overline{O}$. Since $\pi_1(\OO')\simeq \ZZ_2$, there are at least $3$ singular symplectic leaves over $\OO'$, and thus $\dim \fP^X\ge 3$. However, by \cite[Tables]{deGraafElashvili} ${\OO}$ cannot be induced from any Levi of corank $3$, leading to a contradiction.
      
      Let $\OO$ be the same, and $\OO'=A_7$. he corresponding singularity of $\OO'\subset \overline{\OO}$ is of type $A_1$. Assume that $X=\Spec(\CC[\widehat[\OO])$ is singular in a preimage of a point of $\OO'$ under the natural map $X\to \overline{O}$. Since $\pi_1(\OO')\simeq 1$, there are at least $6$ singular symplectic leaves over $\OO'$, and thus $\dim \fP^X\ge 6$. We get a contradiction. Therefore, $\Spec(\CC[\widehat{\OO}])$ is $\QQ$-factorial terminal, and $\widehat{\OO}$ is birationally rigid.
    
     
    An obvious observation is that for each $x\in N(\OO)$ the intersection $\OO\cap \fn_x$ is a dense subset of $\fn_x$, and a $B$-invariant subset of $\fn$. The irreducible components of ${\OO\cap \fn}$ are called \emph{orbital varieties} of $\OO$. Following \cite{Joseph1989} we give an alternative description of orbital varieties. 
    
    For an element $\w\in W$ we set $\fn_w=\overline{B(\fn\cap w^{-1}\fn)}\subset \fn$, and $V(w)=\fn_w\cap \OO$. Every orbital variety is of form $V(w)$, and the set of $w\in W$ leading to the same $V(w)$ is called a \emph{geometric left cell}.
    
    \begin{prop}
        The ST-regions in $N(\OO)$ are in a bijection with orbital varieties of $\OO$. 
    \end{prop}
    \begin{proof}
        Let $\cV_1, \ldots, \cV_k\subset \OO\cap \fn$ be the set of orbital varieties, and $C_1, \ldots, C_k\subset W$ be the corresponding left geometric cells. 
        
        We claim that for each ST-region $S\subset N(\OO)$ there exist $w\in W$, such that $\fn_w=\fn_S$. In \cite{Shi1987} there was constructed a map $\zeta: W_a\to \mathscr{S}$ defined as follows.
        
        For an element $w\in W_a$ let $A_w\subset \fh$ be the corresponding alcove. For each $\alpha\in \Phi^+$ there is an integer $k(w,\alpha)$, such that for any $x\in A_w$ we have $k(w,\alpha)\le \langle x, \alpha \rangle <k(w,\alpha)+1$. 
        
        To $w\in W_a$ we assign the corresponding ST-region $S_w$ by setting $X_\alpha=+$ if $k(w,\alpha)\ge 1$, $X_\alpha=0$ if $1>k(w,\alpha)\ge 0$, and $X_\alpha=-$ if $k(w,\alpha)<0$. By Theorem 2.1 in \emph{loc.cit.} $\zeta$ is surjective.
        
        For a dominant ST-region $S$ let $w'=w\chi$ for $w\in W$ and $\chi\in \ZZ \Phi$ be in the preimage of $S$ under the map $\zeta$. Since $S$ is dominant, $w=1$, and $\chi$ is dominant. Set $\Phi^+_L\subset \Phi^+$ to be a subset of all positive roots $\alpha\in \Phi^+$, such that $k(w, \alpha)=0$. It is clear that $\Phi^+_L$ is a root subsystem generated by a subset $\Delta_L\subset \Delta$ of simple roots and defines a Levi subgroup $L\subset G$. Set $w^0_L$ to be the longest element in $W_L\subset W$. 
    \end{proof}
   
   \begin{example}
        Set $\fg^\vee=Sp(4)$, and $(\OO^\vee, c)=((2^2), (12))$. Then we have $L^\vee=Sp(2)\times Sp(2)$.
        
        There are two ST-regions $S_1$ and $S_2$ in $N(\OO^\vee)$, corresponding to Borel ideals $\fg^\vee_{e_1+e_2}\oplus \fg^\vee_{e_1-e_2}\oplus \fg^\vee_{2e_1}\subset \fn^\vee$ and $\fg^\vee_{e_1+e_2}\oplus \fg^\vee_{2e_2}\oplus \fg^\vee_{2e_1}\subset \fn^\vee$.
        
        Elements of $S_1$ and $S_2$ in the standard coordinates are the elements $(a,b)$ with $a\ge b+1$, $\frac{1}{2}\ge b\ge 0$, and $a\ge b\ge \frac{1}{2}$ respectively. The minimal element of $N(\OO^\vee)$ is $(\frac{1}{2}, \frac{1}{2})$.
        
        Then elements of $S_1^L$ in standard coordinates are elements $(a,b)$ with $a\ge b+1$, $\frac{1}{2}\ge b\ge 0$, such that $2a$ and $2b$ are integral, but $a-b$ is not integral. The minimal element of $S_1^L$ is $(\frac{3}{2}, 0)$.
        
        Elements of $S_2^L$ in standard coordinates are elements $(a,b)$ with $a\ge b\ge \frac{1}{2}$, such that $2a$ and $2b$ are integral, but $a-b$ is not integral. The minimal element of $S_2^L$ is $(1, \frac{1}{2})$.
        
        Therefore, the minimal element of $N(\OO^\vee, c)$ is $(1, \frac{1}{2})$. Applying \cite[Proposition 8.2.3]{LMBM} to the birationally rigid orbit $d_S(\OO^\vee,c)$ corresponding to the partition $(2^2,1)$ we get $\gamma(d_S(\OO^\vee, c))=(1,\frac{1}{2})$, confirming conjecture in this case.
    \end{example}
    
    \begin{example}
        Set $\fg^\vee=Sp(6)$, and $(\OO^\vee, c)=((4,2), (12))$. Then we have $L^\vee=Sp(4)\times Sp(2)$.
        
        There are two ST-regions $S_1$ and $S_2$ in $N(\OO^\vee)$, corresponding to Borel ideals $\fn^\vee-\fg^\vee_{e_1-e_2}$ and $\fn^\vee-\fg^\vee_{e_2-e_3}$ respectively.
        
        Elements of $S_1$ in the standard coordinates are the elements $(a,b,c)$ with $a\ge b$, $b\ge c+1$, $c\ge \frac{1}{2}$, and $a-b<1$. The minimal element of $S_1$ is $(\frac{3}{2}, \frac{3}{2}, \frac{1}{2})$.
        
        Elements of $S_2$ in the standard coordinates are the elements $(a,b,c)$ with $a\ge b+1$, $b\ge c$, $c\ge \frac{1}{2}$, and $b-c<1$. The minimal element of $S_1$ is $(\frac{3}{2}, \frac{1}{2}, \frac{1}{2})$. Therefore, the minimal element of $N(\OO^\vee)$ is $(\frac{3}{2}, \frac{1}{2}, \frac{1}{2})$, which is exactly $\frac{1}{2}h^\vee$.
        
        Then elements of $S_1^L$ in standard coordinates are elements $(a,b,c)$ satisfying the conditions of $S_1$, and additional conditions that $2a$, $2b$, $2c$ are integral, but only one from $a-b$, $b-c$ and $a-c$ is integral. The minimal element of $S_1^L$ is $(2, \frac{3}{2}, \frac{1}{2})$.
        
        Elements of $S_2^L$ in standard coordinates are elements $(a,b,c)$, satisfying the conditions of $S_2$, and additional conditions that $2a$, $2b$, $2c$ are integral, but only one from $a-b$, $b-c$ and $a-c$ is integral. The minimal element of $S_2^L$ is $(2,\frac{1}{2},\frac{1}{2})$. 
        
        Therefore, the minimal element of $N(\OO^\vee, c)$ is $(2, \frac{1}{2},\frac{1}{2})$. Applying \cite[Proposition 8.2.3]{LMBM} to the birationally rigid orbit $d_S(\OO^\vee,c)$ corresponding to the partition $(2^2,1^3)$ we get $\gamma(d_S(\OO^\vee, c))=(\frac{3}{2}, 1, \frac{1}{2})$, that does not lie in $N(\OO^\vee)$ at all.
    \end{example}
    
    
    
    
    
    
    
    
    
    \section{ST-regions}
    \subsection{Classical case}
    We follow \cite{GunSom} to define the partition of $\fh$ in ST-regions.
    
    Namely, for an element $x\in \fh$ we assign to every positive root $\alpha\in \Phi^+$ an element $X_\alpha\in\{+, 0, -\}$ by setting $X_\alpha=+$ if $\langle \alpha, x \rangle \ge 1$, $X_\alpha=0$ if $0\le \langle \alpha, x \rangle < 1$, and $X_\alpha=-$ if $\langle \alpha, x \rangle <0$. We denote the corresponding collection $\{X_\alpha| \alpha\in \Phi^+\}$ for $x$ by $S_x$.
    
    For a given collection $S=\{X_\alpha | \alpha\in \Phi^+\}$ we define the corresponding ST-region to be the union of all $x\in \fh$, such that $S_x=S$. 
    %We note that with this definition our ST-regions are the admissible ST-regions from \cite{Shi1987}. Following the notations of Shi, let $\mathscr{S}$ be the set of all $ST$-regions.
    
    Assume that $S$ is a dominant ST-region, meaning that $X_\alpha\in {0,+}$ for each $\alpha\in \Phi^+$. Set $\fn_S=\bigoplus_{\alpha|X_{\alpha}=+} \fg_\alpha\subset \fn$. That is a $B$-stable ideal in $\fn$, and every $B$-stable ideal can be obtained this way, thus giving us a bijection between dominant ST-regions and $B$-stable ideals in $\fn$. Finally, set $\OO_S\subset \fg$ to be the unique nilpotent orbit, such that $\OO_S\cap \fn_S$ is dense. For an element $x$ of the dominant Weyl chamber $\fC$ we set $\OO_{S_x}\subset \fg$ to be the nilpotent orbit associated with the ST-region $S_x$. 
    
    For a nilpotent orbit $\OO$ we set $N(\OO)$ to be the set of all $x\in \fC$, such that $\OO_{S_x}=\OO$. It is clear that $N(\OO)$ is a finite union of ST-regions.
    
    The following theorem was proved in\cite{GunSom}.
    \begin{theorem}
        Let $\OO^\vee\subset \fg^\vee$ be a nilpotent orbit, and $(e^\vee, h^\vee, f^\vee)$ be the corresponding $\fs\fl_2$-triple, such that $h^\vee\in \fC$. Then $\frac{1}{2}h^\vee$ is the minimal element in $N(\OO^\vee)$.
    \end{theorem}
    Combining with the definition of a generalized duality map $\tilde{D}$, and \cite[Proposition 9.2.1]{LMBM} we get the following reformulation.
    
    
    \begin{theorem}
        Let $\OO^\vee\subset \fg^\vee$ be a nilpotent orbit. Then $\gamma(\tilde{D}(\OO^\vee))$ is the unique minimal element in $N(\OO^\vee)$.
    \end{theorem}
    
    \subsection{$L^\vee$-integral ST-regions}
    
    Let $(L^\vee, \OO^\vee_{L^\vee})$ be a pair of a pseudolevi subalgebra, and a nilpotent orbit in its Lie algebra. To each such pair we assign a subset $N(L^\vee, \OO^\vee_{L^\vee})$ of the dominant Weyl chamber $\fC$ as follows. Recall that for each $x\in \fh^\vee$ one can assign two root subsystems, $\Phi_{int}$ of roots $\alpha$, such that $(\alpha, x)\in \ZZ$, and $\Phi_{sing}$ of roots $\alpha$, such that $(\alpha, x)=0$. These root subsystems define (up to conjugacy class) a pseudolevi $ID(x)$ and a Levi $Sing(x)$ in $G^\vee$. We define $N(L^\vee, \OO^\vee_{L^\vee})$ to be a union of all $x\in \fC$, such that $ID(x)=L^\vee$, and $\OO^\vee_{L^\vee}=\Ind_{Sing(x)}^{ID(x)} \{0\}$. An easy observation shows that $N(L^\vee, \OO^\vee_{L^\vee})$ is empty if $\OO^\vee_{L^\vee}$ is not Richardson orbit, and for $L^\vee=G^\vee$ we have $N(G^\vee, \OO^\vee)\subset N(\OO^\vee)$. One can see that $N(L^\vee, \OO^\vee_{L^\vee})$ is always a union of $L^\vee$-integral elements in a union of ST-regions, each corresponding to the orbit $\Sat_{L^\vee}^{G^\vee} \OO^\vee_{L^\vee}$, and thus $N(L^\vee, \OO^\vee_{L^\vee})\subset N(\Sat_{L^\vee}^{G^\vee} \OO^\vee_{L^\vee})$
    
    Let $(\OO^\vee, \bar{c})$ be a pair of a nilpotent element, and a conjugacy class $\bar{c}$ of $\bar{A}(\OO^\vee)$. For each conjugacy class $c\in A(\OO^\vee)$ that maps to $\bar{c}$ under the natural quotient map $A(\OO^\vee)\to \bar{A}(\OO^\vee)$ let $L_c^\vee\subset G^\vee$ be a maximal pseudolevi defined by $c$, and $\OO_{L_c^\vee}^\vee=\OO^\vee\cap \fl_c^\vee \subset \fl_c^\vee$ be a nilpotent orbit. We define the associated region $N(\OO^\vee, \bar{c})$ to be the union of $N(L_c^\vee, \OO_{L_c^\vee}^\vee)$ for all $c$ in the preimage of $\bar{c}$. 
    We conjecture the following.
    
    \begin{conj}
        $\gamma(\tilde{d}_S(\OO^\vee,\bar{c}))$ is the unique minimal element in $N(\OO^\vee, \bar{c})$.
    \end{conj}
    
    First, we note that by the discussion above $N(\OO^\vee, \bar{c})\subset N(\OO^\vee)$. If $\bar{c}=1$, the proof of the conjecture reduces to showing that $\frac{1}{2}h^\vee\in N(\OO^\vee, \bar{c})$. We note that if $\OO^\vee$ corresponds to Bala-Carter data $(L^\vee, \OO^\vee_{L^\vee})$ then $ID(\frac{1}{2}h^\vee)=L^\vee$, and $\OO^\vee_{L^\vee}$ is induced from the Levi defined by roots $\alpha$, such that $(\alpha, h^\vee)=0$, i.e. $Sing(\frac{1}{2}h^\vee)$. The conjecture for $c=1$ follows.
    
    Below we focus on proving this conjecture for a general $c$. 
    
    We focus on classical types, the case of exceptional $\fg$ will be dealt with later. First step towards the proof will be a description of $N(L^\vee, \OO_{L^\vee}^\vee)$ for a distinguished orbit $\OO_{L^\vee}^\vee$. 
    
    \subsection{Description of $N(L^\vee, \OO_{L^\vee}^\vee)$ for a distinguished orbit}
    \todo{The proof here written for a general pseudolevi, but I think we care only about maximal ones.}
    Assume that $\fg^\vee=\fs\fo_{2n+1}$ is of type $B$. Then $L^\vee=SO(2m)\times \prod_i GL(k_i)\times SO(2l+1)$. Consider the partition of a distinguished orbit $\OO_{L^\vee}^\vee)$. For each $GL$-factor of $L^\vee$ the only distinguished orbit is the regular one. Thus, distinguished orbits in $L^\vee$ are parameterized by the pairs of partitions $(\mu, \nu)$ of $2m$ and $2l+1$ with only odd members, and the multiplicity of each member in the corresponding partition equals $1$.
    
    For $x\in N(L^\vee, \OO^\vee_{L^\vee})$ we have $ID(x)=L^\vee$, and $\OO^\vee_{L^\vee}$ is induced from the $\{0\}$ orbit in $Sing(x)$. So we should classify all possible Levi subgroups $M^\vee$ of $L^\vee$, such that $\OO^\vee_{L^\vee}=\Ind_{M^\vee}^{L^\vee} \{0\}$.
    \begin{prop}
        For a partition $\alpha$ of type $B$ or $D$ set $|\alpha|$to be the number of different members of $\alpha$, and $a(\alpha)=[\frac{|\alpha|+2}{2}]$. There are $a(\mu)a(\nu)$ different Levi subgroups $M^\vee\subset L^\vee$, such that $\OO^\vee_{L^\vee}=\Ind_{M^\vee}^{L^\vee} \{0\}$.
    \end{prop}
    \begin{proof}
        We have $\OO^\vee_{L^\vee}=\OO_\mu\times \prod_i \OO_{reg, i}\times \OO_\nu$, so the problem reduces to finding for each factor all Levi subgroups, such that the orbit is induced from the $\{0\}$ orbit in the Levi.
        
        For each $\OO_{reg,i}\subset \fs\fl(k_i)$ the only such Levi is the torus $T_i\subset GL(k_i)$. It remains to show that orbits $\OO_\mu\subset \fs\fo(2m)$ and $\OO_\nu\subset \fs\fo(2l+1)$ can be induced from the $\{0\}$ orbit in exactly $a(\mu)$ and $a(\nu)$ different Levi subgroups respectively. 
        
        We prove this statement for any distinguished orbit in $\fg=\fs\fo(n)$ corresponding to the partition $\alpha$.  First, we prove the statement for $\fg$ of type $D$ by the induction on the size of $\alpha$. Base case, when size of $\alpha$ is $0$ is trivial.
        
        First, we prove the statement for $\fg$ of type $D$.
        To prove the induction step let $L$ be a Levi subgroup, such that $\OO_\alpha=\Ind_L^G \{0\}$. We know that $L$ is conjugate to a Levi subgroup of the type $\prod_{i=1}^m GL(i)^{k_i}\times SO(l)$. Then $\alpha$ is the $B$-collapse of the partition $\beta=(1^l)+2\sum_{i=1}^m (k_i^{i})$. 
        
        Assume first that $l=0$ (that is possible only if $n$ is even). Then $\beta$ is a partition with only even members, such that $\alpha=\beta_C$. Such partition is uniquely defined by $\alpha$, namely we set $\beta_i=\alpha_{i}+1$ if $i$ is odd, and $\beta_i=\alpha_{i}-1$ if $i$ is even. Such partition $\beta$ gives rise to a unique Levi subgroup 
        $$L=\prod_{i \mbox{ odd}, i\le |a(\alpha)|} GL(i)^{\frac{\alpha_i-\alpha_{i+1}}{2}+1}\times\prod_{i \mbox{ even}, i< |a(\alpha)|} GL(i)^{\frac{\alpha_i-\alpha_{i+1}}{2}-1}. $$ 
        
        Suppose that $l>0$, and therefore $l\ge 2$. Set $t=n-\alpha_1-\alpha_2$, $G'=SO(t)$, and define a partition $\alpha'=(\alpha_3, \ldots, \alpha_k)$ of $t$. It corresponds to a distinguished orbit in $\fg^'$. Set $L'=\prod_{i=3}^m GL(i-2)^{k_i}\times SO(l-2)\subset G'$, it is clear that all orbits in $G'$ are of this form. A direct computations shows that $\OO_\alpha=\Ind_L^G \{0\}$ if and only if $\OO_{\alpha'}=\Ind_{L'}^{G'} \{0\}$. By the induction hypothesis there are $a(\alpha')$ such Levi subgroups $L'$. 
        
        Combining the two cases, we get that there are $a(\alpha')+1=a(\alpha)$ different Levi subgroups $L$, such that $\OO_\alpha=\Ind_L^G \{0\}$, thus proving the induction step. Moreover, we show that such Levis are parameterised by an even number $0\le l\le |\alpha|$. Namely, for a given $l$ we set 
        $$L=\prod_{i=1}^l GL(i)^{\frac{\alpha_i-\alpha_{i+1}}{2}}\times \prod_{i \mbox{ odd}, l<i\le |a(\alpha)|} GL(i)^{\frac{\alpha_i}-\alpha_{i+1}{2}+1}\times\prod_{i \mbox{ even}, l<i< |a(\alpha)|} GL(i)^{\frac{\alpha_i}-\alpha_{i+1}{2}-1}.$$
        
        Now, assume that $\fg$ is of type $B$, and let $L$, $\beta$ be as above. Since $n$ is odd, we have $l\ge 1$. Set $t=n-\alpha_1$, $G'=SO(t)$, and define a partition $\alpha'=(\alpha_2, \ldots, \alpha_k)$ of $t$. It corresponds to a distinguished orbit in $\fg^'$, and $\fg^'$ is of type $D$. Set $L'=\prod_{i=2}^m GL(i-1)^{k_i}\times SO(l-1)\subset G'$, it is clear that all orbits in $G'$ are of this form. A direct computations shows that $\OO_\alpha=\Ind_L^G \{0\}$ if and only if $\OO_{\alpha'}=\Ind_{L'}^{G'} \{0\}$. Thus, there are $a(\alpha')=a(\alpha)$ different Levi subgroups $L$, such that $\OO_\alpha=\Ind_L^G \{0\}$, as asserted. Moreover, they are parameterised by odd numbers $1\le l\le |a(\alpha)|$. Namely, for a given $l$ we set
        $$L=\prod_{i=1}^l GL(i)^{\frac{\alpha_i-\alpha_{i+1}}{2}}\times \prod_{i \mbox{ even}, l<i\le |a(\alpha)|} GL(i)^{\frac{\alpha_i}-\alpha_{i+1}{2}+1}\times\prod_{i \mbox{ odd}, l<i< |a(\alpha)|} GL(i)^{\frac{\alpha_i}-\alpha_{i+1}{2}-1}.$$
        
    \end{proof}
    
    
Let $(\OO,C) \in \Conj(G)$. Choose $e \in \OO$ and a semisimple element $s \in Z_G(e)$ which maps into $C$ under the natural map $Z_G(e) \twoheadrightarrow A(\OO)$. Let $S$ be a maximal torus in $Z_G(e,s)$ and let $M = Z_G(S,s)^{\circ}$. The following are true (see \cite[Section 3.2]{Sommers1998}):
\begin{enumerate}
    \item $M = Z_G(s')^{\circ}$ for a semisimple element $s' \in Z_G(e)$ which maps into $C$ under $Z_G(e) \to A(\OO)$. In particular, $M$ is a pseudolevi.
    \item $e \in \mathfrak{m}$ and the corresponding $M$-orbit $\OO_M := M \cdot e$ is distinguished.
    \item The pseudolevi $M$ is independent of $s$, up to conjugation by $G$.
\end{enumerate}




\begin{lemma}
Let $(\OO,\bar{C}) \in \Ach(G)$ be an Achar datum. Then the following are equivalent
\begin{itemize}
    \item[(i)] $(\OO,\bar{C})$ is distinguished.
    \item[(ii)] $(\OO,C)$ is distinguished, for any preimage $(\OO,C)$ of $(\OO,\bar{C})$.
    \item[(iii)] $(\OO,C)$ is distinguished, for the unique preimage $(\OO,C)$ of $(\OO,\bar{C})$ with $C \subset K$.\todo{this doesnt make sense if K is not normal...}
\end{itemize}
\end{lemma}



A \emph{Bala-Carter datum} for $G$ is a pair $(L,(\OO_L,C_L))$ consisting of a Levi subgroup $L \subset G$ and a distinguished conjugacy datum $(\OO_L,C_L) \in \Conj(L)$. Write $\BC(G)$ for the set of Bala-Carter data for $G$. Note that $G$ acts by conjugation on $\BC(G)$. The following is proved in ??.\todo{I don't think this is needed either}

\begin{prop}
The map
%
$$\mathrm{Sat}: \BC(G)/G \to \Conj(G), \qquad \mathrm{Sat}(L,(\OO_L,C_L)) = \mathrm{Sat}^G_L (\OO_L,C_L)$$
%
is a bijection.
\end{prop}



\begin{lemma}
The homomorphism (\ref{eq:iota}) is injective. \todo{I don't think this is needed}
\end{lemma}

\begin{proof}
Let $H = Z_G(e)$ and $S=Z(L)^{\circ}$. Since $L$ is a Levi subgroup, $L=Z_G(S)$. It suffices to show that $Z_L(e) \cap H^{\circ}$ is connected. Note that
%
$$Z_L(e) \cap H^{\circ} = Z_G(S,e) \cap H^{\circ}= Z_{H^{\circ}}(S)$$
%
The final group is connected since it is the centralizer of a torus in a connected algebraic group, \cite[Theorem 5.3]{Borel}
\end{proof}


We provide below a proof for $\fg^\vee=\fs\fo(2n+1)$. Take $L^\vee=SO(2m)\times SO(2n-2m+1)$, and let $\OO^\vee_{L^\vee}$ be the orbit corresponding to a pair of partitions $(\mu, \nu)$. Since the orbits corresponding to $\mu$ and $\nu$ are distinguished, we have $\mu=(2a_1+1, 2a_2+1, \ldots, 2a_t+1)$ with $t$ even, and $\nu=(2b_1+1, 2b_2+1, \ldots, 2b_s+1)$ with $s$ odd. A direct computation shows that $\nu^C=(2b_1, 2(b_2+1), 2b_3, \ldots, 2(b_{s-1}+1), 2b_s)$.
        
        Therefore, $\mu\cup \nu^C=(k^{m_k}, k-1^{m_{k-1}}, \ldots, 1^{m_1})$ with the following rules
        \begin{itemize}
            \item $m_i\le 1$ if $i$ is odd;
            \item $m_i\le 2$ if $i$ is even. Moreover, if $m_i=2$ then $m_{i-2}=m_{i+2}=0$;
            \item $m_2\le 1$. Moreover, if $m_2=1$ then $\sum_i m_i$ is odd.
        \end{itemize}
        
        Taking the transpose, we have $(\mu\cup \nu^C)^t=(\sum_{i=1}^k m_i, \sum_{i=2}^k m_i, \ldots, m_k)$. 
        We will prove that the $C$-collapse of this partition satisfies the conditions for admitting a birationally rigid cover listed above by induction on $n$. 
        
        First, assume that $n=3$, so $\fg^\vee=\fs\fo(7)$. Then the only distinguished pair $(\OO^\vee, c)$ with $c\neq 1$ is $(\OO^\vee, (12))$, where $\OO^\vee$ corresponds to a partition $(3^2,1)$. Then $d(\OO^\vee, c)$ is the orbit corresponding to the partition $(2^2, 1^2)$ that is birationally rigid.
        
        We proceed with the induction step. First, we claim that if there is $c$, such that there is no $a_i=c$ and no $b_j=c$, then the $C$-collapse of $(\mu\cup \nu^C)^t$ satisfies the conditions for admitting a birationally rigid cover. Set $q$ and $r$ to be the maximal such that $a_q>c$, and $b_r>c$ respectively. Define $\mu'=(2a'_1+1, \ldots, 2a'_t+1)$ and $\nu'=(2b'_1+1, \ldots, 2b'_s+1)$, where $a'_i=a_{i}-1$ if $i\le q$ and $a'_i=a_i$ otherwise, and $b'_j=b_j-1$ if $j\le r$ and $b'_j=b_j$ otherwise. Then $(\mu\cup \nu^C)^t$ is obtained from $(\mu'\cup \nu'^C)^t$ by adding two identical rows of the size of an already existing row in the partition. The statement easily follows. 
       
        1) Assume that $a_t=0$ and $b_s=0$. 
        
        If $a_{t-1}=1$, then we set $\mu'=(2a_1+1, \ldots, 2a_{t-2}+1)$. A direct computation shows that $(\mu\cup \nu^C)^t_i=(\mu'\cup \nu^C)^t_i$ for all $i\ge 4$. Set $\gamma$ to be the partition obtained by deleting the first four rows from $(\mu\cup \nu^C)^t$. Then we have $(\mu\cup \nu^C)^t=(s+t-1, s+t-2^2, s+t-3)\cup \gamma$, and $(\mu'\cup \nu^C)^t=(s+t-3^4)\cup \gamma$. Note that $s+t-1$ is even, and therefore $(\mu\cup \nu^C)^t_C=(s+t-1, s+t-2^2, s+t-3)\cup \gamma_C$, and $(\mu'\cup \nu^C)^t_C=(s+t-3^4)\cup \gamma_C$. We have $\gamma_1=s+t-3-m_4\ge s+t-5$. By the induction hypothesis $(\mu'\cup \nu^C)^t_C$ corresponds to an orbit admitting two-leafless cover. Therefore, the same is true for $(\mu\cup \nu^C)^t_C$.
        
        Let $a_{t-1}=l\ge  2$. Then $b_{s-i}=i$ for all $i\le l-1$. If $b_{s-2}=2$, set $\nu'=(2b_1-3, \ldots, 2b_{s-3}-3, 1)$, and $\mu'=(2a_1-3, \ldots, 2a_{t-1}-3, 1)$. We note that $(\mu\cup \nu^C)^t_{i+4}=(\mu'\cup \nu'^C)^t_{i}$ for all $i\ge 2$, and $(\mu\cup \nu^C)^t_{5}=(\mu'\cup \nu'^C)^t_{1}-1$. Set $\gamma$ to be the partition obtained from $(\mu\cup \nu^C)^t$ by deleting the first four rows.
        
        We have $(\mu\cup \nu^C)^t=(s+t-1, s+t-2^3)\cup \gamma$, and therefore $(\mu\cup \nu^C)^t_C=(s+t-1, s+t-2^2, s+t-3)\cup (\mu'\cup \nu'^C)^t_C$. Since $\sum_{i=5}^k m_i+1=s+t-4$, the statement follows.
        
        Thus, we focus on $a_{t-1}=2$, and $b_{s-2}\ge 3$. Set $\mu'=(2a_1-5, \ldots, 2a_{t-2}-5)$ and $\nu'=(2b_1-5, \ldots, 2b_{s-2}-5)$. For all $i\ge 1$ we have $(\mu\cup \nu^C)^t_{i+6}=(\mu'\cup \nu'^C)^t_{i}$, and we set $\gamma$ to be the partition obtained from $(\mu\cup \nu^C)^t$ by deleting the first six rows. 
        
        $(\mu\cup \nu^C)^t=(s+t-1, s+t-2^3, s+t-3, s+t-4)\cup \gamma$, and therefore $(\mu\cup \nu^C)^t_C=(s+t-1, s+t-2^2, s+t-3^3)\cup (\mu'\cup \nu'^C)^t_C$. Since $\sum_{i=7}^k m_i+1=s+t-4-m_6\ge s+t-5$, the statement follows.
        
        2) Assume that $a_t=0$ and $b_s\ge 1$.
        
        If $b_{s}\ge 2$, then $a_{t-1}=1$, and we proceed analogously to the same situation in the case $a_t=0$ and $b_s=0$. So we may assume that $b_s=1$.
        
        If $a_{t-1}=1$, set $\mu'=(2a_1+1, \ldots, 2a_{t-2}+1)$. For all $i\ge 1$ we have $(\mu\cup \nu^C)^t_{i+4}=(\mu'\cup \nu'^C)^t_{i}$, and we set $\gamma$ to be the partition obtained from $(\mu\cup \nu^C)^t$ by deleting the first four rows. 
        
        $(\mu\cup \nu^C)^t=(s+t, s+t-1, s+t-2, s+t-3)\cup \gamma$, and therefore $(\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-3)\cup (\mu'\cup \nu'^C)^t_C$. Since $\sum_{i=5}^k m_i=\sum_{i=4}^k m_i=s+t-3$, the statement follows.
        
        If $a_{t-1}=2$, set $\mu'=(2a_1+1, \ldots, 2a_{t-2}+1)$. For all $i\ge 1$ we have $(\mu\cup \nu^C)^t_{i+6}=(\mu'\cup \nu'^C)^t_{i}$, and we set $\gamma$ to be the partition obtained from $(\mu\cup \nu^C)^t$ by deleting the first six rows. 
        
        $(\mu\cup \nu^C)^t=(s+t, s+t-1, s+t-2^3, s+t-3)\cup \gamma$, and therefore $(\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-2^2, s+t-3)\cup (\mu'\cup \nu'^C)^t_C$. Since $\sum_{i=6}^k m_i=s+t-3-m_6\ge s+t-5$, the statement follows.
        
        If $a_{t-1}\ge 3$, then $b_{s-1}=2$. We set $\nu'=(2b_1-5, \ldots, 2b_{s-2}-5)$, and $\mu'=(2a_1-5, \ldots, 2a_{t-1}-5, 1)$. We note that $(\mu\cup \nu^C)^t_{i+6}=(\mu'\cup \nu'^C)^t_{i}$ for all $i\ge 2$, and $(\mu\cup \nu^C)^t_{7}=(\mu'\cup \nu'^C)^t_{1}-1$. Set $\gamma$ to be the partition obtained from $(\mu\cup \nu^C)^t$ by deleting the first six rows.
        
        We have $(\mu\cup \nu^C)^t=(s+t, s+t-1, s+t-2^4)\cup \gamma$, and therefore $(\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-2^2, s+t-3)\cup (\mu'\cup \nu'^C)^t_C$. Since $\sum_{i=7}^k m_i+1=s+t-2-m_6\ge s+t-4$, the statement follows.
        
        3) Assume that $a_t\ge 1$. Then $b_s=0$, otherwise we have $c=0$, such that no $a_i$ and no $b_j$ equal to $c$. If $a_t>1$, then $b_{s-1}=1$. Set $\mu'=(2a_1-3, 2a_2-3, \ldots, 2a_t-3)$, and $\nu'=(2b_1-3, \ldots, 2b_{s-2}-3)$. A direct computation shows that $(\mu\cup \nu^C)^t=(s+t-1, s+t-1, s+t-1, s+t-1)\cup (\mu'\cup \nu'^C)^t$. We note that $\sum_{i=5}^{k}m_i=s+t-1-m_4\ge s+t-3$, so the statement follows.
        
        Thus, we have $a_t=1$, and $b_s=0$. Assume that $b_{s-1}\ge 2$.
        
        If $a_{t-1}\ge 2$ set $\mu'=(2a_1-1, \ldots, 2a_{t}-1)$ and $\nu'=(2b_1-1, \ldots, 2b_{s-1}-1, 1)$. A direct computation shows that $(\mu\cup \nu^C)^t=(s+t-1^2)\cup (\mu'\cup \nu'^C)^t$. We note that $\sum_{i=3}^{k}m_i=s+t-1-m_2=s+t-1$, so the statement follows. 
        
        If $a_{t-1}=2$ set $\mu'=(2a_1+1, \ldots, 2a_{t-2}+1)$. A direct computation shows that $(\mu\cup \nu^C)^t_i=(\mu'\cup \nu^C)^t_i$ for all $i\ge 6$. Set $\gamma$ to be the partition obtained by deleting the first six rows from $(\mu\cup \nu^C)^t$. 
        Then we have $(\mu\cup \nu^C)^t=(s+t-1^3, s+t-2^2, s+t-3)\cup \gamma$, and $(\mu'\cup \nu^C)^t=(s+t-3^6)\cup \gamma$. Note that $s+t-1$ is even, and therefore $(\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-2^2, s+t-3)\cup \gamma_C$, and $(\mu'\cup \nu^C)^t_C=(s+t-3^6)\cup \gamma_C$. By the induction hypothesis $(\mu'\cup \nu^C)^t_C$ corresponds to an orbit admitting two-leafless cover. Therefore, the same is true for $(\mu\cup \nu^C)^t_C$.
        
        Now we focus on the situation when $b_{s-1}=1$. If $b_{s-2}=2$, set $\nu'=(2b_1+1, \ldots, 2b_{s-3}+1, 1)$. A direct computation shows that $(\mu\cup \nu^C)^t_i=(\mu\cup \nu'^C)^t_i$ for all $i\ge 5$. Set $\gamma$ to be the partition obtained by deleting the first five rows from $(\mu\cup \nu^C)^t$. 
        Then we have $(\mu\cup \nu^C)^t=(s+t-1^3, s+t-2, s+t-4)\cup \gamma$, and $(\mu'\cup \nu^C)^t=(s+t-3^3, s+t-4^2)\cup \gamma$. Note that $s+t-1$ is even, and therefore $(\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-3^2)\cup \gamma_C$, and $(\mu'\cup \nu^C)^t_C=(s+t-3^3, s+t-4^2)\cup \gamma_C$. We note that $\gamma_1=\sum_{i=6}^{k}m_i=s+t-4-m_5\ge s+t-5$. By the induction hypothesis $(\mu'\cup \nu^C)^t_C$ corresponds to an orbit admitting two-leafless cover. Therefore, the same is true for $(\mu\cup \nu^C)^t_C$.
        
        If $b_{s-2}\ge 3$ then $a_{t-1}=2$. Set $\mu'=(2a_1+1, \ldots, 2a_{t-2}+1)$. A direct computation shows that $(\mu\cup \nu^C)^t_i=(\mu'\cup \nu^C)^t_i$ for all $i\ge 6$. Set $\gamma$ to be the partition obtained by deleting the first six rows from $(\mu\cup \nu^C)^t$. 
        Then we have $(\mu\cup \nu^C)^t=(s+t-1^3, s+t-2, s+t-3, s+t-4)\cup \gamma$, and $(\mu'\cup \nu^C)^t=(s+t-3^4, s+t-4^2)\cup \gamma$. Note that $s+t-1$ is even, and therefore $(\mu\cup \nu^C)^t_C=(s+t-1^3, s+t-3^3)\cup \gamma_C$, and $(\mu'\cup \nu^C)^t_C=(s+t-3^4, s+t-4^2)\cup \gamma_C$. We note that $\gamma_1=\sum_{i=7}^{k}m_i=s+t-4-m_6\ge s+t-5$. By the induction hypothesis $(\mu'\cup \nu^C)^t_C$ corresponds to an orbit admitting two-leafless cover. Therefore, the same is true for $(\mu\cup \nu^C)^t_C$.
        
        
        
        Assume that $\fg$ is exceptional. From \cite{LMBM} we already know the result for $c=1$, so we can assume that $c$ is non-trivial. Note that we can restrict attention to a conjugacy class $c\in \bar{A}(\OO)$. In the tables below for each distinguished pair $(\OO^\vee, c)$ with $c\neq 1$ we list the dual orbit $\OO=d_S(\OO^\vee, c)$. 
        
        $\fg=G_2$
         \begin{table}[H]
        \begin{tabular}{|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$ \\ \hline
           $(G_2(a_1), (12))$ & $\widetilde{A}_1$ \\ \hline
           $(G_2(a_1), (123))$ & ${A}_1$ \\ \hline
        \end{tabular}
    \end{table}
    
    $\fg=F_4$
    
        For $(A_1, (12))$ and $(A_2, (12))$ we look at the Levi of type $B_3$, get $\pi_1^L\simeq \ZZ_2$.
        
        For $(C_3(a_1), (12))$ for Levi $L=C_3$, we have $\pi_1^L\simeq \ZZ_2$.
        For $(B_2, (12))$ take Levi $L=B_3$, we have $\pi_1^L\simeq \ZZ_2$.
         \begin{table}[H]
        \begin{tabular}{|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$  \\ \hline
           $(F_4(a_1), (12))$ & $A_1$\\ \hline
           $(F_4(a_2), (12))$ & ${A}_1+\widetilde{A}_1$ \\ \hline
           $(F_4(a_3), (12))$ & $C_3(a_1)$ \\ \hline
           $(F_4(a_3), (123))$ & $A_1+\widetilde{A_2}$ \\ \hline
           $(F_4(a_3), (12)(34))$ & $B_2$ \\ \hline
           $(F_4(a_3), (1234))$ & $A_2+\widetilde{A}_1$ \\ \hline
        \end{tabular}
    \end{table}
    
     $\fg=E_6$
     
        For $(D_4(a_1), (12))$ take $L=D_5$, get $\pi_1^L\simeq \ZZ_2$.
        For $(A_2, (12))$ take $L=D_5$, get $\pi_1^L\simeq \ZZ_2$.
        \begin{table}[H]
        \begin{tabular}{|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$ \\ \hline
           $(E_6(a_3), (12))$ & $3A_1$\\ \hline
           $(D_4(a_1), (123))$ & $2A_2+A_1$ \\ \hline
        \end{tabular}
    \end{table}
    
    $\fg=E_7$
    
        For $(E_6(a_3), (12))$ take $L=E_6$, get $\pi_1^L\simeq \ZZ_2$.
        For $(D_4(a_1), (12))$ and $(D_4(a_1), (123))$ take $L=E_6$, get $\pi_1^L\simeq S_3$.
        For $(A_2, (12))$ take $L=E_6$, get $\pi_1^L\simeq \ZZ_2$.
        
        For $(D_5(a_1), (12))$ and $(D_4(a_1)+A_1, (12))$ take $L=D_6$, we get $\pi_1^L\simeq \ZZ_2$.
        For  $(A_4, (12))$, $(A_3+A_2, (12))$ and $(A_2+A_1, (12))$ take $L=D_6$, we get $\pi_1^L\simeq \ZZ_2$.
        \begin{table}[H]
        \begin{tabular}{|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$  \\ \hline
           $(E_7(a_3), (12))$ & $(3A_1)'$ \\ \hline
           $(E_6(a_1), (12))$ & $4A_1$ \\ \hline
           $(E_7(a_4), (12))$ & $A_2+2A_1$ \\ \hline
           $(E_7(a_5), (123))$ & $2A_2+A_1$ \\ \hline
           $(E_7(a_5), (12))$ & $(A_3+A_1)'$ \\ \hline
           $(A_4+A_1, (12))$ & $A_3+A_2+A_1$ \\ \hline
         \end{tabular}
    \end{table}
    
    $\fg=E_8$
        
        For $(E_7(a_3), (12))$, $(E_6(a_1), (12))$, $(E_6(a_3), (12))$, $(A_4+A_1, (12))$, $(A_4, (12))$, $(A_3+A_2, (12))$, $(D_4(a_1)+A_1, (12))$, $(A_2+A_1, (12))$, $(A_2, (12))$, $(D_5(a_1), (12))$, and $(D_5(a_1), (12))$ take Levi $L=E_7$, $\pi_1^L\simeq \ZZ_2$.
        For $(D_4(a_1), (12))$ and $(D_4(a_1), (123))$ take $L=E_7$, we get $\pi_1^L=S_3$.
        
        For $(D_6(a_1), (12))$, $(A_4+2A_1, (12))$, $(2A_2, (12))$, and $(D_6(a_2), (12))$ take $L=D_7$, we get $\pi_1^L\simeq \ZZ_2$.
        
        For $(E_6(a_3)+A_1, (12))$ take $L=E_6+A_1$, we get $\pi_1^L\simeq \ZZ_2$.
        
        For $(D_4(a_1)+A_2, (12))$ take $L=D_5+A_2$, we get $\pi_1^L\simeq \ZZ_2$.
        
         \begin{table}[H]
        \begin{tabular}{|c|c|} \hline
           $(\OO^\vee, c)$  &  $\OO$ \\ \hline
           $(E_8(a_3), (12))$ & $3A_1$ \\ \hline
           $(E_8(a_4), (12))$ & $4A_1$ \\ \hline
           $(E_8(a_5), (12))$ & $A_2+3A_1$\\ \hline
           $(E_8(a_6), (123))$ & $2A_2+2A_1$\\ \hline
           $(E_8(a_6), (12))$ & $A_3+2A_1$ \\ \hline
           $(E_8(b_5), (12))$ & $A_3+A_1$ \\ \hline
           $(E_8(b_5), (123))$ & $2A_2+A_1$ \\ \hline
           $(E_8(b_6), (12))$ & $A_3+A_2+A_1$\\ \hline
           $(E_6(a_1)+A_1, (12))$ & $A_3+A_2+A_1$\\ \hline
           $(D_7(a_2), (12))$ & $2A_3$\\ \hline
           $(E_8(a_7), (123)(45))$ & $A_5+A_1$ \\ \hline
           $(E_8(a_7), (12345))$ & $A_4+A_3$ \\ \hline
           $(E_8(a_7), (1234))$ & $D_5(a_1)+A_2$ \\ \hline
           $(E_8(a_7), (12)(34))$ & $D_6(a_2)$ \\ \hline
           $(E_8(a_7), (12))$ & $E_7(a_5)$ \\ \hline
           $(E_8(a_7), (123))$ & $E_6(a_3)+A_1$ \\ \hline
           $(D_4(a_1)+A_1, (123))$ & $E_8(b_6)$ \\ \hline
           
        \end{tabular}
    \end{table}
    \todo{Which pair goes to which orbit?}
    
    We refer to \cite[Propositions 3.8.3, 3.9.5]{MBMat} that every orbit $\OO=d_S(\OO^\vee, c)$ in the tables above admits birationally rigid cover.
    
    
    

{\tiny
\begin{longtable}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|}\label{table:E8Gamma}
\hline
        $\OO^{\vee}$ & $M^{\vee}$ & $\OO$ & $L$ & $\OO_L$ & $R^{\vee}$ & $\OO_{R^{\vee}}$ & $\bar{A}(\OO_{R^{\vee}})$ & $A(\OO_L)$ & $A(\OO)$ & $\Gamma$ & $\#$\\ \hline 
        
        %special distinguished Achar data (except for those of the form (Ov,1) with Ov even)
        $E_8(a_7)$ & $E_7+A_1$ & $E_7(a_5)$ & $E_8$ & $E_7(a_5)$  & $E_7+A_1$ & $E_7(a_5) \times (2)$ & $S_3$ & $S_3$ & $S_3$ & $S_3$ & $(2)$ \\\hline 
        $E_8(a_7)$ & $D_8$ & $D_6(a_2)$ & $E_8$ & $D_6(a_2)$ & $D_8$ & $(7,5,3,1)$ & $\ZZ_2$ & $S_2$ & $S_2$ & $S_2$ & $(2)$\\ \hline
        
        $E_8(a_7)$ & $E_6+A_2$ & $E_6(a_3)+A_1$ & $E_8$ & $E_6(a_3)+A_1$ & $E_6+A_2$ & $ E_6(a_3) \times (3)$ & $S_2$ & $S_2$ & $S_2$ & $S_2$ & $(2)$\\ \hline
        
        
        $E_8(a_7)$ & $D_5+A_3$ & $D_5(a_1)+A_2$ & $E_8$ & $D_5(a_1)+A_2$ & $D_5+A_3$ & $ (7,3) \times (4)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $E_8(a_7)$ & $2A_4$ & $A_4+A_3$ & $E_8$ & $2A_4$ & $2A_4$ & $(5)^2$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $E_8(a_7)$ & $A_5+A_2+A_1$ & $A_5+A_1$ & $E_8$ & $A_5+A_1$  & $A_5+A_2+A_1$ & $(6) \times (3) \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $D_7(a_2)$ & $E_7+A_1$ & $2A_3$ & $E_8$ & $2A_3$ & $D_5+A_3$ & $(7,3) \times (4)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $E_8(b_6)$ & $D_8$ & $A_3+A_2+A_1$ & $E_8$ & $A_3+A_2+A_1$  & $D_8$ & $(9,7)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $E_8(a_6)$ & $D_8$ & $A_3+2A_1$ & $E_8$ & $A_3+2A_1$  & $D_8$ & $(11,5)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $E_8(a_6)$ & $A_8$ & $2A_2+2A_1$ & $E_8$ & $2A_2+2A_1$  & $A_8$ & $(9)$ & $1$ & $1$ & $1$ & $1$ & $(1)$ \\ \hline
        
        $E_8(b_5)$ & $E_7+A_1$ & $A_3+A_1$ & $E_8$ & $A_3+A_1$ & $E_7+A_1$ & $E_7(a_2) \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $E_8(b_5)$ & $E_6+A_2$ & $2A_2+A_1$ & $E_8$ & $2A_2+A_1$ & $E_6+A_2$ & $E_6 \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $E_8(a_5)$ & $D_8$ & $A_2+3A_1$ & $E_8$ & $A_2+3A_1$ & $D_8$ & $(13,3)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $E_8(a_4)$ & $D_8$ & $4A_1$ & $E_8$ & $4A_1$ & $D_8$ & $(15,1)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $E_8(a_3)$ & $E_7+A_1$ & $3A_1$ & $E_8$ & $3A_1$ & $E_7+A_1$ & $E_7 \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        %special non-distinguished Achar data with Cbar\neq 1
        $E_6(a_1)$ & $A_7$ & $D_4+A_1$ & $E_7$ & $4A_1$ & $A_7$ & $(7,1)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $D_6(a_1)$ & $D_5+2A_1$ & $A_5$ & $D_7$ & $(3,2^2,1^7)$ & $E_7+A_1$ & $D_6(a_1)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $E_7(a_5)$ & $A_5+A_2$ & $E_6(a_3)+A_1$ & $E_7$ & $2A_2+A_1$ & $A_5+A_2$ & $(6) \times (2,1)$ & $1$ & $1$ & $S_2$ & $1$ & $(4)$ \\ \hline
        
        
        $E_7(a_5)$ & $A_1+D_6$ & $E_7(a_5)$ & $E_7$ & $(A_3+A_1)'$ & $D_8$ & & $1$ & $1$ & $S_3$ & $1$ & $(8)$ \\ \hline
        
        
        $D_6(a_2)$ & $D_4+A_3$ & $D_6(a_2)$ & $D_7$ & $(3,2^4,1^3)$ & $D_5+A_3$ & $(5^2) \times (4)$ & $1$ & $1$ & $S_2$ & $1$ & $(4)$\\ \hline
        
        
        $E_6(a_3)+A_1$ & $A_5+2A_1$ & $E_7(a_5)$ & $E_6+A_1$ & $3A_1 \times (1^2)$ & $D_8$ & ? & $1$ & $1$ & $S_3$ & $1$ & $(8)$ \\ \hline
        
        
        $E_6(a_3)$ & $A_5+A_1$ & $D_5+A_1$ & $E_6$ & $3A_1$ & $E_7+A_1$ & $(A_5)'' \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $A_4$ & $2A_3$ & $D_6$ & $D_6$ & $(3,2^4,1)$ & $D_5+A_3$ & $(5^2) \times (1^4)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
    
        $D_4(a_1)+A_2$ & $A_3+A_2+2A_1$ & $A_7$ & $D_5+A_2$ & $(3,2^2,1^3) \times (1^3)$ & $E_7+A_1$ & $(A_5)'' \times (1^2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $D_4(a_1)$ & $3A_2$ & $E_6+A_1$ & $E_6$ & $2A_2+A_1$ & $E_6+A_2$ & $2A_2 \times (3)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $D_4(a_1)$ & $A_3+2A_1$ & $E_7(a_2)$ & $D_5$ & $(3,2^2,1^3)$ & $E_7+A_1$ & $(A_3+A_1)'' \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $2A_2$ & $A_2+4A_1$ & $D_7$ & $D_4+A_2$ & $(3,2^2,1) \times (1^2)$ & $E_7+A_1$ & $2A_2 \times (1^2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $A_2$ & $4A_1$ & $E_7$ & $D_4$ & $(3,2^2,1)$ & $E_7+A_1$ & $(3A_1)'' \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$ \\ \hline
         
        %(Ov,1) with Ov not even
        $A_1$ & $A_1$ & $E_8(a_1)$ & $A_1$ & $\{0\}$ & $E_7+A_1$ & $\{0\} \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $2A_1$ & $2A_1$ & $E_8(a_2)$ & $2A_1$ & $\{0\}$ & $D_8$ & $(3,1^{13})$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$ \\ \hline
        
        
        $3A_1$ & $3A_1$ & $E_8(a_3)$ & $3A_1$ & $\{0\}$ & $E_7+A_1$ & $2A_1 \times (2)$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        $4A_1$ & $4A_1$ & $E_8(a_4)$ & $4A_1$ & $\{0\}$ & $D_8$ & $(2^8)$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        
        $A_2+A_1$ & $A_2+A_1$ & $E_8(a_4)$ & $A_2+A_1$ & $\{0\}$ & $E_7+A_1$ & $A_2 \times(2)$ & $S_2$ & $1$ & $S_2$ & $S_2$ & $(8)$\\ \hline
        
        
        $A_2+2A_1$ & $A_2+2A_1$ & $E_8(b_4)$ & $A_2+2A_1$ & $\{0\}$ & $D_8$ & $(3^3,1^7)$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        $A_3$ & $A_3$ & $E_7(a_1)$ & $A_3$ & $\{0\}$  & $D_8$ & $(5,1^{11})$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        $A_2+3A_1$ & $A_2+3A_1$ & $E_8(a_5)$ & $A_2+3A_1$ & $\{0\}$  & $E_7+A_1$ & $(A_2+2A_1) \times (2)$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        $2A_2+A_1$ & $2A_2+A_1$ & $E_8(b_5)$ & $2A_2+A_1$ & $\{0\}$  & $E_7+A_1$ & $2A_2 \times (2)$ & $1$ & $1$ & $S_3$ & $1$ & $(3)$\\ \hline
        
        $A_3+A_1$ & $A_3+A_1$ & $E_8(b_5)$ & $A_3+A_1$ & $\{0\}$  & $E_7+A_1$ & $A_3 \times (2)$ & $1$ & $1$ & $S_3$ & $1$ & $(5)$\\ \hline
        
        $2A_2+2A_1$ & $2A_2+2A_1$ & $E_8(a_6)$ & $2A_2+2A_1$ & $\{0\}$  & $D_8$ & $(3^5,1)$ & $1$ & $1$ & $S_3$ & $1$ & $(3)$ \\ \hline
        
        
        \cellcolor{blue!50}$A_3+2A_1$ & $A_3+2A_1$ & $E_8(a_6)$ & $A_3+2A_1$ & $\{0\}$  & $D_8$ & $(5,2^4,1^3)$ & $1$ & $1$ & $S_3$ & $1$ & \\ \hline
        
        \cellcolor{blue!50}$D_4(a_1)+A_1$ & $D_4+A_1$ & $E_8(a_6)$ & $D_4+A_1$ & $(2^2,1^4) \times \{0\}$ & $E_7+A_1$ & $D_4(a_1)\times (2)$ & $S_3$ & $1$ & $S_3$ & $S_3$ & \\ \hline
        
        $A_3+A_2$ & $A_3+A_2$ & $D_7(a_1)$ & $A_3+A_2$ & $\{0\}$  & $D_8$ & $(5,3^2,1^5)$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        $A_3+A_2+A_1$ & $A_3+A_2+A_1$ & $E_8(b_6)$ & $A_3+A_2+A_1$ & $\{0\}$  & $E_7+A_1$ & $(A_3+A_2) \times(2)$ & $1$ & $1$ & $S_3$ & $1$ & $(3)$ \\ \hline
        
        $D_4+A_1$ & $D_4+A_1$ & $E_6(a_1)$ & $D_4+A_1$ & $\{0\}$ & $E_7+A_1$ & $D_4 \times (2)$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        

        \cellcolor{blue!50}$A_4+A_1$ & $A_4+A_1$ & $E_6(a_1)+A_1$ & $A_4+A_1$ & $\{0\}$ & $E_7+A_1$ & $A_4 \times (2)$ & $S_2$ & $1$ & $S_2$ & $S_2$ & \\ \hline
        
        
        \cellcolor{blue!50}$2A_3$ & $2A_3$ & $D_7(a_2)$ & $2A_3$ & $\{0\}$ & $D_8$ & $(4^4)$ & $1$ & $1$ & $S_2$ & $1$ & \\ \hline
        
        $D_5(a_1)$ & $D_5$ & $E_6(a_1)$ & $D_5$ & $(2^2,1^6)$ & $D_8$ & $(7,3,1^6)$ & $\ZZ_2$ & $1$ & $S_2$ & $S_2$ & $(8)$\\ \hline
        
        
        \cellcolor{blue!50}$A_4+2A_1$ & $A_4+2A_1$ & $D_7(a_2)$ & $A_4+2A_1$ & $\{0\}$ & $D_8$ & $(5^2,3,1^3)$ & $\ZZ_2$ & $1$ & $S_2$ & $S_2$ & \\ \hline
        
        $A_5$ & $A_5$ & $D_6(a_1)$ & $A_5$ & $\{0\}$  & $E_7+A_1$ & $A_5'' \times \{0\}$ & $1$ & $1$ & $S_2$ & $1$ & $(4)$ \\ \hline
        
        \cellcolor{blue!50}$D_5(a_1)+A_1$ & $D_5+A_1$ & $E_7(a_4)$ & $D_5+A_1$ & $(2^2,1^6) \times \{0\}$ & $E_7+A_1$ & $D_5(a_1) \times (2)$ & $1$ & $1$ & $S_2$ & $1$ & \\ \hline
        
        $A_4+A_2+A_1$ & $A_4+A_2+A_1$ & $A_6+A_1$ & $A_4+A_2+A_1$ & $\{0\}$ & $E_7+A_1$ & $(A_4+A_2) \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $A_4+A_3$ & $A_4+A_3$ & $E_8(a_7)$ & $A_4+A_3$ & $\{0\}$ & $D_8$ & $(5^3,1)$ & $1$ & $1$ & $S_5$ & $1$ & $(3)$\\ \hline
        
        
        $A_5+A_1$ & $A_5+A_1$ & $E_8(a_7)$ & $A_5+A_1$ & $\{0\}$ & $D_8$ & $(6^2,2^2)$ & & $1$ & $S_5$ & & $(6)$\\ \hline
        
        
        $D_5(a_1)+A_2$ & $D_5+A_2$ & $E_8(a_7)$ & $D_5+A_2$ & $(2^2,1^6) \times \{0\}$ & $D_8$ & $(7,3^3)$ & & $1$ & $S_5$ & & $(6)$\\ \hline
        
        
        $E_6(a_3)+A_1$ & $E_6+A_1$ & $E_8(a_7)$ & $E_6+A_1$ & $A_2 \times \{0\}$ & $E_7+A_1$ & $(A_5+A_1) \times (2)$ & & $S_2$ & $S_5$ & & $(6)$\\ \hline
        
    
        $E_7(a_5)$ & $E_7$ & $E_8(a_7)$ & $E_7$ & $D_4(a_1)$ & $E_7+A_1$ & $D_6(a_2) \times (2)$ & & $S_3$ & $S_5$ & & $(6)$\\ \hline
        
        
        $D_5+A_1$ & $D_5+A_1$ & $E_6(a_3)$ & $D_5+A_1$ & $\{0\}$ & $E_7+A_1$ & $(D_5+A_1) \times \{0\}$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        

        $D_6(a_1)$ & $D_6$ & $E_6(a_3)$ & $D_6$ & $(2^2,1^8)$  & $D_8$ & $(9,3,1^4)$ & $S_2$ & $1$ & $S_2$ & $S_2$ & $(8)$\\ \hline
        
    
        $A_6+A_1$ & $A_6+A_1$ & $A_4+A_2+A_1$ & $A_4+A_2+A_1$ & $\{0\}$ & $E_7+A_1$ & $A_6 \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
    
        $E_7(a_4)$ & $E_7$ & $D_5(a_1)+A_1$ & $E_7$ & $A_2+2A_1$ & $E_7+A_1$ & $D_6(a_1) \times (2)$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $D_6$ & $D_6$ & $A_4$ & $D_6$ & $\{0\}$ & $D_8$ & $(11,1^5)$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        
        $D_7(a_2)$ & $D_7$ & $A_4+2A_1$ & $D_7$ & $(2^4,1^6)$ & $D_8$ & $(9,5,1^2)$ & $\ZZ_2$ & $1$ & $S_2$ & $S_2$ & $(8)$\\ \hline
        
        
        
        $A_7$ & $A_7$ & $D_4(a_1)+A_2$ & $A_7$ & $\{0\}$ & $D_8$ & $(8^2)$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        
        $E_6(a_1)+A_1$ & $E_6+A_1$ & $A_4+A_1$ & $E_6+A_1$ & $A_1 \times \{0\}$ & $E_7+A_1$ & $E_6(a_1) \times (2)$ & $S_2$ & $1$ & $S_2$ & $S_2$ & $(8)$\\ \hline
        
        
        $E_7(a_3)$ & $E_7$ & $A_4$ & $E_7$ & $A_2$  & $E_7+A_1$ & $D_6 \times (2)$ & $S_2$ & $1$ & $S_2$ & $S_2$ & $(8)$ \\ \hline
        
        
        $E_6+A_1$ & $E_6+A_1$ & $D_4(a_1)$ & $E_6+A_1$ & $\{0\}$  & $E_7+A_1$ & $E_6 \times (2)$ & $1$ & $1$ & $S_3$ & $1$ & $(3)$\\ \hline
        
        
        $E_7(a_2)$ & $E_7$ & $D_4(a_1)$ & $E_7$ & $2A_1$  & $E_7+A_1$ & $E_7(a_2) \times \{0\}$ & $1$ & $1$ & $S_3$ & $1$ & $(8)$ \\ \hline
        
    
        $D_7$ & $D_7$ & $2A_2$ & $D_7$ & $\{0\}$  & $D_8$ & $(13,1^3)$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        $E_7(a_1)$ & $E_7$ & $A_3$ & $E_7$ & $A_1$  & $E_7+A_1$ & $E_7(a_1) \times \{0\}$ & $1$ & $1$ & $1$ & $1$ & $(1)$\\ \hline
        
        
        $E_7$ & $E_7$ & $A_2$ & $E_7$ & $\{0\}$  & $E_7+A_1$ & $E_7 \times \{0\}$ & $1$ & $1$ & $S_2$ & $1$ & $(3)$\\ \hline
        
        \caption{Special Achar data (not of the form $(\OO^{\vee},1)$ with even $\OO^{\vee}$) in type $E_8$}
    \end{longtable}
}

    
    \begin{center}
\begin{tabular}{|c|c|c|c|c|c|} \hline
$\OO^\vee$ & $\Bar{A}(\OO^\vee)$  & $\OO$ & ${A}(\OO)$ & $L$, $\OO_L$ & ${A}(\OO_L)$  \\ \hline
$\{0\}$ & $1$& $G_2$ & $1$ & & \\ \hline
$A_1$& $1$& $G_2(a_1)$ & $S_3$ & $\widetilde{A}_1$, $\{0\}$& $1$\\ \hline
$\widetilde{A}_1$ & $1$& $G_2(a_1)$ & $S_3$ & ${A}_1$, \{0\}& $1$\\ \hline
$G_2(a_1)$ & $S_3$& $G_2(a_1)$ & $S_3$ &  & \\ \hline
$G_2$ & $1$& $\{0\}$ & $1$ && \\ \hline
\end{tabular}
\end{center}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Distinguished Sommers data}

The following is immediate from Corollary \ref{corollary: distinguished}.

\begin{prop}
Suppose $G$ is a simple group of classical type. Then the set of distinguihsed Sommers data is in bijection with a set $S$ consisting of (pairs of) partitions. 

\begin{itemize}
    \item[(i)] If $\fg=\mathfrak{sl}(n)$, then $S$ is the set of partitions of $n$ with no repeated parts. Such a partition corresponds to the Sommers datum $(\fg,\OO_p)$, where $\OO_p$ is the nilpotent orbit corresponding to $p$.
    \item[(ii)] If $\fg = \mathfrak{so}(2n+1)$, then $S$
    is the set of unordered pairs $\{p,q\}$ of $B/D$-partitions such that $|p|+|q|=n$ and both $p$ and $q$ have no repeated parts. A pair of this form corresponds to the Sommers datum $(\mathfrak{so}(2|p|) \times \mathfrak{so}(2|q|+1),\OO_p \times \OO_q)$, where $\OO_p$, $\OO_q$ are the nilpotents orbit corresponding to $p$, $q$.
    \item[(iii)] If $\fg = \mathfrak{sp}(2n)$, then $S$
    is the set of unordered pairs $\{p,q\}$ of $C$-partitions such that $|p|+|q|=n$ and both $p$ and $q$ have no repeated parts. A pair of this form corresponds to the Sommers datum $(\mathfrak{so}(2|p|) \times \mathfrak{so}(2|q|),\OO_p \times \OO_q)$, where $\OO_p$, $\OO_q$ are the nilpotents orbit corresponding to $p$, $q$.
    \item[(iv)] If $\fg = \mathfrak{so}(2n)$, then $S$
    is the set of unordered pairs $\{p,q\}$ of $B/D$-partitions such that $|p|+|q|=n$ and both $p$ and $q$ have no repeated parts. A pair of this form corresponds to the Sommers datum $(\mathfrak{so}(2|p|) \times \mathfrak{so}(2|q|),\OO_p \times \OO_q)$, where $\OO_p$, $\OO_q$ are the nilpotents orbit corresponding to $p$, $q$.
\end{itemize}
\end{prop}



Gamma computations







Suppose $\fg^{\vee}$ is of type $X \in \{B,C,D\}$ and let
%
$$\epsilon = \begin{cases*}
\phantom{-}1 & if $X \in \{B,D\}$\\
-1 & if $X=C$\end{cases*}.$$
%
Suppose $\OO^{\vee}=\OO_{\lambda}$ for $\lambda \in \mathcal{P}_X(n)$. Write $\lambda^1$ (resp. $\lambda^{-1}$) for the subpartitions consisting of all odd (resp. even) parts of $\lambda$. Note that every part of $\lambda^{-\epsilon}$ has even multiplicity. So $m = \frac{1}{2}\#\lambda^{-\epsilon}$ is an integer. Furthermore, $\lambda^{\epsilon}$ corresponds to an even orbit $\OO^{\vee}_k$ in a Lie algebra $\fg^{\vee}_k$ of type $X$. Consider the Levi subalgebra $\fl^{\vee} = \prod_{i=1}^m \mathfrak{gl}(\lambda^{\epsilon}_i) \times \fg^{\vee}_k$ of $\fg^{\vee}$ and the nilpotent orbit $\OO_{L^{\vee}} = \prod_{i=1}^m \OO_{prin} \times \OO^{\vee}_k$ (here `prin' denotes the principal nilpotent orbit). Then $\OO^{\vee} = \Sat^{G^{\vee}}_{L^{\vee}} \OO_{L^{\vee}}$, see Proposition \ref{prop:inclusionclassical}. Hence, $\OO = d(\OO^{\vee}) = \Ind^G_L \OO_L$, where $\OO_L = \prod_{i=1}^m \{0\} \times d(\OO_k)$, see Proposition \ref{prop:propsofd}(iii). We claim:


    \begin{proof}
        1) is straightforward from the definition of $K(\OO)$. Indeed, it is enough to show the statement for a Levi with one $\fg\fl$ factor. On the level of partitions saturating from $\OO^\vee_{reg}\times \OO^\vee_k\subset \fl^\vee=\fg\fl(m)\times \fg^\vee(k)$  corresponds to adding two rows of size $k$, where $k$ is even (resp. odd, even) for $\fg^\vee$ of type B (resp. C, D). Clearly, that doesn't change the number of odd (resp. even, odd) members of the partition, and the parity of their height.
        
         Let us show 2) for $\fg^\vee$ of type B, the other classical types are completely analogous. First, we need to introduce some notations. For a partition $\lambda=(\lambda_1,\ldots, \lambda_k)$ of a type C we define an \emph{even block} to be a collection of an even number of rows $(\lambda_i, \lambda_{i+1}, \ldots, \lambda_{i+2k-1})$, such that each $\lambda_j$ in even block is even, and both $\lambda_{i-1}$ and $\lambda_{i+2k}$ are either odd or $0$ (we set $\lambda_0=0$). Say, that orbit $\OO$ satisfies (*) if the corresponding partition $\alpha$ is a union of even blocks and pairs of odd rows $(2l+1, 2l+1)$. 
         
         \begin{claim}
            \begin{itemize}
                \item[1)] The orbit $\OO$ dual to an even orbit $\OO^\vee\subset \fg^\vee$ satisfies (*);
                \item[2)] If $\OO_k\subset \fg(k)$ satisfies (*), the orbit $\OO=\Ind_{GL(m)\times G(k)}^G \{0\}\times \OO_k$ satisfies (*);
                \item[3)] The induction in 2) is birational.
            \end{itemize}   
         \end{claim}
         
         Every part of the claim is an easily checkable combinatorial statement about partitions.
    \end{proof}
    
    We finish by noting that if $\OO$ is birationally induced from an orbit $\OO_L\subset \fl$, and a Galois cover $\widetilde{\OO}$ is birationally induced from a Galois cover $\widetilde{\OO}_L$ of $\OO_L$ the Galois groups of $\widetilde{\OO}\to \OO$ and $\widetilde{\OO}_L\to \OO_L$ are isomorphic. Since all $G$-equivariant covers are Galois for $G$ of adjoint type in classical types, it follows that the Galois group $\Gamma$ of $D(\OO^\vee)=\widetilde{\OO}\to \OO=d(\OO^\vee)$ is isomorphic to the Galois group $\Gamma_k$ of $D(\OO^\vee_k)=\widetilde{\OO}_k\to \OO_k=d(\OO^\vee_k)$. The latter group is isomorphic to $\bar{A}(\OO^\vee_k)$ by \cref{prop: Gamma even}, and thus to $\bar{A}(\OO^\vee)$ by \cref{lem: reduction to even}. That finishes the proof of \cref{prop: Gamma unmarked}.



       Let us show 2) for $\fg^\vee$ of type B, the other classical types are completely analogous. First, we need to introduce some notations. For a partition $\lambda=(\lambda_1,\ldots, \lambda_k)$ of a type C we define an \emph{even block} to be a collection of an even number of rows $(\lambda_i, \lambda_{i+1}, \ldots, \lambda_{i+2k-1})$, such that each $\lambda_j$ in even block is even, and both $\lambda_{i-1}$ and $\lambda_{i+2k}$ are either odd or $0$ (we set $\lambda_0=0$). Say, that orbit $\OO$ satisfies (*) if the corresponding partition $\alpha$ is a union of even blocks and pairs of odd rows $(2l+1, 2l+1)$. 
         
         \begin{claim}
            \begin{itemize}
                \item[1)] The orbit $\OO$ dual to an even orbit $\OO^\vee\subset \fg^\vee$ satisfies (*);
                \item[2)] If $\OO_k\subset \fg(k)$ satisfies (*), the orbit $\OO=\Ind_{GL(m)\times G(k)}^G \{0\}\times \OO_k$ satisfies (*);
                \item[3)] The induction in 2) is birational.
            \end{itemize}   
         \end{claim}
         
         Every part of the claim is an easily checkable combinatorial statement about partitions.
    \end{proof}



\begin{lemma}\label{lem:Gammadistinguishedbasic}
Suppose $G$ is a simple adjoint group of type $B$, $C$, or $D$ and let $(\OO^{\vee},\bar{C}) \in \LA^*(G^{\vee})$. Assume that $(\OO^{\vee},\bar{C})$ corresponds to a distinguished basic block or a distinguished unmarked partition. Then there is a group isomorphism
%
$$\bar{A}(\OO_{R^{\vee}}) \simeq A(d_S(\OO^{\vee},\bar{C})).$$
\end{lemma}

\begin{proof}
If $\nu=\emptyset$, then the statement follows from Lemma \ref{lem:Gammaunmarked}. So we can assume that $\nu \neq \emptyset$. Let $X \in \{B,C,D\}$ be the Lie type of $G^{\vee}$ and let $\pi$ be the partition corresponding to the dual orbit $\OO=d_S(\OO^{\vee},\bar{C})$. Recall that $\pi$ was computed in Section \ref{sec:basic block}.
\begin{itemize}
    \item If $X=B$, then $\lambda=[2k_1-1, 2k_2-1, \ldots, 2k_{2m+1}-1]$ with $k_1> k_2>\ldots>k_{2m}\ge k_{2m+1}>0$ and $\nu=[2k_1-1, 2k_{2m+1}-1]$. By the description of $\pi$ in Lemma \ref{lem:dualtobasicblock} and Proposition \ref{prop:Aclassical}, $A(\OO) \simeq (\ZZ_2)^{m-1}$. 
    
    On the other hand, to compute the pair $(R^\vee, \OO_{R^{\vee}})$ from the McNinch-Sommers datum $\mathbb{L}(\OO^{\vee},\bar{C})$ we need to find the pair $(\nu_0, \eta_0)$ attached to the pair $\OO^\vee, \Bar{C}$ in \cref{sec: Sommers}. We have $\Bar{C}=\prod_{i=1}^{m} \bar{\theta}_i$, and thus $\widetilde{s}(\bar{C})=\prod_{i=1}^{2m} \upsilon_{\lambda_i} = \prod_{i=1}^{2m} \upsilon_{2k_i-1}$. Therefore, $\nu_0=[2k_1-1, \ldots,  2k_{2m}-1]$, and $\eta_0=[2k_{2m+1}-1]$. \cref{thm:inflchars} and \cref{lem:gamma_0} imply that $R^\vee \simeq SO(\sum_{i=1}^{2m} (2k_i-1))\times SO(2k_{2m+1}-1)$, and $\OO_{R^{\vee}} = \OO_{[2k_1-1, \ldots,  2k_{2m}-1]} \times \OO_{[2k_{2m+1}-1]}$, so $\bar{A}(\OO_{R^{\vee}}) \simeq (\ZZ_2)^{m-1}$ by Corollary \ref{cor:Abarclassical}.
    

    \item If $X=C$, then $\lambda=[2k_1, 2k_2, \ldots, 2k_{2m}]$ with $k_1\ge  k_2>\ldots>k_{m-1}\ge k_{2m}\ge 0$ and $\nu=[2k_2, 2k_{2m}]$ or $\nu=[2k_2]$. In the former case, $A(\OO) \simeq (\ZZ_2)^m$ (Lemma \ref{lem:dualtobasicblock} and Proposition \ref{prop:Aclassical}). A similar computation to the above shows that $R^\vee \simeq Sp(\sum_{i=2}^{2m-1} 2k_i)\times Sp(2k_1+2k_m)$, and $\OO_{R^{\vee}} = \OO_{[2k_2, \ldots, 2k_{2m-1}]} \times \OO_{[2k_1, 2k_{2m}]}$. Therefore, $\bar{A}(\OO_{R^{\vee}}) \simeq \ZZ_2 \times (\ZZ_2)^{m-1} \simeq (\ZZ_2)^m$ (Corollary \ref{cor:Abarclassical}). In the latter case, $A(\OO) \simeq (\ZZ_2)^{m-1}$ (Lemma \ref{lem:dualtobasicblock} and Proposition \ref{prop:Aclassical}), $R^\vee \simeq Sp(\sum_{i=2}^{2m-1} 2k_i)\times Sp(2k_1)$, $\OO_{R^{\vee}} = \OO_{[2k_2, 2k_3 \ldots, 2k_{2m}]} \times \OO_{[2k_1]}$, and $\bar{A}(\OO_{R^{\vee}}) \simeq (\ZZ_2)^{m-1}$ (Corollary \ref{cor:Abarclassical}). We note that for this computation it is not important whether $k_{2m}=0$. 
    
    \item If $X=D$, then $\lambda=[2k_1-1, 2k_2-1, \ldots, 2k_{2m}-1]$ with $k_1\ge k_2>\ldots>k_{2m-1}\ge k_{2m}>0$ and $\nu=[2k_2-1, 2k_{2m}-1]$. In this case, $A(\OO) \simeq (\ZZ_2)^{m-2}$  (Lemma \ref{lem:dualtobasicblock} and Proposition \ref{prop:Aclassical}). On the other hand, a similar computation to the type B case, shows that $R^\vee\simeq SO(\sum_{i=2}^{2m-1} (2k_i-1))\times SO(2k_1+2k_{2m}-2)$, and $\OO_{R^{\vee}} = \OO_{[2k_2-1, \ldots, 2k_{2m-1}-1]} \times \OO_{[2k_1-1, 2k_{2m}-1]}$. So  $\bar{A}(\OO_{R^\vee})\simeq (\ZZ_2)^{m-2}$ (Corollary \ref{cor:Abarclassical}).
\end{itemize}

    
\end{proof}

Applying \cref{R0toR} \footnote{Why can we apply this remark? $\underline{\mathfrak{r}}^{\vee}$ is only a pseudo-Levi subalgebra, not Levi. Is this remark used anywhere else? Mitya: Fixed the remark, it was supposed to be about pseudo-Levi from the beginning.}


\begin{rmk}\label{R0toR}
Suppose that $L^\vee\subset G^\vee$ is standard Levi, and $R_0^\vee \subset L^\vee$ is standard pseudo-Levi subgroup. Let $I_0$ be the set of simple roots of $\fl^\vee$ which are not in $\fr_0^\vee$ and let $I$ be the set of simple roots of $\fg^{\vee}$ which are not in $I_0$. Then $R^{\vee} \subset G^{\vee}$ is the standard pseudo-Levi subgroup corresponding to $I$.
\end{rmk}


    
Now \cref{thm:Gamma} follows from the following lemma.

\begin{lemma}\label{lem:Gammaclassical}
Suppose $G$ is a simple adjoint group of type $B$, $C$, or $D$, and let $(\OO^{\vee},\bar{C}) \in \LA^*(G^{\vee})$. Then there is a group isomorphism
%
$$\bar{A}(\OO_{R^{\vee}}) \simeq \Gamma(D(\OO^{\vee},\bar{C})).$$
\end{lemma}

\begin{proof}
In view of Lemma \ref{lem:Gammaclassicaldistinguished}, we can assume that $(\OO^{\vee},\bar{C})$ is not distinguished. So suppose that 
%
$$(\OO^\vee, \bar{C}) = \Sat^{G^{\vee}}_{M^{\vee}} (\OO_{M^{\vee}},\bar{C}_{M^{\vee}})$$
%
for a maximal Levi subalgebra $\fm^{\vee}= \mathfrak{gl}(a)\times \fg^\vee(m)\subset \fg^\vee$. We can always assume that $\OO_{M^{\vee}} = \OO_{prin} \times \underline{\OO}^{\vee}$. Let $\underline{\bar{C}}\in \bar{A}(\underline{\OO}^{\vee})\simeq \bar{A}(\OO_{M^{\vee}})$ be the element corresponding to $\bar{C}_{M^{\vee}}\in \bar{A}(\OO_{M^{\vee}})$. Let $^{\langle \nu\rangle} \underline{\lambda}$ be the reduced marked partition corresponding to the pair $(\underline{\OO}^\vee, \underline{\bar{C}})$. We note that $\lambda=\underline{\lambda}\cup [a,a]$. Let $^{\langle \nu\rangle} \underline{\lambda}=^{\langle \underline{\nu}^1\rangle} \underline{\lambda}^1\cup ^{\langle \underline{\nu}^2\rangle} \underline{\lambda}^2\cup \ldots \cup ^{\langle \underline{\nu}^k\rangle} \underline{\lambda}^k$ be a decomposition into basic blocks. There is at most one block $^{\langle \underline{\nu}^l\rangle} \underline{\lambda}^l$, such that $\underline{\lambda}^{l}_1\ge a\ge \underline{\lambda}^{l}_{|\underline{\lambda}^l|}$. If there is no such block, we formally add an empty unmarked basic block $^{\langle \underline{\nu}^l\rangle} \underline{\lambda}^l=^{\langle \emptyset\rangle} \emptyset$ and renumber the remaining $^{\langle \underline{\nu}^i\rangle} \underline{\lambda}^i$'s, so that $\underline{\lambda}^{l-1}_{|\underline{\lambda}^{l-1}|}>a>\underline{\lambda}^{l+1}_{1}$. 
        
Let $\lambda^i=\underline{\lambda}^i$ if $i\neq l$, and $\lambda^l=\underline{\lambda}^l\cup [a,a]$. For all $i$ we set $\nu^i=\underline{\nu}^i$. Then $^{\langle \nu \rangle} \lambda=^{\langle \nu^1\rangle} \lambda^1\cup ^{\langle \nu^2\rangle} \lambda^2\cup \ldots \cup ^{\langle \nu^k\rangle} \lambda^k$ is a decomposition into basic blocks.
%\footnote{Is this true? Suppose $\fg^\vee$ is of type $B$. If $\nu^t=\emptyset$, and the height of $a$ in $\lambda^t$ is odd, then $\lambda^t$ may further split into smaller basic blocks. Mitya: I don't understand this comment. A basic unmarked block can be split into smaller basic blocks, there is no problem with that. I never claimed or used the uniqueness of the decomposition into smaller blocks, or any kind of minimality of smaller blocks.}
        
%Let $(L^\vee, ??, \OO^\vee_{L^\vee})$ and $(\underline{L}^{\vee}, ??, \underline{\OO}^{\vee}_{\underline{L}^{\vee}})$ be the corresponding McNinch-Sommers data.
        
Let $\underline{\OO}=d_S(\underline{\OO}^\vee, \underline{\bar{C}})$. Assume first that $\underline{\OO}$ is very even in type $D$. Then $\underline{\OO}$ is special, and therefore $\underline{\bar{C}}=1$. Thus, $\bar{C}=1$, and the claim follows from \cref{lem:Gammaunmarked}. Therefore, we can assume that $\underline{\OO}$ is not very even. Then the orbit $\OO$ is birationally induced from $\{0\}\times \underline{\OO}$ if and only if there is no collapse on the level of partitions. \cref{block division of dual} implies that $\OO=d_S(\OO^\vee, \bar{C})$ is birationally induced from $\{0\}\times \underline{\OO}=\{0\}\times d_S(\underline{\OO}^\vee, \underline{\bar{C}})$ if and only if $d_S(^{\langle \nu^l\rangle} \lambda^l)$ is birationally induced from $\{0\}\times d_S(^{\langle \underline{\nu}^l\rangle} \underline{\lambda}^l)$. By the results of \cref{lem: Abar distinguished basic} and \cref{cor:Abarclassical} \footnote{I don't understand. In \cref{lem: Abar distinguished basic} it is proven that the induction is always birational and $\bar{A}$ does not change. Also you want to also address \cref{sec:proofsclassical3} for $\underline{\nu}^l = \emptyset$. But there it also says that induction is always birational. I am confused... Mitya: I fixed the argument for $\eta=\emptyset$. Now it is written separately, the earlier argument considered only marked basic blocks. For \cref{sec:proofsclassical3} as we discussed, the argument for birational is correct because we start with a partition that has all odd members} this induction is not birational if and only if all of the following conditions hold.
    \begin{itemize}
        \item $a$ is not a member of $\underline{\lambda}^l$, equivalently of $\underline{\lambda}$;
        \item $a$ is odd (resp. even, odd) if $\fg^\vee$ is of type $B$ (resp. $C$, $D$);
        %, equivalently in $\lambda^l$ or in $\lambda$\todo{Why equivalently in $\lambda$?}, 
        is odd (resp. even, even) if $^{\langle \underline{\nu}^l\rangle} \underline{\lambda}^l$ is a basic block of type $B$ (resp. $C$, $D$).
    \end{itemize}
\footnote{Not quite correct. Assume $a$ is not a member of $\underline{\lambda}$. Then when $a$ is odd, the induction is not birational if and only if $a$ has odd (generalized) height in $\eta_0$. When $a$ is even, the induction is not birational if and only if $a$ has odd (generalized) height in $\nu_0$. Note that this is equivalent to that $a$ has odd height in both $\lambda$ and $\nu$. But this is exactly the definition of non-special marked partition.  }

    
%\footnote{One issue with the claim: the parity of $a$ is not mentioned. Suppose $\fg^\vee$ is of type $B$. Assume $a$ is not a member of $\underline{\lambda}$. For odd $a$, the induction is not birational when adding the double rows $(a,a)$ iff $\mathrm{ht}_\lambda(a)$ is odd and $\mathrm{ht}_\nu(a)$ is even (equivalent to $\nu^t=\emptyset$?). These are exactly the conditions above in the text. So the discussions below are fine. For even $a$, the induction is not birational iff $\mathrm{ht}_\lambda(a)$ is odd and $\mathrm{ht}_\nu(a)$ is odd. In this case, $\bar{A}(\OO^{\vee}_2)\simeq \bar{A}(\underline{\OO}^{\vee}_2)$ but $\Gamma$ increases by a $\ZZ_2$-factor. Therefore $\bar{A}$ and $\Gamma$ won't match. This case is exactly ruled out by the assumption that $(\OO^\vee, \bar{C})$ is special. So the claim in the text is not true when $a$ is even.\\
%I suggest state this claim as an independent lemma, which might be useful for future purpose. Also it is already used in the proof of \cref{lem: Abar distinguished basic}. \\
%Mitya: Fixed an issue about the parity, added that it must be odd (even, odd). As for the independent lemma, I don't think we use it anywhere. This claim uses the already proven \cref{lem: Abar distinguished basic}, and this condition comes from studying when $\bar{A}$ changes.}
        
Let $(L^\vee, tZ(L^{\vee})^{\circ}, \OO^\vee_{L^\vee})=\mathbb{L}(\OO^\vee, \Bar{C})\in \MS(G^\vee)$ and $(\underline{L}^{\vee}, \underline{t}Z(\underline{L}^{\vee})^{\circ}, \underline{\OO}^{\vee}_{\underline{L}^{\vee}})=\mathbb{L}(\underline{\OO}^\vee, \Bar{\underline{C}})\in \MS(G^\vee(m))$ be the McNinch-Sommers data constructed in \eqref{eq:defofL}. Recall that $\underline{L}^{\vee}=\underline{L}^{\vee}_1\times \underline{L}^{\vee}_2$ is a product of two simple factors, and 
Recall from \cref{defn:C0} the partitions $\underline{\nu}_0$ and $\underline{\eta}_0$ attached to the distinguished pair $(\underline{\OO}^\vee, \Bar{\underline{C}})$. 

, and let $\underline{\eta_0}$ and $\underline{}$ be 
$\underline{\OO}^{\vee}_{\underline{L}^{\vee}}=\underline{\OO}^{\vee}_1\times \underline{\OO}^{\vee}_2$, the explicit description for the distinguished LA datum $(\OO^\vee, \Bar{C})$ is provided in \todo{add reference to Shilin. Shilin: The following `alternative description' is exactly what was in my mind.}. In what follows we assume that $\fg^\vee$ is of type $B$, the other types are completely analogous. We will use the following alternative description of $(\nu_0, \eta_0)$. For each basic block $^{\langle \nu^i\rangle} \lambda^i$ let $\eta_0^i$ be the union of the second marked row and all rows before the first marked row. That is, if $\nu^i= \emptyset$ then $\eta_0^i=\lambda^i$, and $\eta_0^i$ consists of $1$ (in type $B$) or $2$ (in types $C$ and $D$) rows otherwise\footnote{The second part is not true. Also you already assume $\fg^\vee$ is of type $B$, why are there blocks of type $C$?}. Let $\nu^i_0=\lambda^i-\eta_0^i$. Then $\eta_0=\bigcup \eta_0^i$, and $\nu_0=\bigcup \nu^i_0$. In particular, we note that each distinguished\todo{Why distinguished?} basic block contribute to an even number of rows in $\nu_0$, and only the first (type $B$) basic block contributes an odd number of rows to $\eta_0$. It is clear that this property is preserved by saturation, and \todo{And what?}. Thus, if we use only this property, we can analyze $\Bar{A}(\OO_{R^\vee})$ considering only saturation from a maximal Levi $L=GL(a)\times SO(2n-2a+1)$. If $a$ is even, then $\Bar{A}$ does not change, so we can assume $a$ is odd. Arguing as above, there is a unique basic block $^{\langle \nu^l\rangle} \lambda^l$ in which $a$ lands. We adopt the same notations. If $a$ is a member of $\underline{\lambda}^l$, then $\Bar{A}$ does not change. Then $\Bar{A}$ is increased by $\ZZ/2\ZZ$ factor if and only if $a$ is odd\footnote{When the parity of $a$ is fixed, then only one of the two cases below can happen. If $a$ is odd, $a \in \eta_0$. If $a$ is even, then $a \in \nu_0$. Now $\nu_0$ is of type D, so adding even $a$ doesn't change $\bar{A}$.}, $a\notin \underline{\lambda}$, and one of the following holds.
\begin{itemize}
    \item[(i)] $a\in \eta_0$, and $a$ is of odd height in $\eta_0$;
    \item[(ii)] $a\in \nu_0$, and $a$ is of even height in $\nu_0$. 
\end{itemize}
    If $\nu^l=\varnothing$, then $a\in \eta_0$, and by the discussion above $a$ is of odd height in $\eta_0$ if and only if $a$ is of odd (resp. even) height in $\lambda^l$, where $^{\langle \nu^l\rangle} \lambda^l$ is a basic block of type $B$ (resp. $C$\todo{Typo? Type $D$?}). If $\nu^l\neq \emptyset$,  $a\in \nu_0$. Note that $a$ is of odd\todo{Contradict with (ii).} height in $\nu_0$ if and only if $a$ is of odd (resp. even) height in $\lambda^l$, where $^{\langle \nu^l\rangle} \lambda^l$ is a basic block of type $B$ (resp. $C$\todo{Typo? Type $D$?}). Thus, these conditions are equivalent to the conditions above.

   %\textcolor{red}{then case (i) cannot happen by Definition \ref{defn:block} of basic blocks, the definition of $\eta_0^l$ and that $a \notin \underline{\nu}^l=\nu^l$. Therefore we are in case (ii) and}
    
    When the conditions are satisfied, we have $\bar{A}(\OO^{\vee}_2)\simeq \bar{A}(\underline{\OO}^{\vee}_2)\times \ZZ_2$, and the generalized Springer map associated to the induction from $\underline{\OO}$ to $\OO$ is generically $2$ to $1$. It implies that \cref{thm:Gamma} in classical types can be deduced from the analogous statement for distinguished pairs $(\OO^\vee, \bar{C})$, which was proved in \cref{lem:Gammaclassicaldistinguished}.
\end{proof}


        \begin{enumerate}
    \item[(i)] If $G=SO(2n+1)$ or $G=SO(2n)$, then
      \[ \gamma(\widetilde{\OO}) = \rho^+(g(y) \cup f_0(x)). \]
    \item[(ii)] If $G=Sp(2n)$, then
      \[ \gamma(\widetilde{\OO}) = \rho^+(g(y) \cup f_1(x)). \]
\end{enumerate}

==> earlier_version.tex <==

\section{Introduction}

Let $G$ be a complex reductive algebraic group with Lie algebra $\fg$. A \emph{nilpotent cover} is a finite connected $G$-equivariant cover of a nilpotent co-adjoint orbit $\OO \subset \fg^*$. Write $\Cov(G)$ for the (finite) set of isomorphism classes of nilpotent covers for $G$. In \cite{LMBM}, we attach to each nilpotent cover $\widetilde{\OO}$ a finite set $\mathrm{Unip}_{\widetilde{\OO}}(G)$ of irreducible unitary representations of $G$ called \emph{unipotent representations}. Such representations possess a variety of special properties and are conjectured to form the building blocks of the unitary dual. They include, as a proper subset, all special unipotent representations in the sense of Arthur (\cite{Arthur1983}) and Barbasch-Vogan (\cite{BarbaschVogan1985}).The purpose of this article is to give a description of the sets $\mathrm{Unip}_{\widetilde{\OO}}(G)$ in terms of the Langlands dual group $G^{\vee}$. 

Our description involves several types of parameters related to $G^{\vee}$, which we will now briefly describe:
\begin{itemize}
    \item An \emph{Achar datum} for $G^{\vee}$ is a pair $(\OO^{\vee},\bar{C})$ consisting of a nilpotent orbit $\OO^{\vee} \subset \fg^{\vee}$ and a conjugacy class $\bar{C}$ in Lusztig's canonical quotient $\bar{A}(\OO^{\vee})$ of the $G^{\vee}$-equivariant fundamental group of $\OO^{\vee}$, see \ref{subsec:Abar}. Write $\Ach(G^{\vee})$ for the (finite) set of Achar data for $G^{\vee}$.\todo{define special Achar data}
    \item A \emph{Sommers datum} for $G^{\vee}$ is a pair $(L^{\vee},\OO_{L^{\vee}})$ consisting of a pseudolevi subgroup $L^{\vee} \subset G^{\vee}$ (i.e. the centralizer in $G^{\vee}$ of a semisimple element) and a nilpotent orbit $\OO_{L^{\vee}} \subset \fl^{\vee}$. Write $\Som(G^{\vee})$ for the (finite) set of $G^{\vee}$-conjugacy classes of Sommers data for $G^{\vee}$.
\end{itemize}
Choose a Cartan subalgebra $\fh \subset \fg$ and let $W$ denote the Weyl group. We define in Section \ref{subsec:Achar} natural surjective maps
%
$$\fh^*/W \twoheadrightarrow \Som(G^{\vee}) \twoheadrightarrow \Ach(G^{\vee})$$
%
For each $(\OO^{\vee},\bar{C}) \in \Ach(G^{\vee})$, we show in Theorem \ref{thm:inflchars} that there is a unique minimal-length element element $\gamma(\OO^{\vee},\bar{C}) \in \fh^*/W$ which maps to $(\OO^{\vee},\bar{C})$ under the pair of maps above. This element determines an infinitesimal character for $U(\fg)$ by the Harish-Chandra isomorphism, and hence a maximal ideal $I(\OO^{\vee},\bar{C})$ in $U(\fg)$. We define
%
\begin{align*}
\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G) = \{&\text{irreducible $G$-equivariant Harish-Chandra $U(\fg)$-bimodules}\\
&\text{which are annihilated on both sides by} I(
\OO^{\vee},\bar{C})\}.\end{align*}
%
The notation suggests a relationship between $\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G)$ and $\mathrm{Unip}_{\widetilde{\OO}}(G)$. To make this relationship precise, we define in Section \ref{sec:mainresults} a natural duality map
%
$$D: \Ach^*(G^{\vee}) \to \Cov(G)$$
%
This map generalizes several well-known duality maps, including those of Barbasch-Vogan-Lusztig-Spaltenstein (\cite{BarbaschVogan1985}), Sommers (\cite{Sommers2001}), Achar (\cite{Achar2003}) and Mason-Brown-Matvieievskyi-Losev (\cite{LMBM}). It enjoys various nice properties. For example, it is injective and intertwines saturation of Achar data with induction of nilpotent covers. Our first main result is the following.

\begin{theorem}[See Theorem \ref{thm:inflchars} below]\label{theorem:main1intro}
Let $(\OO^{\vee},\bar{C}) \in \Ach^*(G^{\vee})$ and let $\widetilde{\OO} = D(\OO^{\vee},\bar{C})$. Then there is an equality
%
$$\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G) = \mathrm{Unip}_{\widetilde{\OO}}(G).$$
\end{theorem}

We define in Section \ref{sec:mainresults} a natural injective map
%
$$\mathbb{L}: \Ach^*(G^{\vee}) \hookrightarrow \Som(G^{\vee})$$
%
which is right-inverse to the projection $\Som(G^{\vee}) \to \Ach(G^{\vee})$. Our second main result gives a parameterization of $\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G)$ in terms of the Langlands dual group. 

\begin{theorem}[See Corollary \ref{cor:HC} below]\label{theorem:main2intro}
Assume $G$ is adjoint. Let $(\OO^{\vee},\bar{C}) \in \Ach^*(G^{\vee})$ and let $(R^{\vee},\OO_{R^{\vee}}) = \mathbb{L}(\OO^{\vee},\bar{C})$. Then there is a natural bijection
%
$$\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G) \simeq \{\text{irreducible representations of } \bar{A}(\OO_{R^{\vee}})\}.$$
\end{theorem}
%
\begin{rmk}
In fact, the representations in $\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G)$ are the irreducible objects in a monoidal category $\HC^G(U(\fg)/I(\OO^{\vee},\bar{C}))$, defined in terms of the ideal $I(\OO^{\vee},\bar{C})$. The bijection in Theorem \ref{theorem:main2intro} comes from a monoidal equivalence of categories
%
$$\HC^G(U(\fg)/I(\OO^{\vee},\bar{C})) \simeq \bar{A}(\OO_{R^{\vee}})\modd$$
\end{rmk}

Now fix a nilpotent orbit $\OO^{\vee} \subset \fg^{\vee}$. Choose an $\mathfrak{sl}(2)$-triple $(e^{\vee},f^{\vee},h^{\vee})$ with $e^{\vee} \in \OO^{\vee}$. The corresponding map $\psi_{\OO^{\vee}}: SL(2) \to G^{\vee}$ is a unipotent Arthur parameter for the complex group $G$ and the corresponding Arthur packet coincides with the set $\mathrm{Unip}_{(\OO^{\vee},1)}(G)$. So in fact Theorem \ref{theorem:main2intro} provides, as a special case, a parameterization of the elements of a unipotent Arthur packet for a complex reductive group (such a parameterization was previously obtained in \cite{BarbaschVogan1985} only in the special case when $\OO^{\vee}$ is even). 


\subsection{Acknowledgments}

\tableofcontents

\section{Preliminaries}

Let $G$ be a complex connected reductive algebraic group. A \emph{nilpotent orbit} for $G$ is a co-adjoint orbit $\OO \subset \fg^*$ which is stable under scaling. Let
%
$$\Orb(G) := \{\text{nilpotent orbits $\OO \subset \fg^*$}\}$$
%
It is well-known that $\Orb(G)$ is finite. For each $\OO \in \mathsf{Orb}(G)$, choose an element $e \in \OO$, and let $A(\OO)$ denote the (finite) component group of the centralizer of $e$ in $G$. Note that $A(\OO)$ is independent (up to conjugacy) of the choice of $e$ in $\OO$. 

A \emph{conjugacy datum} for $G$ is a pair $(\OO,C)$ consisting of a nilpotent orbit $\OO \in \mathsf{Orb}(G)$ and a conjugacy class $C$ in $A(\OO)$. Let
%
$$\Conj(G) := \{\text{conjugacy data $(\OO,C)$ for $G$}\}$$
%
A \emph{pseudolevi subgroup} of $G$ is the identity component of the centralizer of a semisimple element $s \in G$. A \emph{Sommers datum} for $G$ is a pair $(M,\OO_M)$ consisting of a pseudolevi subgroup $M \subset G$ and a nilpotent orbit $\OO_M \in \Orb(M)$. Note that $G$ acts by conjugation on the set of Sommers data. Let
%
$$\Som(G) := \{\text{Sommers data $(M,\OO_M)$ for $G$}\}/G.$$

\subsection{Saturation}

Suppose $L \subset G$ is a Levi subgroup. If $\OO_L \in \Orb(L)$, then $G\cdot \OO_L \in \Orb(G)$. This defines a map
%
\begin{equation}\label{eq:satorb}\mathrm{Sat}^G_L: \Orb(L) \to \Orb(G), \qquad \mathrm{Sat}^G_L\OO_L = G \cdot \OO_L.\end{equation}
%
Now choose $e \in \OO_L$. The inclusion $Z_L(e) \subset Z_G(e)$ induces a group homomorphism
%
\begin{equation}\label{eq:iota}\iota: A(\OO_L) \to A(\mathrm{Sat}^G_L\OO_L).\end{equation}
%
Thus we get a map
%
\begin{equation}\label{eq:satconj}\mathrm{Sat}^G_L: \Conj(L) \to \Conj(G), \qquad \mathrm{Sat}^G_L(\OO_L,C_L) = (\mathrm{Sat}^G_L\OO_L, \iota(C_L)).\end{equation}
%
Finally, a pseudolevi subgroup of $L$ is a pseudolevi subgroup of $G$. So there is a tautological map
%
$$\Sat^G_L: \Som(L) \to \Som(G)$$
%
A nilpotent orbit (resp. conjugacy datum, resp. Sommers datum) is \emph{distinguished} if cannot be obtained by saturation from a proper Levi subgroup. Note that a Sommers datum $(M,\OO_M) \in \Som(G)$ is distinguished if and only if $M$ is not contained in a proper Levi subgroup of $G$.

\subsection{Maps $\alpha$ and $\beta$}\label{subsec:alphabeta}

Following \cite{Sommers1998}, we will define maps $\alpha$ and $\beta$ between $\Som(G)$ and $\Conj(G)$. First, we will define a map $\alpha:\Conj(G) \to \Som(G)$. Let $(\OO,C) \in \Conj(G)$. Choose $e \in \OO$ and a semisimple element $s \in Z_G(e)$ which maps to $C$ under the natural map $Z_G(e) \twoheadrightarrow A(\OO)$. Let $S$ be a maximal torus in $Z_G(e,s)$ and let $M = Z_G(S,s)^{\circ}$. By the discussion in \cite[Section 3.2]{Sommers1998}, $M \subset G$ is a pseudolevi subgroup, well-defined up to conjugacy. Let $\OO_M = M \cdot e \in \Orb(M)$. Then we get a well-defined map
%
\begin{equation}\label{eq:alpha}\alpha: \Conj(G) \to \Som(G), \qquad \alpha(\OO,C) = (M,\OO_M).\end{equation}
%
We say that $(M, \OO_M)$ is \emph{large} if $\OO_M$ is distinguished. Write $\Som_{large}(G)$ for the set of large Sommers data.

The following can be deduced from \cite[Proposition 12]{Sommers1998}.

\begin{prop}\label{prop:imageSommers}
The image of the map $\alpha: \Conj(G) \to \Som(G)$ is contained in $\Som_{large}(G)$.
\end{prop}

If $Z(G)$ is connected, we can define a map in the opposite direction. Let $(M,\OO_M) \in \Som(G)$. By \cite[Remark 3]{Sommers1998}, the component group of $Z(M)$ is cyclic. Choose an element $x \in Z(M)$ which maps to a generator of this cyclic group and choose $e \in \OO_M$. Let $\OO = G\cdot e$. Since $x$ is contained in $Z(M)$, it centralizes $e$ and hence determines a conjugacy class $C$ in $A(\OO)$. By \cite[Proposition 8]{Sommers1998}, the pair $(\OO,C) \in \Conj(G)$ is well-defined (i.e. independent of the choices of $x$ and $e$). Thus, we get a map
%
$$\beta: \Som(G) \to \Conj(G), \qquad \beta(M,\OO_M) = (\OO,C)$$
%
\begin{lemma}\label{lem:alphabeta}
Suppose $Z(G)$ is connected. Then the following are true
\begin{itemize}
    \item[(i)] For any $(\OO,C) \in \Conj(G)$
    %
    $$\beta(\alpha(\OO,C)) = (\OO,C)$$
    \item[(ii)] For any $(M,\OO_M) \in \Som_{large}(G)$
    %
    $$\alpha(\beta(M,\OO_M)) = (M,\OO_M)$$
\end{itemize}
\end{lemma}

\begin{proof}
Let $(\OO,C) \in \Conj(G)$. Choose $e \in \OO$, $s \in Z_G(e)$, and $S \subset Z_G(e,s)$ as in the paragraph preceding Proposition \ref{prop:imageSommers}. Let $M=Z_G(S,s)^{\circ}$. Note that $s \in Z(M)$. For (i), it suffices to show that $s$ maps to a generator of $Z(M)/Z(M)^{\circ}$. This follows from \cite[Remark 3]{Sommers1998}. (ii) is a consequence of \cite[Propositions 11, 12]{Sommers1998}.
\end{proof}

\begin{rmk}
If $Z(G)$ is connected then Lemma \ref{lem:alphabeta} implies that $\alpha$ and $\beta$ define inverse bijections between $\Conj(G)$ and $\Som_{large}(G)$. This is the content of \cite[Theorem 13]{Sommers1998}.
\end{rmk}


\begin{prop}\label{prop:twodiagrams}
Suppose $Z(G)$ is connected and let $L \subset G$ be a Levi subgroup. Then $Z(L)$ is connected and the following diagrams commute

\begin{center}
    \begin{tikzcd}
    \Som(L) \ar[d,twoheadrightarrow,"\beta^L"] \ar[r,"\mathrm{Sat}^G_L"] & \Som(G) \ar[d,twoheadrightarrow,"\beta^G"]\\
    \Conj(L) \ar[r,"\mathrm{Sat}^G_L"]& \Conj(G)
    \end{tikzcd}
    \begin{tikzcd}
    \Conj(L) \ar[d,hookrightarrow,"\alpha^L"] \ar[r,"\mathrm{Sat}^G_L"] & \Conj(G) \ar[d,hookrightarrow,"\alpha^G"]\\
    \Som(L) \ar[r,"\mathrm{Sat}^G_L"]& \Som(G)
    \end{tikzcd}
\end{center}

\end{prop}

\begin{proof}
The connectedness of $Z(L)$ is standard, see e.g. \cite[Lemma 9]{NairPrasad} for a proof. The commutativity of the first diagram is immediate from the definitions of $\beta$ and $\Sat^G_L$. For the second diagram, we argue as follows. Let $(\OO_L,C_L) \in \Conj(L)$. Let $(\OO,C) = \Sat^G_L (\OO_L,C_L)$ and $(M,\OO_M) = \alpha(\OO_L,C_L)$. We wish to show that $(M,\OO_M) = \alpha^G(\OO,C)$. By the commutativity of the first diagram, we have
%
$$\Sat^G_L \beta^L(M,\OO_M)) = \beta^G(M,\OO_M)$$
%
Hence by (i) of Lemma \ref{lem:alphabeta}
%
$$\Sat^G_L(\OO_L,C_L) = \beta^G(M,\OO_M)$$
%
By Proposition \ref{prop:imageSommers}, $\OO_M$ is distinguished. So by (ii) of Lemma \ref{lem:alphabeta}, we have
%
$$(M,\OO_M) = \alpha^G(\OO,C)$$
%
as desired.
\end{proof}



\subsection{Bala-Carter theorems}

Write 
%
\begin{align*}
    \Orb_0(G) &:= \{(L,\OO_L) \mid \OO_L \text{ distinguished}\}/G\\
    \Conj_0(G) &:= \{(L,(\OO_L,C_L)) \mid (\OO_L,C_L) \text{ distinguished}\}/G\\
    \Som_0(G) &:= \{(L,(M,\OO_M)) \mid (M,\OO_M) \text{ distinguished}\}/G 
\end{align*} 
\todo{$M \subset L$?}
%
where $L$ runs over all Levi subgroups of $G$. There are surjective maps
%
$$\Sat: \Orb_0(G) \to \Orb(G), \quad \Sat: \Conj_0(G) \to \Conj(G), \quad \Sat: \Som_0(G) \to \Som(G)$$
%
\begin{prop}\label{prop:BalaCarter}
The following are true:
\begin{itemize}
    \item[(i)] $\Sat: \Orb_0(G) \to \Orb(G)$ is a bijection.
    \item[(ii)] If $Z(G)$ is connected, then $\Sat: \Conj_0(G) \to \Conj(G)$ is a bijection.
    \item[(iii)] $\Sat: \Som_0(G) \to \Som(G)$ is a bijection.
\end{itemize}
\end{prop}

\begin{proof}
(i) is the classical Bala-Carter theorem, see \cite[Theorem 8.2.12]{CM} for a proof. For (iii), note that $(M,\OO_M) \in \Som(G)$ is distinguished if and only if $\fz(\fg)=\fz(\fm)$. But if $(M,\OO_M) \in \Som(G)$, there is a unique Levi subgroup $L \subset G$ containing $M$ such that $\fz(\fm)=\fz(\fl)$, namely $L:=Z_G(\fz(\fm))$. This proves (iii).

For (ii), suppose
%
$$\Sat(L,(\OO_L,C_L)) = \Sat(L',(\OO_{L'},C_{L'})) = (\OO,C).$$
%
Let $(M,\OO_M) = \alpha^L(\OO_L,C_L)$ and $(M',\OO_{M'}) = \alpha^{L'}(\OO_{L'},C_{L'})$. By (i) of Lemma \ref{lem:alphabeta}, we have $\beta^L(M,\OO_M) = (\OO_L,C_L)$ and $\beta^{L'}(M',\OO_{M'}) = (\OO_{L'},C_{L'})$. So by the first commutative diagram of Proposition \ref{prop:twodiagrams}, both $(M,\OO_M) \in \Som(L)$ and $(M',\OO_{M'}) \in \Som(L')$ are distinguished. By the second commutative diagram of Proposition \ref{prop:twodiagrams}, we have
%
$$\Sat (L,(M,\OO_M)) = \Sat (L', (M',\OO_{M'}))  = \alpha^G(\OO,C).$$
%
So by (iii), $(L,(M,\OO_M))$ and $(L', (M',\OO_{M'}))$ are conjugate, and hence $(L,(\OO_L,C_L))$ and $(L',(\OO_{L'},C_{L'}))$ are conjugate. This completes the proof.
\end{proof}




\subsection{Nilpotent covers}

A \emph{nilpotent cover} for $G$ is a finite connected $G$-equivariant cover of a nilpotent $G$-orbit. A map of nilpotent covers is a $G$-equivariant morphism $\widetilde{\OO} \to \widehat{\OO}$ which intertwines the covering maps. Let
%
$$\Cov(G) := \{\text{isomorphism classes of nilpotent covers $\widetilde{\OO}$ for $G$}\}$$
%
If $\OO \in \Orb(G)$, then (isomorphism classes of) nilpotent covers of $\OO$ are in one-to-one correspondence with (conjugacy classes of) subgroups of $A(\OO)$. In particular, $\Cov(G)$ is finite. 


Following \cite{LMBM}, we will define an equivalence relation $\sim$ on $\Cov(G)$. Suppose $\widetilde{\OO} \to \widehat{\OO}$ is a morphism of covers. Then there is an induced map of affine varieties $\Spec(\CC[\widetilde{\OO}]) \to \Spec(\CC[\widehat{\OO}])$. We write $\widetilde{\OO} \geqslant \widehat{\OO}$ if this map is \'{e}tale over all $G$-orbits in $\Spec(\CC[\widehat{\OO}])$ of codimension $2$ (it is automatically \'{e}tale over the open $G$-orbit $\widehat{\OO}$) This defines a partial order on $\Cov(G)$. 

\begin{definition}[Definition 6.5.1, \cite{LMBM}]
Let $\sim$ be the equivalence relation on $\Cov(G)$ defined by taking the symmetric closure of $\geqslant$. Let
%
$$\underline{\Cov}(G) := \Cov(G)/\sim$$
%
For $\widetilde{\OO} \in \Cov(G)$, let $[\widetilde{\OO}] \in \underline{\Cov}(G)$ denote the equivalence class of $\widetilde{\OO}$.
\end{definition}

We will need some basic facts about equivalence classes in $\Cov(G)$.

\begin{lemma}[Lemma 6.5.3, \cite{LMBM}]
Let $[\widetilde{\OO}] \in \underline{\Cov}(G)$. Then the following are true:
\begin{itemize}
    \item[(i)] $[\widetilde{\OO}]$ contains a unique maximal cover $\widetilde{\OO}_{max}$.
    \item[(ii)] $\widetilde{\OO}_{max}$ is Galois over every cover in $[\widetilde{\OO}]$.
\end{itemize}
\end{lemma}




\subsection{Induction}\label{subsec:induction}

Suppose $L \subset G$ is a Levi subgroup and let $\mathbb{O}_L \in \Orb(L)$. Fix a parabolic subgroup $P \subset G$ with Levi decomposition $P = LU$. The annihilator of $\fp$ in $\fg^*$ is a $P$-stable subspace $\fp^{\perp} \subset \fg^*$. Form the $G$-equivariant fiber bundle $G \times^Q (\overline{\mathbb{O}}_L \times \mathfrak{p}^{\perp})$ over the partial flag variety $G/P$. There is a proper $G$-equivariant map
%
$$\mu: G \times^P (\overline{\mathbb{O}}_L \times \mathfrak{p}^{\perp}) \to \mathfrak{g}^* \qquad \mu(g,\xi) = \Ad^*(g)\xi$$
%
The image of $\mu$ is a closed irreducible $G$-invariant subset of $\cN$, and hence the closure in $\fg^*$ of a nilpotent $G$-orbit, denoted $\mathrm{Ind}^G_L\mathbb{O}_L  \in \Orb(G)$. It is a standard fact that $\Ind^G_L \OO_L$ is independent of the choice of parabolic $P$. The correspondence
%
$$\mathrm{Ind}^G_L: \Orb(L) \to \Orb(G)$$
%
is called \emph{Lusztig-Spaltenstein} induction. 

Now let $\widetilde{\OO}_L \in \Cov(L)$ and form the affine variety $\Spec(\CC[\widetilde{\OO}_L])$. There is an $L$-action on $\Spec(\CC[\widetilde{\OO}_L])$ (induced from the $L$-action on $\widetilde{\mathbb{O}}_L$) and a finite surjective $L$-equivariant map $\Spec(\CC[\widetilde{\OO}_L]) \to \overline{\mathbb{O}}_L$. Let $\widetilde{\mu}$ denote the composition
%
$$G \times^P (\Spec(\CC[\widetilde{\OO}_L]) \times \mathfrak{p}^{\perp}) \to G \times^P (\overline{\mathbb{O}}_L \times \mathfrak{p}^{\perp}) \overset{\mu}{\to} \fg^*.$$
%
The image of $\widetilde{\mu}$ is the closure of $\Ind^G_L\OO_L$ and the preimage of $\Ind^G_L\OO_L$ is a nilpotent cover, denoted $\Bind^G_L \widetilde{\OO}_L \in \Cov(G)$. Again, $\Bind^G_L\widetilde{\OO}_L$ is independent of the choice of parabolic $P$ (see \cite[Proposition 2.4.1(i)]{LMBM}). The correspondence
%
$$\Bind^G_L: \Cov(L) \to \Cov(G)$$
%
is called \emph{birational induction}. We will need several basic facts about birational induction.

\begin{prop}\label{prop:propsofbind}
Birational induction has the following properties

\begin{enumerate}
    \item[(i)] Suppose $M \subset G$ is a Levi subgroup containing $L$. Then
    %
    $$\mathrm{Bind}^G_L = \mathrm{Bind}^G_M \circ \mathrm{Bind}^M_L.$$
    \item[(ii)] For any $\widetilde{\OO}_L \in \Cov(L)$, $\deg(\widetilde{\OO}_L)$ divies $\deg(\Bind^G_L \widetilde{\OO}_L)$.
    \item[(iii)] Suppose $\widetilde{\OO}_L, \widehat{\OO}_L \in \Cov(L)$ and let $\widetilde{\OO} = \Bind^G_L \widetilde{\OO}_L$, $\widehat{\OO} = \Bind^G_L \widehat{\OO}_L$. If there is a finite Galois $L$-equivariant covering $\widehat{\OO}_L \to \widetilde{\OO}_L$, then there is a finite Galois $G$-equivariant covering $\widehat{\OO} \to \widetilde{\OO}$ and a group isomorphism
%
$$\Aut(\widehat{\OO},\widetilde{\OO}) \simeq \Aut(\widehat{\OO}_L, \widetilde{\OO}_L).$$
\end{enumerate}
\end{prop}

\begin{proof}
(i) and (ii) are (ii) and (iv) of \cite[Proposition 2.4.1]{LMBM}. For (iii), we argue as follows\todo{Mitya finish}
\end{proof}

A nilpotent orbit (resp. nilpotent cover) is \emph{rigid} (resp. \emph{birationally rigid}) if it cannot be obtained by induction (resp. birational induction) from a proper Levi subgroup. Note that if $\OO \in \Orb(G)$ is rigid and $\widetilde{\OO}$ covers $\OO$, then $\widetilde{\OO}$ is birationally rigid. Let
%
$$\Cov_0(G) := \{(L,\widetilde{\OO}_L) \mid \widetilde{\OO}_L \text{ is birationally rigid}\}/G$$

\begin{prop}[Proposition 2.4.1(iii), \cite{LMBM}]\label{prop:bindinjective}
The map
%
$$\Bind: \Cov_0(G) \to \Cov(G), \qquad \Bind(L,\widetilde{\OO}_L) = \Bind^G_L \widetilde{\OO}_L$$
%
is a bijection. 
\end{prop}

We will see in Section \ref{subsec:unipotent} that birational induction preserves the equivalence relation on nilpotent covers and (in classical types) takes maximal covers to maximal covers. 

We conclude this subsection by describing a large class of orbits which are birationally induced from $\{0\}$. Suppose $\OO \in \Orb(G)$. Using an $\Ad(\fg)$-invariant identification $\fg \simeq \fg^*$, we can regard $\OO$ as a nilpotent $G$-orbit in $\fg$. Choose an element $e \in \OO$ and an $\mathfrak{sl}(2)$-triple $(e,f,h)$. The operator $\ad(h)$ defines a $\ZZ$-grading on $\fg$
%
$$\fg = \bigoplus_{i \in \ZZ} \fg_i, \qquad \fg_i := \{\xi \in \fg \mid \ad(h)(\xi) = i\xi\}.$$
%
We say that $\OO$ is \emph{even} if $\fg_i=0$ for every odd integer $i$. In any case, we can define a parabolic subalgebra
%
\begin{equation}\label{eq:JMlevi}\mathfrak{p}_{\OO} = \mathfrak{l}_{\OO} \oplus \mathfrak{n}_{\OO}, \qquad \fl_{\OO} := \fg_0, \qquad \fn_{\OO} := \bigoplus_{i \geq 1} \fg_i.\end{equation}
%
We call $\fp_{\OO}$ (resp. $\fl_{\OO}$) the \emph{Jacobson-Morozov} parabolic (resp. Levi) associated to $\OO$. Both $\fp_{\OO}$ and $\fl_{\OO}$ are well-defined up to conjugation by $G$. The following result is well-known. The proof is contained in \cite{Kostant1959}, see also \cite[Thm 3.3.1]{CM}.

\begin{prop}\label{prop:even}
Suppose $\OO$ is an even nilpotent $G$-orbit. Then
%
$$\OO = \mathrm{Bind}^G_{L_{\OO}} \{0\}.$$
\end{prop}



\subsection{Truncated induction}
\todo{revise this section}There is a generalization of Lusztig-Spaltenstein induction defined in \cite[Chp 13.3]{Lusztig1984}. Suppose $M$ is a connected reductive algebraic group which is \emph{endoscopic} for $G$. This is equivalent to the requirement that $M$ is the Langlands dual group of a pseudolevi subgroup of $G^{\vee}$.
Then there is a map
%
$$\mathrm{J}^G_M: \Orb(M) \to \Orb(G)$$ ?
%
called \emph{truncated induction}. If $M$ is a Levi subgroup of $G$, then $\mathrm{J}^G_M$ coincides with $\Ind^G_M$. 

\subsection{Primitive ideals}

Let $U(\fg)$ be the universal enveloping algebra of $\fg$. Recall that $U(\fg)$ has a natural natural filtration and there is a $G$-equivariant isomorphism $\gr U(\fg) \simeq S(\fg)$. Now let $I \subset U(\fg)$ be a two-sided ideal. Then $\gr(I)$ corresponds under the isomorphism $\gr U(\fg) \simeq S(\fg)$ to a $G$-invariant ideal in $S(\fg)$. The \emph{associated variety} of $I$ is defined to be the vanishing locus $V(I) \subset \fg^*$ of this ideal.

A two-sided ideal $I \subset U(\fg)$ is said to be \emph{primitive} if it is the annihilator of a simple left $U(\fg)$-module. If $I$ is primitive, then $V(I)$ is irreducible (see \cite{Joseph1985}) and hence the closure of a (unique) nilpotent orbit.

By Quillen's lemma, the intersection of $I$ with the center $\mathfrak{Z}(\fg)$ of $U(\fg)$ is the kernel of an algebra homomorphism $\mathfrak{Z}(\fg) \to \CC$, called the \emph{infinitesimal character} of $I$. Such homomorphisms are identified via the Harish-Chandra isomorphism with $W$-orbits on $\fh^*$. For each $\gamma \in \fh^*/W$, there is a \emph{unique} maximal (primitive) ideal in $U(\fg)$ with infinitesimal character $\gamma$, which we will denote by $J(\gamma) \subset U(\fg)$.


\subsection{Barbasch-Vogan-Lusztig-Spaltenstein duality}

Let $G^{\vee}$ be the Langlands dual group of $G$ and let $\fg^{\vee}$ be its Lie algebra. If we fix a Cartan subalgebra $\fh \subset \fg$, we get a Cartan subalgebra $\fh^{\vee} \subset \fg^{\vee}$ and a canonical identification $\fh^{\vee} \simeq \fh^*$. To each nilpotent $G^{\vee}$ orbit $\OO^{\vee} \in \Orb(G^{\vee})$ we can associate a maximal ideal in $U(\fg)$ in the following manner. First, using an $G^{\vee}$-invariant isomorphism $(\fg^{\vee})^* \simeq \fg^{\vee}$, we can identify $\OO^{\vee}$ with a nilpotent $G^{\vee}$-orbit in $\fg^{\vee}$ (still denoted $\OO^{\vee}$). Next, we choose an $\mathfrak{sl}(2)$-triple $(e^{\vee},f^{\vee},h^{\vee})$ with $e^{\vee} \in \OO^{\vee}$ and $h^{\vee} \in \fh^{\vee} \simeq \fh^*$. The element $\frac{1}{2}h^{\vee}$ is well-defined up to the $W$-action on $\fh^*$, and hence determines an infinitesimal character for $U(\fg)$, which we will denote by $\gamma_{\OO^{\vee}}$. \todo{include discussion of LS duality}

\begin{definition}\label{def:specialunipotent}
Let $\OO^{\vee} \in \Orb(G^{\vee})$. Then the \emph{special unipotent ideal} attached to $\OO^{\vee}$ is the maximal ideal $J(\gamma_{\OO^{\vee}}) \subset U(\fg)$.
\end{definition}


For each nilpotent orbit $\OO^{\vee} \in \Orb(G^{\vee})$, let $d(\OO^{\vee})$ denote the (unique) open $G$-orbit in $V(J(\gamma_{\OO^{\vee}}))$. This defines a map
%
$$d: \Orb(G^{\vee}) \to \Orb(G)$$
%
called \emph{Barbasch-Vogan-Lusztig-Spaltenstein duality}. We will sometimes write $d^G$ instead of $d$, when we wish to emphasize the dependence on $G$. 

\begin{prop}[Proposition A2, \cite{BarbaschVogan1985}]\label{prop:propsofd}
The map $d$ enjoys the following properties:
\begin{itemize}
    \item[(i)] $d$ is order-reversing (with respect to the clsoure orderings on $\Orb(G)$ and $\Orb(G^{\vee})$).
    \item[(ii)] $d^3=d$.
    \item[(iii)] If $L \subset G$ is a Levi subgroup, then
    %
    $$d^G \circ \Sat^{G^{\vee}}_{L^{\vee}} = \Ind^G_L \circ d^L$$
\end{itemize}
\end{prop}



\subsection{The associated variety of a maximal ideal}\label{subsec:maximal}

\todo{is this section needed?}To each element $\gamma \in \fh^*$, one can associate a nilpotent orbit for $G$, namely the (unique) open orbit in $V(J(\gamma))$. This defines a ($W$-invariant) map from $\fh^*$ to $\Orb(G)$. This map can be computed, using ideas in \cite{BarbaschVogan1985}. 

Let $L^{\vee}_{\gamma}$ be the pseudolevi subgroup of $G^{\vee}$ defined by $\exp(2\pi i \gamma)$,
%
$$L^{\vee}_{\gamma} = Z_{G^{\vee}}(\exp(2\pi i \gamma))^{\circ} \subset G^{\vee},$$
%
and let $L_{\gamma,0}$ be the Levi subgroup of $G^{\vee}$ (and of $L^{\vee}_{\gamma}$) defined by $\gamma$,
%
$$L^{\vee}_{\gamma,0} = Z_{G^{\vee}}(\gamma) \subset L^{\vee}_{\gamma}.$$
%
Note that the roots for $L^{\vee}_{\gamma}$ (resp. $L^{\vee}_{\gamma,0}$) are precisely the roots for $G^{\vee}$ which are integral (resp. singular) on $\gamma$. Let $\OO^{\vee}_{\gamma}$ be the Richardson orbit for $L^{\vee}_{\gamma}$ corresponding to $L^{\vee}_{\gamma,0}$, i.e., 
%
$$\OO^{\vee}_{\gamma} = \Ind^{L^{\vee}_{\gamma}}_{L^{\vee}_{\gamma,0}} \{0\} \in \Orb(L^{\vee}_{\gamma}).$$
%
Finally, let $L_{\gamma}$ be the Langlands dual of $L^{\vee}_{\gamma}$ (an endoscopic group for $G$).

\begin{prop}[Proposition A2, \cite{BarbaschVogan1985}]
Let $\gamma \in \fh^*$. Then $V(J(\gamma))$ is the closure of the nilpotent orbit $J^G_{L_{\gamma}} d(\OO^{\vee}_{\gamma})$.
\end{prop}


\subsection{Sommers duality}

Following \cite{Sommers2001}, we will define a surjective map 
%
$$d_S: \Conj(G^{\vee}) \twoheadrightarrow \Orb(G)$$
%
called \emph{Sommers duality}. Suppose $(\OO^{\vee},C) \in \Conj(G^{\vee})$. Let $(M^{\vee}, \OO_{M^{\vee}}) = \alpha(\OO^{\vee},C)$ (see (\ref{eq:alpha}), and let $M$ denote the Langlands dual of $M^{\vee}$. Then we define
%
$$d_S(\OO^{\vee},C) :=  J^G_M d(\OO_{M^{\vee}}) \in \Orb(G)$$
%
We will sometimes write $d_S^G$ instead of $d_S$ when we wish to emphasize the dependence on $G$.

\begin{prop}[Section 6, \cite{Sommers2001}]\label{prop:propsofds}
The map $d_S: \Conj(G^{\vee}) \to \Orb(G)$ has the following properties:
\begin{itemize}
    \item[(i)] $d_S$ is surjective.
    \item[(ii)] If $L \subset G$ is a Levi subgroup, then
    %
    $$d_S^G \circ \Sat^{G^{\vee}}_{L^{\vee}} = \Ind^G_L \circ d_S^L$$
    \item[(iii)] $d_S(\OO^{\vee},1) = d(\OO^{\vee})$, for every $\OO^{\vee} \in \Orb(G^{\vee})$.
\end{itemize}
\end{prop}




\subsection{Lusztig's canonical quotient}\label{subsec:Abar}

For each $\OO \in \Orb(G)$, there is a canonically defined quotient group $\bar{A}(\OO)$ of $A(\OO)$, called \emph{Lusztig's canonical quotient}. In \cite{Lusztig1984}, this quotient is defined in the case when $\OO$ is \emph{special}, but in fact Lusztig's definition is valid for arbitrary $\OO$. An alternative description of $\bar{A}(\OO)$ is provided in \cite[Section 5]{Sommers2001}), which we briefly recall here. 

Sommers defines the \emph{$\tilde{b}$-value} of any $(\OO, C) \in \Conj(G)$ as follows.
For any $(M, \OO_M)$ such that $\beta(M, \OO_M) = (\OO, C)$, apply the original Lusztig-Spaltenstein duality map $d^M_{LS}$ with respect to $M$, we obtain the orbit $\OO_M' = d^M(\OO_M) \subset \fm$ (here $d_{LS}^M$ stays within $\fm$ and we don't pass to the dual group). We define $\tilde{b}_{(\OO,C)} := \frac{1}{2}(\dim M - \dim \OO_M' - \rank G )$, where $\rank G$ is the rank of $G$. Equivalently, $\tilde{b}_{(\OO,C)}$ is the dimension of the Springer fiber attached to any element in $\OO_M'$. Sommers shows that $\tilde{b}_{(\OO,C)}$ only depends on $(\OO,C)$ and is independent of the choice of $(M, \OO_M)$ (\cite[Proposition 1]{Sommers2001}. In fact, $\tilde{b}_{(\OO,C)}$ coincides with the dimension of the Springer fibers of the orbit $d_S(\OO,C)$ in $\fg^\vee$ (see \cite[Section 6]{Sommers2001}). The $\tilde{b}$-values satisfy the property that $\tilde{b}_{\OO,C} \geq \tilde{b}_{\OO,1}$ for any conjugacy class $C$ of $A(\OO)$ (\cite[Proposition 3]{Sommers2001}).

Next, let $H'_\OO$ be the union of all conjugacy class $C$ in $A(\OO)$ such that $\tilde{b}_{\OO,C} = \tilde{b}_{\OO,1}$. A case-by-case calculation shows that $H'_\OO$ is a subgroup of $A(\OO)$ and coincides with a subgroup $H_\OO$ which Lusztig defines using Springer theory and generic degrees of irreducible representations of the Weyl group, so that $\bar{A}(\OO) = A(\OO)/ H_\OO = A(\OO)/ H'_\OO$ (\cite[Theorem 6]{Sommers2001}).


\subsection{Achar data}\label{subsec:Achar}
An \emph{Achar datum} for $G$ is a pair $(\OO, \bar{C})$ consisting of a nilpotent orbit $\OO \in \Orb(G)$ and a conjugacy class $\bar{C}$ in $\bar{A}(\OO)$. Let
%
$$\Ach(G) := \{\text{Achar data $(\OO,\bar{C})$ for $G$}\}$$
%
The following is proved in \cite{Achar2003}.
%
\begin{lemma}[\cite{Achar2003}, Theorems 5.1,6.1]\label{lem:AtoAbar}
Let $\OO \in \Orb(G)$ and let $C_1$ and $C_2$ be conjugacy classes in $A(\OO)$. Then the following are equivalent
\begin{itemize}
    \item[(i)] $d_S(\OO,C_1) = d_S(\OO,C_2)$.
    \item[(ii)] $C_1$ and $C_2$ have the same image in $\bar{A}(\OO)$. 
\end{itemize}
\end{lemma}

\todo{S.Y.: $G_{ad}$ is probably a more standard notations}
Now let $G^{ad} = G/Z(G)$. The surjective map $\Conj(G) \to \Conj(G^{ad})$ induces a map $\Ach(G) \to \Ach(G^{ad})$. Since $\bar{A}(\OO)$ is independent of isogeny\todo{Reference}, the latter map is a bijection. The composition 
%
$$\Som(G) = \Som(G^{ad}) \overset{\beta}{\twoheadrightarrow} \Conj(G^{ad}) \twoheadrightarrow \Ach(G^{ad}) \simeq \Ach(G)$$
%
defines a surjective map
%
$$\pi: \Som(G) \twoheadrightarrow \Ach(G)$$
%
\begin{lemma}\label{lem:SomAch}
The following are true:
\begin{itemize}
    \item[(i)] The map $d_S: \Conj(G^{\vee}) \to \Orb(G)$ factors through the quotient map $\Conj(G^{\vee}) \twoheadrightarrow \Ach(G^{\vee})$. 
    \item[(ii)] The composition $\Som_{large}(G^{\vee}) \overset{\pi}{\twoheadrightarrow} \Ach(G^{\vee}) \overset{d_S}{\twoheadrightarrow} \Orb(G)$ coincides with the map 
    %
    $$(M^{\vee},\OO_{M^{\vee}}) \mapsto J^G_M d(\OO_{M^{\vee}})$$
\end{itemize}
\end{lemma}

\begin{proof}
We can assume without loss that $G^{\vee}$ is adjoint. (i) is immediate from Lemma \ref{lem:AtoAbar}. For (ii), write $f: \Som(G^{\vee}) \to \Orb(G)$ for the map defined by $f(M^{\vee},\OO_{M^{\vee}}) = J^G_M d(\OO_{M^{\vee}})$. Then by definition, $d_S: \Conj(G^{\vee}) \to \Orb(G)$ is the composition %
$$\Conj(G^{\vee}) \overset{\alpha}{\to} \Som(G^{\vee}) \overset{f}{\to} \Orb(G).$$
%
So the composition 
%
$$\Som_{large}(G^{\vee}) \overset{\pi}{\twoheadrightarrow} \Ach(G^{\vee}) \overset{d_S}{\twoheadrightarrow} \Orb(G)$$
%
coincides with the composition
%
\begin{equation}\label{eq:1}\Som_{large}(G^{\vee}) \overset{\beta}{\to} \Conj(G^{\vee}) \overset{\alpha}{\to} \Som(G^{\vee}) \overset{f}{\to} \Orb(G)\end{equation}
%
By Lemma \ref{lem:alphabeta}(ii), $\alpha \circ \beta$ is the identity on $\Som_{large}(G^{\vee})$. So (\ref{eq:1}) coincides with the map $f: \Som_{large}(G^{\vee}) \to \Orb(G)$, as desired.
\end{proof}

We will write $d_S: \Ach(G^{\vee}) \to \Orb(G)$ for the map induced from $d_S: \Conj(G^{\vee}) \to \Orb(G)$ and $\underline{d}_S: \Som_{large}(G^{\vee}) \to \Orb(G)$ for the composition in Lemma \ref{lem:SomAch}(ii). By definition, the latter map factors through the former (but it may not factor through the map $d_S: \Conj(G^{\vee}) \to \Orb(G)$ if $Z(G^{\vee})$ is disconnected). 

We wish to define a notion of `saturation' for Achar data analogous to (\ref{eq:satconj}). We will need the following lemma.

\begin{lemma}\label{lem:K(O)}
Suppose $Z(G)$ is connected. Then for each $\OO \in \Orb(G)$, there is a subgroup $K(\OO) \subset A(\OO)$ such that
    \begin{itemize}
        \item[(i)] The quotient map $A(\OO) \to \bar{A}(\OO)$ restricts to an isomorphism $K(\OO) \xrightarrow{\sim} \bar{A}(\OO)$.
        \item[(ii)] The natural map from conjugacy classes in $K(\OO)$ to conjugacy classes in $A(\OO)$ is injective.
        \item[(iii)] If $L \subset G$ is a Levi subgroup and $\OO_L \in \Orb(L)$ such that $\OO=\mathrm{Sat}^G_L \OO_L$, then the homomorphism $\iota$ defined in (\ref{eq:iota}) maps $K(\OO_L)$ to $K(\OO)$.
    \end{itemize}
\end{lemma}

\begin{proof}
For $G$ a classical group, subgroups with these properties were exhibited in \cite[Section 5]{Sommers2001}. For $G$ an adjoint exceptional group, there are three possibilities:
\begin{enumerate}
    \item $A(\OO) \simeq \bar{A}(\OO)$.
    \item $A(\OO) \simeq S_2$, $\bar{A}(\OO) \simeq 1$.
    \item $G$ is of type $E_8$, $\OO$ is the distinguished orbit $E_8(b_6)$, $A(\OO) \simeq S_3$, and $\bar{A}(\OO) \simeq S_2$.
\end{enumerate}
In the first case, we take $K(\OO)=A(\OO)$.In the second case, we take $K(\OO)=\{1\}$. In the third case, we take $K(\OO)$ to be any order $2$ subgroup of $A(\OO)$. It is an easy exercise to check that conditions (i), (ii), and (iii) are satisfied for these choices of $K(\OO)$.
\end{proof}

Suppose $Z(G)$ is connected and $\bar{C}$ is a conjugacy class in $\bar{A}(\OO)$. Let $C'$ be the preimage of $\bar{C}$ under the isomorphism $K(\OO) \xrightarrow{\sim} \bar{A}(\OO)$ of Lemma \ref{lem:K(O)}(i). By Lemma \ref{lem:K(O)}(ii), there is a unique conjugacy class $C$ in $A(\OO)$ such that $C \cap K(\OO) = C'$. Taking $(\OO,\bar{C})$ to $(\OO,C)$ defines an injective map $\Ach(G) \to \Conj(G)$, right-inverse to the projection $\Conj(G) \to \Ach(G)$. Thus the composition
%
$$\Ach(G) \simeq \Ach(G^{ad}) \hookrightarrow \Conj(G^{ad}) \overset{\alpha}{\hookrightarrow} \Som(G^{ad}) = \Som(G)$$
%
defines an injective map
%
$$\eta: \Ach(G) \hookrightarrow \Som(G)$$
%
right-inverse to $\pi$. 

Now suppose $L \subset G$ is a Levi subgroup and let $\OO_L \in \Orb(L)$. Recall, there is a homomorphism
%
$$\iota: A(\OO_L) \to A(\mathrm{Sat}^G_L \OO_L),$$
%
see (\ref{eq:iota}). 

\begin{prop}\label{prop:iotaAbar}
The homomorphism $\iota: A(\OO_L) \to A(\Sat^G_L\OO_L)$ descends to a homomorphism $\bar{\iota}: \bar{A}(\OO_L) \to \bar{A}(\Sat^G_L\OO_L)$. 
\end{prop}

\begin{proof}
  Let $\OO = \Sat^G_L\OO_L$. It follows from the definition of $\Tilde{b}$-value and Proposition \ref{prop:twodiagrams} that 
  $$\tilde{b}(\Sat^G_L(\OO_L, C_L)) = \Tilde{b}(\OO_L,C_L)$$ 
  for any conjugacy class $C_L$ in $A(\OO_L)$. Therefore $\iota(H'_{\OO_L}) \subset H'_\OO$ and the proposition holds. 
\end{proof}

Using Proposition \ref{prop:iotaAbar}, we can define a map
%
$$\mathrm{Sat}^G_L: \Ach(L) \to \Ach(G), \qquad \mathrm{Sat}^G_L(\OO_L, \bar{C}_L) = (\mathrm{Sat}^G_L\OO_L, \bar{\iota}(\bar{C}_L))$$
%

\begin{prop}\label{prop:twodiagramsAbar}
The following are true:
\begin{itemize}
    \item[(i)] Let $L \subset G$ be a Levi subgroup. Then the following diagrams commute
\begin{center}
    \begin{tikzcd}
    \Som(L) \ar[r,"\Sat^G_L"] \ar[d,twoheadrightarrow, "\pi^L"]& \Som(G) \ar[d,twoheadrightarrow, "\pi^G"]\\
    \Ach(L) \ar[r,"\Sat^G_L"]& \Ach(G) 
    \end{tikzcd}
    \begin{tikzcd}
    \Ach(L) \ar[r,"\Sat^G_L"] \ar[d,hookrightarrow, "\eta^L"]& \Ach(G) \ar[d,hookrightarrow, "\eta^G"]\\
    \Som(L) \ar[r,"\Sat^G_L"]& \Som(G) 
    \end{tikzcd}
\end{center}
%\item[(ii)] If $(\OO,\bar{C})$ is distinguished, then $\pi^{-1}(\OO,\bar{C})$ consists of large Sommers data.
\item[(ii)] Let $(M_1,\OO_{M_1}), (M_2, \OO_{M_2}) \in \Som_{large}(G)$. Then $\pi(M_1,\OO_{M_1}) = \pi(M_2, \OO_{M_2})$ if and only if $\underline{d}_S(M_1,\OO_{M_1}) = \underline{d}_S(M_2,\OO_{M_2})$ and $G \cdot \OO_{M_1} = G \cdot \OO_{M_2}$.
\end{itemize}
\end{prop}

\begin{proof}
We can assume without loss that $Z(G)$ is connected. For (i), we consider the following diagrams
\begin{center}
    \begin{tikzcd}
        \Conj(L) \ar[d,twoheadrightarrow] \ar[r,"\Sat^G_L"] & \Conj(G) \ar[d,twoheadrightarrow]\\
        \Ach(L) \ar[r,"\Sat^G_L"] & \Ach(G)
    \end{tikzcd}
    \begin{tikzcd}
        \Ach(L) \ar[d,hookrightarrow] \ar[r,"\Sat^G_L"] & \Ach(G) \ar[d,hookrightarrow] \\
        \Conj(L) \ar[r,"\Sat^G_L"] & \Conj(G)
    \end{tikzcd}
\end{center}
In the left diagram, the vertical maps are the natural projections. In the right diagram, the vertical maps are the injections defined in the paragraph following Lemma \ref{lem:K(O)}. The left diagram commutes by Proposition \ref{prop:iotaAbar} and the right diagram commutes by Lemma \ref{lem:K(O)}. The diagrams in (i) are obtained by pasting the diagrams above to those of Proposition \ref{prop:twodiagrams}. (ii) is immediate from Lemma \ref{lem:AtoAbar} and the definition of $\underline{d}_S$.
\end{proof}

An Achar datum $(\OO,\bar{C}) \in \Ach(G)$ is said to be \emph{distinguished} if it cannot be obtained by saturation from a proper Levi subgroup. Let
%
$$\Ach_0(G) := \{(L,(\OO_L,\bar{C}_L)) \mid (\OO_L,\bar{C}_L) \text{ is distinguished}\}/G$$
%
where, as usual, $L$ runs over all Levi subgroups of $G$.

\begin{prop}\label{prop:uniquedistinguishedAbar}
The map
%
$$\mathrm{Sat}: \Ach_0(G) \to \Ach(G), \qquad \mathrm{Sat}(L,(\OO_L,\bar{C}_L)) = \Sat^G_L(\OO_L,\bar{C}_L)$$
%
is a bijection.
\end{prop}

\begin{proof}
This is completely analagous to the proof of Proposition \ref{prop:BalaCarter}(ii). We replace $\alpha$ and $\beta$ with $\eta$ and $\pi$ and Proposition \ref{prop:twodiagrams} with Proposition \ref{prop:twodiagramsAbar}.
\end{proof}
  
\subsection{Special Achar data}\label{subsec:specialAchar}

Let $(\OO,\bar{C}) \in \Ach(G)$ and let $\OO^{\vee} = d_S^{G^{\vee}}(\OO,\bar{C})$. Following Achar (\cite{Achar2003}) We say that $(\OO,\bar{C})$ is \emph{special} if there is a conjugacy class $\bar{C}' \subset \bar{A}(\OO^{\vee})$ such that
%
$$d_S^G(\OO^{\vee},\bar{C}') = \OO$$
%
Let
%
$$\Ach^*(G) := \{\text{special Achar data $(\OO,\bar{C})$ for $G$}\}$$
%
and
%
$$\Ach^*_0(G) := \{(L,(\OO_L,\bar{C}_L)) \mid (\OO_L,\bar{C}_L) \text{ is special and distinguished}\}/G$$
%
where, as usual, $L$ runs over all Levi subgroups of $G$. We will need several basic facts about special Achar data.

\begin{prop}\label{prop:specialtospecial}
The following are true:
\begin{itemize}
    \item[(i)] For any orbit $\OO \in \Orb(G)$, the Achar datum $(\OO,1)$ is special.
    \item[(ii)] The bijection of Proposition \ref{prop:uniquedistinguishedAbar} induces an injection
    %
    $$\Sat^{-1}: \Ach^*(G) \hookrightarrow \Ach^*_0(G)$$
\end{itemize}
\end{prop}

\begin{proof}
(i) is \cite[Proposition 2.7]{Achar2003}. We proceed to proving (ii). In classical types all distinguished Achar data are special, see \cite[Section 5.2]{Achar2003}. So (ii) is immediate. In exceptional types, a list of \todo{Lucas finish}
\end{proof}


\subsection{The Namikawa space}

Let $\widetilde{\OO} \in \Cov(G)$. Associated to $\widetilde{\OO}$ is a certain finite-dimensional complex vector space $\fP(\widetilde{\OO})$ called the \emph{Namikawa space} for $\widetilde{\OO}$. This space is defined as follows. Choose $(L,\widetilde{\OO}_L) \in \Cov_0(G)$ such that $\Bind(L,\widetilde{\OO}_L) = \widetilde{\OO}$. By Proposition \ref{prop:bindinjective}, $(L,\widetilde{\OO}_L)$ is unique (up to conjugation by $G$). Choose a parabolic subgroup $P\subset G$ with Levi decomposition $P=LU$. Form the variety $Y=G \times^P(\Spec(\CC[\widetilde{\OO}_L]) \times \fp^{\perp})$ and consider the proper $G$-equivariant map $\widetilde{\mu}:Y \to \overline{\OO}$ defined in Section \ref{subsec:induction}. This map admits a Stein factorization
%
$$Y \to \Spec(\CC[\widetilde{\OO}]) \to \overline{\OO}$$
%
(the first map is birational and the second is finite). We define $\fP(\widetilde{\OO})$ to be the second cohomology of the regular locus of $Y$
%
$$\fP(\widetilde{\OO}) := H^2(Y^{reg},\CC).$$
%
\begin{prop}[Proposition 7.2.2, \cite{LMBM}]\label{prop:Namikawacenter}
There is a linear isomorphism
%
$$\fP(\widetilde{\OO}) \simeq \fz(\fl \cap [\fg,\fg])$$
\end{prop}

Another description of $\fP(\widetilde{\OO})$ can be obtained by analyzing the geometry of $\Spec(\CC[\widetilde{\OO}])$. The discussion below closely follows \cite[Section 4.5]{LMBM}, and we refer the reader there for proofs and references. Note that $\Spec(\CC[\widetilde{\OO}])$ is a symplectic singularity, and therefore decomposes as a union of finitely-many symplectic leaves. For each codimension 2 leaf $\fL_k \subset X$, the formal slice to $\fL_k \subset X$ is identified with the formal neighborhood at $0$ in a Kleinian singularity $\Sigma_k = \CC^2/\Gamma_k$, see \cite{Namikawa}. Under the McKay correspondence, $\Gamma_k$ corresponds to a complex simple Lie algebra $\fg_k$ of type A, D, or E. Fix a Cartan subalgebra $\fh_k \subset \fg_k$. Write $\Lambda_k \subset \fh_k^*$ for the weight lattice and $W_k$ for the Weyl group. If we choose a point $x \in \fL_k$, there is a natural identification $H^2(\widetilde{\mu}^{-1}(x),\ZZ) \simeq \Lambda_k$, and $\pi_1(\fL_k)$ acts on $\Lambda_k$ by diagram automorphisms. The \emph{partial Namikawa space} corresponding to $\fL_k$ is the subspace
%
$$\fP_{k}(\widetilde{\OO}) := (\fh_{k}^*)^{\pi_1(\fL_k)}.$$
%

\begin{prop}[\cite{Losev4}, Lem 2.8]\label{prop:partialdecomp}
There is a linear isomorphism
%
\begin{equation}\label{eq:partialdecomp}\fP(\widetilde{\OO}) \simeq H^2(\widetilde{\OO},\CC) \oplus \bigoplus_k \fP_k(\widetilde{\OO}).\end{equation}
\end{prop}

Comparing Propositions \ref{prop:Namikawacenter} and \ref{prop:partialdecomp}, we arrive at the following (purely geometric) criterion for birational rigidity.

\begin{prop}[Proposition 3.7.1, \cite{MBMat}]\label{prop:criterionbirigidcover}
Let $\widetilde{\OO} \in \Cov(G)$. Then $\widetilde{\OO}$ is birationally rigid if and only if the following conditions hold:
\begin{itemize}
    \item[(i)]  $H^2(\widetilde{\OO},\CC)=0$.
    \item[(ii)] $\Spec(\CC[\widetilde{\OO}])$ has no codimension 2 leaves.
\end{itemize}
\end{prop}

We note that the spaces $H^2(\widetilde{\OO},\CC)$ and $\fP_k(\widetilde{\OO})$ admit \emph{Lie-theoretic descriptions}. We begin by describing $H^2(\widetilde{\OO},\CC)$. Assume for simplicity that $G$ is simply connected and semisimple. Let $R$ denote the reductive part of the stabilizer of $e \in \OO$ and let $\mathfrak{r}$ be its Lie algebra. We note that $\fr$ does not depend on the choice of $e$ in $\OO$, and the adjoint action of $R$ on $\fz(\fr)$ factors through $R/R^{\circ} \simeq \pi_1(\widetilde{\OO})$. 

\begin{lemma}[Lemma 7.2.7, \cite{LMBM}]\label{lem:coputeH2}
There is a natural identification
%
$$H^2(\widetilde{\OO},\CC) \simeq \fz(\mathfrak{r})^{\pi_1(\widetilde{\OO})}$$    
\end{lemma}

\begin{rmk}\label{rmk:H2}
If $\widetilde{\OO} = \widehat{\OO}$ is the \emph{universal} cover of $\OO$, then $H^2(\widehat{\OO},\CC) \simeq \fz(\mathfrak{r})$ by Lemma \ref{lem:computeH2}. In particular,  $H^2(\widehat{\OO},\CC)=0$ if and only if $\mathfrak{r}$ is semisimple. On the other hand, if $\widetilde{\OO} = \OO$, then $H^2(\widetilde{\OO},\CC) \simeq \fz(\mathfrak{r})^{\pi_1(\OO)}$ was computed in every case by Biswas and Chatterjee in \cite{BISWAS}. 
\end{rmk}

We proceed to describing the partial Namikawa spaces $\fP_k(\widetilde{\OO})$. Assume that $H^2(\widetilde{\OO},\CC)=0$. Suppose $Q \subset G$ is a parabolic subgroup with Levi factor $M$ and $\widetilde{\OO}_M \in \Cov(M)$ satisfies $\widetilde{\OO}=\mathrm{Bind}^G_M \widetilde{\OO}_M$. The triple $(Q,M,\widetilde{\OO}_M)$ gives rise to a projective birational morphism (generalizing the map $Y \to \Spec(\CC[\widetilde{\OO}])$)
%
\begin{equation}\label{eq:partialresolution}
\rho: G \times^Q (\Spec(\CC[\widetilde{\OO}_{M}]) \times \fq^{\perp}) \to \Spec(\CC[\widetilde{\OO}])\end{equation}
%
\begin{prop}[Prop 7.5.6, \cite{LMBM}]\label{prop:adaptedresolutiondatum}
For each codimension 2 leaf $\fL_k \subset \widetilde{X}$, there is a unique pair $(M_k,\widetilde{\OO}_{M_k})$ consisting of a Levi subgroup $M_k \subset G$ and a nilpotent cover $\widetilde{\OO}_{M_k} \in \Cov(M_k)$ such that
\begin{itemize}
    \item[(i)] $L \subset M_k$.
    \item[(ii)] $\widetilde{\OO} = \mathrm{Bind}^G_{M_k} \widetilde{\OO}_{M_k}$.
    \item[(iii)] For any parabolic $Q \subset G$ with Levi factor $M_k$, the morphism (\ref{eq:partialresolution}) resolves $\Sigma_k$ and preserves $\Sigma_j$ for $j\neq k$.
\end{itemize}
\end{prop}

The pair $(M_k,\widetilde{\OO}_{M_k})$ appearing in Proposition \ref{prop:adaptedresolutiondatum} is called the $\fL_k$-\emph{adapted resolution datum.} 

\begin{prop}[Proposition 3.6.4, \cite{MBMat}]
Let $\fL_k \subset \Spec(\CC[\widetilde{\OO}])$ be a codimension 2 leaf and let $(M_k, \widetilde{\OO}_{M_k})$ be the $\fL_k$-adapted resolution datum. Then the isomorphism $\fP(\widetilde{\OO}) \simeq \fz(\fl \cap [\fg,\fg])$ of Proposition \ref{prop:Namikawacenter} restricts to an isomorphism $\fP_k(\widetilde{\OO}) \simeq \fz(\fm_k \cap [\fg,\fg])$
\end{prop}

We conclude by sketching a simpe criterion for birational induction. For any $\OO \in \Orb(G)$, let $\mathcal{P}_{rig}(\OO)$ denote the set of $G$-conjugacy classes of pairs $(L,\OO_L)$ consisting of a Levi subgroup $L \subset G$ and a rigid nilpotent orbit $\OO_L \in \Orb(L)$ such that $\OO=\Ind^G_L \OO_L$. \todo{note on how to compute this set}Consider the integer
%
\begin{equation}\label{eq:m(O)}
m(\OO) = \max \{\dim \fz(\fl) \mid (L,\OO_L) \in \mathcal{P}_{rig}(\OO)\}.\end{equation}

\begin{lemma}\label{lem:bindcriterion}
Suppose $m(\OO) = \dim \fP(\OO)$ and there is a unique pair $(L,\OO_L) \in \mathcal{P}_{rig}(\OO)$ such that $\dim(\fz(\fl)) = m(\OO)$. Then $\OO=\Bind^G_L \OO_L$. 
\end{lemma}

\begin{proof}
    
\end{proof}

\subsection{Unipotent ideals and bimodules}\label{subsec:unipotent}

In \cite[Section 6]{LMBM}, we define a map
%
$$I: \Cov(G) \to \{\text{maximal ideals in } U(\fg)\}$$
%
The image of this map is the set of \emph{unipotent ideals} in $U(\fg)$. If $\widetilde{\OO} \in \Cov(G)$, denote by $\gamma(\widetilde{\OO}) \in \fh^*/W$ the infinitesimal character of $I(\widetilde{\OO})$. 

We will need several basic facts about unipotent ideals and their infinitesimal characters.

\begin{prop}[Propositions 6.5.4, 8.1.1, \cite{LMBM}]\label{prop:unipotentfacts}
The following are true:
\begin{itemize}
    \item[(i)] If $\widetilde{\OO},\widehat{\OO} \in \Cov(G)$, then 
    %
    $$I(\widetilde{\OO}) = I(\widehat{\OO}) \iff \widetilde{\OO} \sim \widehat{\OO}.$$
    \item[(ii)] Suppose $L \subset G$ is a Levi subgroup. Let $\widetilde{\OO}_L \in \Cov(L)$ and $\widetilde{\OO} = \Bind^G_L \widetilde{\OO}_L$. Then 
    %
    $$\gamma(\widetilde{\OO}_L) = \gamma(\widetilde{\OO})$$
    %
    in $\fh^*/W$. 
\end{itemize}
\end{prop}


\begin{cor}\label{cor:bindequivalence}
$\Bind^G_L$ descends to a map on equivalence classes
    %
    $$\Bind^G_L: \underline{\Cov}(L) \to \underline{\Cov}(G)$$
\end{cor}

\begin{proof}
Suppose $\widetilde{\OO}_L \sim \widehat{\OO}_L$ in $\Cov(L)$ and let $\widetilde{\OO} = \Bind^G_L \widetilde{\OO}_L$, $\widehat{\OO} = \Bind^G_L \widehat{\OO}_L$. By (i) and (ii) of Proposition \ref{prop:unipotentfacts}, we have
%
$$\gamma(\widetilde{\OO}) = \gamma(\widehat{\OO})$$
%
But $I(\widetilde{\OO})$ and $I(\widehat{\OO})$ are maximal ideals in $U(\fg)$, and hence uniquely determined by their infinitesimal characters. So in fact
%
$$I(\widetilde{\OO}) = I(\widehat{\OO})$$
%
and therefore $\widetilde{\OO} \sim \widehat{\OO}$ by Proposition \ref{prop:unipotentfacts}(i).
\end{proof}

\begin{prop}
Suppose $G$ is a simple group of classical type. If $\widetilde{\OO}_L \in \Cov(L)$ is maximal in its equivalence class, then $\Bind^G_L \widetilde{\OO}_L \in \Cov(G)$ is maximal in its equivalence class. 
\end{prop}

\begin{proof}
\todo{Mitya write -- also this doesnt appear to be cited anywhere}
\end{proof}

For $\widetilde{\OO} \in \Cov(G)$, let $\HC^G(U(\fg)/I(\widetilde{\OO}))$ denote the category of Harish-Chandra $U(\fg)$-bimodules annihilated (on both sides) by $I(\widetilde{\OO})$. This is a monoidal category under $\otimes_{U(\fg)}$. In \cite{LMBM}, this category is described in terms of representations of a certain finite group. Let $\widetilde{\OO}_{max} \in \Cov(G)$ denote the maximal cover in the equivalence class $[\widetilde{\OO}]$ and let
%
$$\Gamma(\widetilde{\OO}) := \Aut(\widetilde{\OO}_{max},\OO)$$
%
Note that $\Gamma(\widetilde{\OO})$ is a finite group. 

\begin{theorem}[Theorem 6.6.2, \cite{LMBM}]\label{thm:classificationHC}
Let $\widetilde{\OO} \in \Cov(G)$. Then there is an equivalence of monoidal categories
%
$$\HC^G(U(\fg)/I(\widetilde{\OO})) \simeq \Gamma(\widetilde{\OO})\modd$$
\end{theorem}








\section{Main results}\label{sec:mainresults}

If $\OO \in \Orb(G)$, write $\OO_{univ} \in \Cov(G)$ for the universal $G$-equivariant cover of $\OO$.

\begin{prop}\label{prop:distinguishedbirigid}
The following are true:\todo{rewrite in terms of Achar data (no Sommers data)}
\begin{itemize}
    \item[(i)] Suppose $(M^{\vee},\OO_{M^{\vee}}) \in \Som_{large}(G^{\vee})$ and $\pi(M^{\vee},\OO_{M^{\vee}}) \in \Ach(G^{\vee})$ is special and distinguished and let $\mathfrak{r}$ denote the reductive part of the centralizer of an element in $\underline{d}_S(M^{\vee},\OO_{M^{\vee}})$. Then $Z(\mathfrak{r})=0$.
    \item[(ii)] Suppose $(M^{\vee},\OO_{M^{\vee}}) \in \Som_{large}(G^{\vee})$ and $\pi(M^{\vee},\OO_{M^{\vee}}) \in \Ach(G^{\vee})$ is special and distinguished. Then $\underline{d}_S(M^{\vee},\OO_{M^{\vee}})_{univ}$ is birationally rigid.
    \item[(iii)] Suppose $(M^{\vee},\OO_{M^{\vee}}), (N^{\vee},\OO_{N^{\vee}}) \in \Som_{large}(G^{\vee})$, $\pi(M^{\vee},\OO_{M^{\vee}}), \pi(N^{\vee}_1,\OO_{N^{\vee}}) \in \Ach(G^{\vee})$ are special and distinguished, and
    %
$$\underline{d}_S(M^{\vee},\OO_{M^{\vee}}) = \underline{d}_S(N^{\vee},\OO_{N^{\vee}})$$
    %
    Then $G^{\vee} \cdot \OO_{M^{\vee}} = G^{\vee} \cdot \OO_{N^{\vee}}$.
\end{itemize}
\end{prop}

\begin{proof}
If $G$ is a simple adjoint group of classical (resp. exceptional) type, then (i), (ii), and (iii) are proved in Section \ref{subsec:proofsclassical1} (resp. Section \ref{subsec:proofsexceptional1}). Thus, it suffices to explain how to reduce to this case. 

In claims (i) and (iii) all of the relevant objects are independent of isogeny. Moreover, if $\fg=\fg_1 \times \fg_2$, then $\Som_{large}(G^{\vee}) = \Som_{large}(G_1^{\vee}) \times \Som_{large}(G_2^{\vee})$, $\Ach(G^{\vee}) = \Ach(G^{\vee}_1) \times \Ach(G^{\vee}_2)$, $\Orb(G) = \Orb(G_1) \times \Orb(G_2)$, and $\underline{d}_S^G = \underline{d}_S^{G_1} \times \underline{d}_S^{G_2}$. To complete the reduction, we note that the condition $Z(\mathfrak{r})=0$ holds for a product $\OO_1 \times \OO_2$ if and only if it holds for $\OO_1$ and $\OO_2$.

For (ii), the cover $\underline{d}_S(M^{\vee},\OO_{M^{\vee}})_{univ} \in \Cov(G)$ depends on the isogeny, so some care is required. Suppose there is an isogeny $G^{\vee}_1 \times G^{\vee}_2 \to G^{\vee}$ and that the assertion in (ii) holds for both $G_1$ and $G_2$. For $(M^{\vee},\OO_{M^{\vee}})$ as in the statement of (i), let $\widetilde{\OO} = \underline{d}_S(M^{\vee},\OO_{M^{\vee}})_{univ} \in \Cov(G)$ and let $\widehat{\OO} = \underline{d}_S^{G_1 \times G_2}(M^{\vee},\OO_{M^{\vee}})_{univ} \in \Cov(G_1 \times G_2)$. Pulling back along the isgoney $G \to G_1 \times G_2$, we can regard $\widehat{\OO}$ as an element of $\Cov(G)$. Note that there is a ($G$-equivariant) covering map $\widetilde{\OO} \to \widehat{\OO}$. By our assumption, $\widehat{\OO}$ is birationally rigid. We wish to show that the same is true of $\widetilde{\OO}$. By Proposition \ref{prop:criterionbirigidcover}, it suffices to show that $H^2(\widetilde{\OO},\CC)=0$ and $\Spec(\CC[\widetilde{\OO}])$ has no codimension 2 leaves. By Lemma \ref{lem:coputeH2}, $H^2(\widetilde{\OO},\CC) \subset Z(\mathfrak{r})$, where $\mathfrak{r}$ denotes the reductive part of the centralizer of an element in $\OO$, and by (i), $Z(\mathfrak{r})=0$. Hence, $H^2(\widetilde{\OO},\CC)=0$. Since $\widehat{\OO}$ is birationally rigid, Proposition \ref{prop:criterionbirigidcover} implies that $\Spec(\CC[\widehat{\OO}])$ has no codimension 2 leaves. Since $\widetilde{\OO}$ covers $\widehat{\OO}$, the same is true of $\Spec(\CC[\widetilde{\OO}])$, see  \cite[Lemma 7.6.6]{LMBM}. So $\widetilde{\OO}$ is birationally rigid.
\end{proof}

Now suppose $(\OO^{\vee},\bar{C}) \in \Ach^*(G^{\vee})$ is a distinguished Achar datum. Let $(M^{\vee},\OO_{M^{\vee}}) = \alpha(\OO^{\vee},\bar{C}) \in \Som_{large}(G^{\vee})$. Then $\pi(M^{\vee},\OO_{M^{\vee}}) = (\OO^{\vee},\bar{C})$ and $d_S(\OO^{\vee},\bar{C}) = \underline{d}_S(M^{\vee},\OO_{M^{\vee}})$, see Lemma \ref{lem:SomAch}(ii). So by Proposition \ref{prop:distinguishedbirigid}(i), $d_S(\OO^{\vee},\bar{C})_{univ}$ is birationally rigid. Consider the map
%
$$D_0: \Ach^*_0(G^{\vee}) \to \Cov_0(G), \qquad D_0(L^{\vee},(\OO_{L^{\vee}},\bar{C}_{L^{\vee}})) = (L,d_S^L(\OO_{L^{\vee}},\bar{C}_{L^{\vee}})_{univ})$$
%
We define $D$ to be the composition
%
$$D: \Ach^*(G^{\vee}) \overset{\Sat^{-1}}{\to} \Ach_0^*(G^{\vee}) \overset{D_0}{\to} \Cov_0(G) \overset{\Bind}{\to} \Cov(G)$$
%
where $\Sat^{-1}$ is the map of Proposition \ref{prop:specialtospecial}(ii). 


\begin{prop}\label{prop:propsofD}
The map 
%
$$D: \Ach^*(G^{\vee}) \to \Cov(G)$$
%
has the following properties:
\begin{itemize}
    \item[(i)] $D$ is injective (and in fact, remains injective after composition with $\Cov(G) \twoheadrightarrow \underline{\Cov}(G)$).
    \item[(ii)] If $(\OO^{\vee},\bar{C})$ is distinguished, then $D(\OO^{\vee},\bar{C})$ is birationally rigid.
    \item[(iii)] If $L \subset G$ is a Levi subgroup, then
    %
    $$D^G \circ \Sat^{G^{\vee}}_{L^{\vee}} = \Bind^G_L \circ D^L $$
\end{itemize}
\end{prop}

\begin{proof}
(ii) follows immediately from the definition of $D$. We proceed to proving (i). Recall that $\Sat^{-1}: \Ach^*(G^{\vee}) \to \Ach^*_0(G^{\vee})$ is injective by Proposition \ref{prop:specialtospecial}(ii) and $\Bind: \Cov_0(G) \to \Cov(G)$ is injective by Proposition \ref{prop:bindinjective}. Thus, it is enough to show that $D_0$ is injective, or, equivalently, that $(\OO^{\vee},\bar{C}) \mapsto d_S(\OO^{\vee},\bar{C})_{univ}$ is injective on special distinguished Achar data. Suppose $(\OO^{\vee}_1,\bar{C}_1), (\OO^{\vee}_2,\bar{C}_2) \in \Ach^*(G^{\vee})$ are two such Achar data such that $D(\OO^{\vee}_1,\bar{C}_1) = D(\OO^{\vee}_2,\bar{C}_2)$. Let $(M^{\vee}_1,\OO_{M^{\vee}_1}) = \alpha(\OO^{\vee}_1,\bar{C}_1)$ and  $(M^{\vee}_2,\OO_{M^{\vee}_2}) = \alpha(\OO^{\vee}_2,\bar{C}_2)$. Then $\underline{d}_S(M_1^{\vee},\OO_{M^{\vee}_1}) = d_S(\OO^{\vee}_1,\bar{C}_1) = d_S(\OO^{\vee}_2,\bar{C}_2) = \underline{d}_S(M^{\vee}_2,\OO_{M^{\vee}_2})$. So by Proposition \ref{prop:distinguishedbirigid}(ii), $G^{\vee}\cdot \OO_{M^{\vee}_1} = G^{\vee}\cdot \OO_{M^{\vee}_2}$. Then by Proposition \ref{prop:twodiagramsAbar}(ii), $(\OO^{\vee}_1,\bar{C}_1)=(\OO^{\vee},\bar{C}_2)$, as asserted.

For (iii), let $L \subset G$ be a Levi subgroup of $G$ and let $(\OO_{L^{\vee}},\bar{C}_{L^{\vee}}) \in \Ach^*(L^{\vee})$. Suppose $\Sat(K^{\vee},(\OO_{K^{\vee}},\bar{C}_{K^{\vee}})) = (\OO_{L^{\vee}},\bar{C}_{L^{\vee}})$ for $(K^{\vee},(\OO_{K^{\vee}},\bar{C}_{K^{\vee}})) \in \Ach^*_0(L^{\vee})$ and let $\widetilde{\OO}_K = d_S^K(\OO_{K^{\vee}},\bar{C}_{K^{\vee}})_{univ}$. Then
%
$$D^G(\Sat^{G^{\vee}}_{L^{\vee}}(\OO_{L^{\vee}},\bar{C}_{L^\vee}) = \Bind^G_K\widetilde{\OO}_L$$
%
whereas
%
$$\Bind^G_L(D^L(\OO_{L^{\vee}},\bar{C}_{L^\vee})) = \Bind^G_L \Bind^L_K \widetilde{\OO}_K.$$
%
Now (iii) is immediate from the transitivity of birational induction, see Proposition \ref{prop:propsofbind}(i).
\end{proof}

\begin{rmk}
We note that $D$ generalizes the duality maps of Barbasch-Vogan-Lusztig-Spaltenstein, Sommers, Achar, and Losev-Mason-Brown-Matvieievskyi. More precisely, if $(\OO^{\vee},\bar{C}) \in \Ach^*(G^{\vee})$, then
\begin{itemize}
    \item[(i)] $D(\OO^{\vee},\bar{C})$ is a cover of $d_S(\OO^{\vee},\bar{C})$.
    \item[(ii)] If $\bar{C}=1$, then $D(\OO^{\vee},\bar{C}) = d_{LMBM}(\OO^{\vee})$.
    \item[(iii)]  If $\bar{C}=1$, then $D(\OO^{\vee},\bar{C})$ is a cover of $d_{BV}(\OO^{\vee})$.
    \item[(iv)] Compatibility with Achar??
\end{itemize}
Only (iv) requires comment.\todo{say something!}
\end{rmk}

Let $\gamma \in \fh^*$. Recall the subgroups $L^{\vee}_{\gamma,0} \subset L^{\vee}_{\gamma} \subset G^{\vee}$ defined in Section \ref{subsec:maximal}. Consider the Sommers datum
%
$$\Som(\gamma) := (L^{\vee}_{\gamma}, \Ind^{L^{\vee}_{\gamma}}_{L^{\vee}_{\gamma,0}}\{0\}) \in \Som(G^{\vee})$$
%
This defines a map
%
$$\Som: \fh^*/W \to \Som(G^{\vee})$$
%
Composing with $\pi: \Som(G^{\vee}) \to \Ach(G^{\vee})$, we get a further map
%
$$\Ach: \fh^*/W \to \Ach(G^{\vee}).$$

Choose a $W$-invariant non-degenerate symmetric form on $\fh^*$ and write $\lVert \cdot \rVert$ for the associated length function\footnote{S.Y.: I've changed $|\cdot|$ to $\lVert \cdot \rVert$ since we are also using $|\cdot|$ for the size of a partition. It could be confusing especially during the proofs for classical types}.

\begin{theorem}\label{thm:inflchars}
Let $(\OO^{\vee},\bar{C}) \in \Ach^*(G^{\vee})$. Then there is a unique minimal-length $W$-orbit
%
$$\gamma(\OO^{\vee},\bar{C}) \in \fh^*/W$$
%
such that $\Ach(\gamma(\OO^{\vee},\bar{C})) = (\OO^{\vee},\bar{C})$. Furthermore,
%
$$\gamma(\OO^{\vee},\bar{C}) = \gamma(D(\OO^{\vee},\bar{C})).$$
\end{theorem}

\begin{proof}
Arguing as in the proof of Proposition \ref{prop:distinguishedbirigid}, we can reduce to the case when $G$ is a simple group of adjoint type. The classical cases are handled in Section \ref{subsec:proofsclassical2}. The exceptional cases are handled in Section \ref{subsec:proofsexceptional1}.
\end{proof}


\begin{lemma}\label{lem:lift}
Suppose $(\OO^{\vee},\bar{C}) \in \Ach^*(G^{\vee})$ is distinguished and let
%
$$R^{\vee} = Z_{G^{\vee}}(\exp(2\pi i \gamma(\OO^{\vee},\bar{C})))^{\circ}, \qquad \OO_{R^{\vee}} = \OO^{\vee} \cap \mathfrak{r}^{\vee}.$$
%
Then the following are true:
\begin{itemize}
    \item[(i)] $\OO_{R^{\vee}}$ is a distinguished nilpotent $R^{\vee}$-orbit.
    \item[(ii)] $\pi(R^{\vee},\OO_{R^{\vee}}) = (\OO^{\vee},\bar{C})$.
\end{itemize}
\end{lemma}

\begin{proof}
\todo{prove this}
\end{proof}

Using Lemma \ref{lem:lift}, we will define an injective map
%
$$\mathbb{L}: \Ach^*(G^{\vee}) \to \Som(G^{\vee}).$$
%
This map is defined as follows. Let $(\OO^{\vee},\bar{C}) \in \Ach^*(G^{\vee})$. Choose $(L^{\vee},(\OO_{L^{\vee}},\bar{C}_{L^{\vee}})) \in \Ach^*_0(G^{\vee})$ such that $(\OO^{\vee},\bar{C}) = \Sat(L^{\vee},(\OO_{L^{\vee}},\bar{C}_{L^{\vee}}))$. Let
%
$$s = \exp(2\pi i \gamma(\OO,\bar{C})), \qquad R^{\vee} = Z_{G^{\vee}}(s)^{\circ}, \qquad R^{\vee}_0 = Z_{L^{\vee}}(s)^{\circ}, \qquad \OO_{R^{\vee}_0} = \mathfrak{r}^{\vee}_0 \cap \OO^{\vee}.$$
%
By Lemma \ref{lem:lift}, $(R_0^{\vee},\OO_{R^{\vee}_0}) \in \Som_{large}(L^{\vee})$. Define
%
$$\mathbb{L}(\OO^{\vee},\bar{C}) = (R^{\vee},\Sat^{R^{\vee}}_{R^{\vee}_0} \OO_{R^{\vee}_0})$$
%
\begin{lemma}\label{lem:liftproperties}
The map $\mathbb{L}: \Ach^*(G^{\vee}) \to \Som(G^{\vee})$ is right inverse to $\pi$. In particular, it is injective. 
\end{lemma}

\begin{proof}
We can assume without loss that $Z(G^{\vee})$ is connected. Since $R^{\vee}$ (resp. $R^{\vee}_0$) is the connected centralizer of $s$, the image of $s$ generates the cyclic group $Z(R^{\vee})/Z(R^{\vee})^{\circ}$ (resp. $Z(R^{\vee}_0)/Z(R^{\vee}_0)^{\circ}$), see \cite[Remark 3]{Sommers1998}. So, by definition
%
$$\pi^{G^{\vee}}(R^{\vee},\Sat^{R^{\vee}}_{R^{\vee}_0} \OO_{R^{\vee}_0}) = (\Sat^{G^{\vee}}_{R^{\vee}}\OO_{R^{\vee}},\bar{s}), \qquad \pi^{L^{\vee}}(R^{\vee}_0,\OO_{R^{\vee}_0}) = (\Sat^{L^{\vee}}_{R^{\vee}_0}\OO_{R^{\vee}_0}, \bar{s}).$$
%
Hence,
%
$$\pi^{G^{\vee}}(R^{\vee},\Sat^{R^{\vee}}_{R^{\vee}_0} \OO_{R^{\vee}_0}) = \Sat^{G^{\vee}}_{L^{\vee}} \pi^{L^{\vee}}(R^{\vee}_0,\OO_{R^{\vee}_0})$$
%
But by Lemma \ref{lem:lift}(ii),, $\pi^{L^{\vee}}(R^{\vee}_0,\OO_{R^{\vee}_0}) = (\OO_{L^{\vee}},\bar{C}_{L^{\vee}})$. So
%
$$\pi^{G^{\vee}}(\mathbb{L}(\OO^{\vee},\bar{C})) = \pi^{G^{\vee}}(R^{\vee},\Sat^{R^{\vee}}_{R^{\vee}_0} \OO_{R^{\vee}_0}) = \Sat^{G^{\vee}}_{L^{\vee}}(\OO_{L^{\vee}},\bar{C}_{L^{\vee}}) = (\OO^{\vee},\bar{C}).$$
%
This completes the proof.
\end{proof}

\begin{theorem}\label{thm:Gamma}
Assume $G$ is adjoint. Let $(\OO^{\vee},\bar{C}) \in \Ach^*(G^{\vee})$ and let $(R^{\vee},\OO_{R^{\vee}}) = \mathbb{L}(\OO^{\vee},\bar{C})$. Then there is a group isomorphism
%
$$\bar{A}(\OO_{R^{\vee}}) \simeq \Gamma(D(\OO^{\vee},\bar{C})).$$
\end{theorem}

\begin{proof}
Arguing as in the proof of Proposition \ref{prop:distinguishedbirigid}, we can reduce to the case when $G$ is a simple group of adjoint type. For $G$ a group, see Lemma \ref{lem:Gammaclassical}. For $G$ exceptional, see Section \ref{subsec:proofsexceptional2}. 
\end{proof}

\begin{rmk}\label{rmk:even}
We note that there is a case-free proof of Theorem \ref{thm:Gamma} in the following special case: $\OO^{\vee}$ is even and $\bar{C}=1$. Under these assumptions, $(R^{\vee},\OO_{R^{\vee}}) = (G^{\vee},\OO^{\vee})$ and $I(\widetilde{\OO}) = J(\gamma_{\OO^{\vee}})$, cf. ?? \todo{Reference missing}. So it suffices to show that $\bar{A}(\OO^{\vee}) \simeq \Gamma(D(\OO^{\vee},\bar{C}))$. Let $\OO=d(\OO^{\vee})$. By \cite[Proposition 7.4 and Theorem 6.1]{LosevHC}, there is a monoidal equivalence
%
$$\HC^G(U(\fg)/J(\gamma_{\OO^{\vee}})) \simeq \bar{A}(\OO)\modd$$
%
And by \cite[Theorem 6.6.2]{LMBM}, there is a monoidal equivalence
%
$$\HC^G(U(\fg)/J(\gamma_{\OO^{\vee}})) \simeq \Gamma(D(\OO^{\vee},\bar{C}))\modd$$
%
So by the Tannakian formalism, there is a group isomorphism $\bar{A}(\OO) \simeq \Gamma(D(\OO^{\vee},\bar{C}))$. Since $\OO^{\vee}$ is even, and hence special, there is a further isomorphism $\bar{A}(\OO^{\vee}) \simeq \bar{A}(\OO)$, see \cite{Lusztig1984}. Thus, $\bar{A}(\OO^{\vee}) \simeq \Gamma(D(\OO^{\vee},\bar{C}))$, as asserted.
\end{rmk}

Combining Theorem \ref{thm:Gamma} with Theorem \ref{thm:classificationHC}, we arrive at the following result.

\begin{cor}\label{cor:HC}
Assume $G$ is adjoint. Let $(\OO^{\vee},\bar{C}) \in \Ach^*(G^{\vee})$. Let $\mathbb{L}(\OO^{\vee},\bar{C}) = (R^{\vee},\OO_{R^{\vee}})$ and $\widetilde{\OO} = D(\OO^{\vee},\bar{C})$. Then there is an equivalence of monoidal categories
%
$$\HC^G(U(\fg)/I(\widetilde{\OO})) \simeq \bar{A}(\OO_{R^{\vee}})\modd $$
\end{cor}

\begin{rmk}
Corollary \ref{cor:HC} implies that the unipotent representations attached to $\widetilde{\OO}$ are in one-to-one correspondence with irreducible representations of $\bar{A}(\OO_{R^{\vee}})$. In the special case when $\OO^{\vee}$ is even and $\bar{C}=1$, this (weaker) statement was proved in \cite[Theorem III]{BarbaschVogan1985}.
\end{rmk}



\begin{comment}
    For the cases of type $B$ and $D$, the proof is similar. The only difference is that, for an orbit of type $B$ or $D$ of the form
	  	\[   \OO = (a_{2q+1} \geqslant a_{2q} \geqslant \cdots \geqslant a_0 ) \cup (\mu, \mu) \]
	with  the centralizers now look like
	\[  L^{\tilde{\psi}}  \simeq S( \underbrace{O(a_{2q+1} - a_{2q})^1_\Delta \times Sp(a_{2q} - a_{2q-1})^2_\Delta \times \cdots \times \textcolor{red}{O (a_{2i+1}-\mu)^{2q-2i+1}_\Delta } }_{M} 
	\textcolor{red}{\times}
	\underbrace{ \textcolor{red}{ O(\mu - a_{2i})^{2q-2i+3}_\Delta} \times  \cdots  \times Sp(a_0)^{2q+4}_\Delta }_{N} ) \]
	and
	\[  L^{\psi} \simeq \textcolor{blue}{GL(\mu)} \times S ( \underbrace{O(a_{2q+1} - a_{2q})^1_\Delta \times Sp(a_{2q} - a_{2q-1})^2_\Delta \times \cdots  \times \textcolor{red}{O (a_{2i+1} - a_{2i})^{2q-2i+1}_\Delta} \times  \cdots  \times Sp(a_0)^{2q+2}_\Delta}_{Q} ). \]
	Note that $L^{\tilde{\psi}}$ stays the factor if the multiplicity of each factor after and including $O(\mu - a_{2i})^{2q-2i+3}_\Delta$ drops by 2:
	\[  L^{\tilde{\psi}}  \simeq S( \underbrace{O(a_{2q+1} - a_{2q})^1_\Delta \times Sp(a_{2q} - a_{2q-1})^2_\Delta \times \cdots \times \textcolor{red}{O (a_{2i+1}-\mu)^{2q-2i+1}_\Delta } }_{M} 
	\textcolor{red}{\times}
	\underbrace{ \textcolor{red}{ O(\mu - a_{2i})^{2q-2i+1}_\Delta} \times  \cdots  \times Sp(a_0)^{2q+2}_\Delta }_{N} ). \]
	We then have a natural inclusion $O (a_{2i+1}-\mu)^{2q-2i+1}_\Delta \times O(\mu - a_{2i})^{2q-2i+1}_\Delta \hookrightarrow O (a_{2i+1} - a_{2i})^{2q-2i+1}_\Delta$. Then the remaining description of the inclusion $L^{\tilde{\psi}} \hookrightarrow L^\psi$ is the same as the case of type $C$.
	
	({\bf Alternative proof: repeat the exact same proof of type $C$ for $O(2n+1)$ and $O(2n)$} and then restrict to the special orthogonal groups). 
\end{comment}	

==> introduction__first_draft_.tex <==

\section{Introduction}

Let $G$ be a complex reductive algebraic group with Lie algebra $\fg$. A \emph{nilpotent cover} is a finite connected $G$-equivariant cover of a nilpotent co-adjoint orbit $\OO \subset \fg^*$. Write $\Cov(G)$ for the (finite) set of isomorphism classes of nilpotent covers for $G$. In \cite{LMBM}, we attach to each nilpotent cover $\widetilde{\OO}$ a finite set $\mathrm{Unip}_{\widetilde{\OO}}(G)$ of irreducible unitary representations of $G$ called \emph{unipotent representations}. Such representations possess a variety of special properties and are conjectured to form the building blocks of the unitary dual. They include, as a proper subset, all special unipotent representations in the sense of Arthur (\cite{Arthur1983}) and Barbasch-Vogan (\cite{BarbaschVogan1985}).The purpose of this article is to give a description of the sets $\mathrm{Unip}_{\widetilde{\OO}}(G)$ in terms of the Langlands dual group $G^{\vee}$. 

Our description involves several types of parameters related to $G^{\vee}$, which we will now briefly describe:
\begin{itemize}
    \item A \emph{Lusztig-Achar datum} for $G^{\vee}$ is a pair $(\OO^{\vee},\bar{C})$ consisting of a nilpotent orbit $\OO^{\vee} \subset \fg^{\vee}$ and a conjugacy class $\bar{C}$ in Lusztig's canonical quotient $\bar{A}(\OO^{\vee})$ of the $G^{\vee}$-equivariant fundamental group of $\OO^{\vee}$, see Section \ref{subsec:Abar}. Write $\LA(G^{\vee})$ for the (finite) set of Lusztig-Achar data for $G^{\vee}$. We will also consider a subset $\LA^*(G^{\vee}) \subset \LA(G^{\vee})$ defined in \cite[Section 3]{Achar2003}. This subset includes, as a proper subset, all pairs of the form $(\OO^{\vee},1)$ --- its elements are called \emph{special Lusztig-Achar data}.
    \item A \emph{McNinch-Sommers datum} for $G^{\vee}$ is a triple $(L^{\vee},tZ^{\circ},\OO_{L^{\vee}})$ consisting of a connected reductive subgroup $L^{\vee} \subset G^{\vee}$, a coset $tZ^{\circ}$ in the component group of $Z=Z(L)$ such that $L^{\vee}=Z_{G^{\vee}}(t)^{\circ}$, and a nilpotent orbit $\OO_{L^{\vee}} \subset \fl^{\vee}$. Write $\MS(G^{\vee})$ for the (finite) set of $G^{\vee}$-conjugacy classes of McNinch-Sommers data for $G^{\vee}$.
\end{itemize}
Choose a Cartan subalgebra $\fh \subset \fg$ and let $W$ denote the Weyl group. We define in Section \ref{subsec:Achar} natural surjective maps
%
$$\fh^*/W \twoheadrightarrow \MS(G^{\vee}) \twoheadrightarrow \LA(G^{\vee})$$
%
For each $(\OO^{\vee},\bar{C}) \in \LA^*(G^{\vee})$, we show in Theorem \ref{thm:inflchars} that there is a unique minimal-length element element $\gamma(\OO^{\vee},\bar{C}) \in \fh^*/W$ which maps to $(\OO^{\vee},\bar{C})$ under the composition above. This element determines an infinitesimal character for $U(\fg)$ by the Harish-Chandra isomorphism, and hence a maximal ideal $I(\OO^{\vee},\bar{C})$ in $U(\fg)$. We consider the finite set
%
\begin{align*}
\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G) = \{&\text{irreducible $G$-equivariant Harish-Chandra $U(\fg)$-bimodules}\\
&\text{which are annihilated on both sides by } I(
\OO^{\vee},\bar{C})\}.\end{align*}
%
The notation suggests a relationship between $\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G)$ and $\mathrm{Unip}_{\widetilde{\OO}}(G)$. To make this relationship precise, we define in Section \ref{sec:mainresults} a natural duality map
%
$$D: \LA^*(G^{\vee}) \to \Cov(G)$$
%
This map generalizes several well-known duality maps, including those of Barbasch-Vogan-Lusztig-Spaltenstein (\cite{BarbaschVogan1985}), Sommers (\cite{Sommers2001}), Achar (\cite{Achar2003}) and Mason-Brown-Matvieievskyi-Losev (\cite{LMBM}). It enjoys various nice properties. For example, it is injective and intertwines saturation of Lusztig-Achar data (an operation we define) with induction of nilpotent covers. Our first main result is the following.

\begin{theorem}[See Theorem \ref{thm:inflchars} below]\label{theorem:main1intro}
Let $(\OO^{\vee},\bar{C}) \in \LA^*(G^{\vee})$ and let $\widetilde{\OO} = D(\OO^{\vee},\bar{C})$. Then there is an equality
%
$$\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G) = \mathrm{Unip}_{\widetilde{\OO}}(G).$$
\end{theorem}

We define in Section \ref{sec:mainresults} an injective map
%
$$\mathbb{L}: \LA^*(G^{\vee}) \hookrightarrow \MS(G^{\vee})$$
%
which is right inverse to the projection $\MS(G^{\vee}) \twoheadrightarrow \LA(G^{\vee})$. Our second main result gives a parameterization of $\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G)$ in terms of the Langlands dual group. 

\begin{theorem}[See Corollary \ref{cor:HC} below]\label{theorem:main2intro}
Assume $G$ is adjoint. Let $(\OO^{\vee},\bar{C}) \in \LA^*(G^{\vee})$ and let $(R^{\vee},tZ^{\circ},\OO_{R^{\vee}}) = \mathbb{L}(\OO^{\vee},\bar{C})$. Then there is a natural bijection
%
$$\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G) \simeq \{\text{irreducible representations of } \bar{A}(\OO_{R^{\vee}})\}.$$
\end{theorem}
%
\begin{rmk}
In fact, the representations in $\mathrm{Unip}_{(\OO^{\vee},\bar{C})}(G)$ are the irreducible objects in a monoidal category $\HC^G(U(\fg)/I(\OO^{\vee},\bar{C}))$, defined in terms of the ideal $I(\OO^{\vee},\bar{C})$. The bijection in Theorem \ref{theorem:main2intro} comes from a monoidal equivalence of categories
%
$$\HC^G(U(\fg)/I(\OO^{\vee},\bar{C})) \simeq \bar{A}(\OO_{R^{\vee}})\modd$$
\end{rmk}

Now fix a nilpotent orbit $\OO^{\vee} \subset \fg^{\vee}$. Choose an $\mathfrak{sl}(2)$-triple $(e^{\vee},f^{\vee},h^{\vee})$ with $e^{\vee} \in \OO^{\vee}$. The corresponding map $\psi_{\OO^{\vee}}: SL(2) \to G^{\vee}$ is a unipotent Arthur parameter for the complex group $G$ and the corresponding Arthur packet coincides with the set $\mathrm{Unip}_{(\OO^{\vee},1)}(G)$. So in fact Theorem \ref{theorem:main2intro} provides, as a special case, a parameterization of the elements of the unipotent Arthur packets for a complex reductive group (such a parameterization was previously obtained in \cite{BarbaschVogan1985} and \cite{Wong2018} in the special case when $\OO^{\vee}$ is special). 

We conclude with a few remarks regarding symplectic duality, which appears to be connected, in somewhat mysterious ways, to the main results of this paper. In \cite[Section 9.3]{LMBM} it was conjectured that the nilpotent Slodowy slice $S^\vee$ to the orbit $\OO^\vee\subset \fg^\vee$ is symplectically dual to the affinization of the nilpotent cover $D(\OO^\vee, 1)$. In ongoing work, Finkelberg, Hanany, and Nakajima produce for each nilpotent orbit $\OO^{\vee} \subset \mathfrak{so}(2n)$, $\mathfrak{sp}(2n)$ an ortho-symplectic quiver gauge theory $Q$ with Higgs branch $S^\vee$ and Coulomb branch isomorphic to the affinization of a certain nilpotent cover of  $d(\OO^\vee)$ with Galois group $\bar{A}(\OO^\vee)$. It is reasonable to conjecture that this nilpotent cover is isomorphic to $D(\OO^{\vee},1)$. The results of this paper offer strong evidence in this direction; by Theorem \ref{thm:Gamma}, $D(\OO^{\vee},1)$ is a Galois cover with Galois group $\bar{A}(\OO^\vee)$. 

%In their ongoing work, Finkelberg, Hanany, and Nakajima produce an ortho-symplectic quiver gauge theory $Q$ such that the Higgs branch $\cM_H(Q)$ is isomorphic to $S^\vee$ and the Coulomb branch $\cM_C(Q)$ is isomorphic to the affinization of a cover of the orbit $d(\OO^\vee)$ with Galois group $\bar{A}(\OO^\vee)$. It is natural to conjecture that Thus, the results of this paper provide additional evidence for the conjecture in \cite[Section 9.3]{LMBM}. We remark that for $\fg=\fs\fp(2n)$, $\cM_C(Q)$ does not coincide with the affinization of a nilpotent cover, but the latter often can be considered as a local picture at the most singular point of $\cM_C(Q)$. We also note that covers of non-special orbits cannot be obtained by this construction. We would like to express our gratitude to Hiraku Nakajima for explaining these results.

